Anda: Unlocking Efficient LLM Inference with a Variable-Length Grouped Activation Data Format

The widely-used, weight-only quantized large language models (LLMs), which leverage low-bit integer (INT) weights and retain floating-point (FP) activations, reduce storage requirements while maintaining accuracy. However, this shifts the energy and latency bottlenecks towards the FP activations that are associated with costly memory accesses and computations. Existing LLM accelerators focus primarily on computation optimizations, overlooking the potential of jointly optimizing FP computations and data movement, particularly for the dominant FP-INT GeMM operations in LLM inference. To address these challenges, we investigate the sensitivity of activation precision across various LLM modules and its impact on overall model accuracy. Based on our findings, we first propose the Anda data type: an adaptive data format with group-shared exponent bits and dynamic mantissa bit allocation. Secondly, we develop an iterative post-training adaptive precision search algorithm that optimizes the bit-width for different LLM modules to balance model accuracy, energy efficiency, and inference speed. Lastly, a suite of hardware optimization techniques is proposed to maximally exploit the benefits of the Anda format. These include a bit-plane-based data organization scheme, Anda-enhanced processing units with bit-serial computation, and a runtime bit-plane Anda compressor to simultaneously optimize storage, computation, and memory footprints. Our evaluations on FPINT GeMM operations show that Anda achieves a 2.4x speedup, 4.0x area efficiency, and 3.1x energy efficiency improvement on average for popular LLMs including OPT, LLaMA, and LLaMA-2 series over the GPU-like FP-FP baseline. Anda demonstrates strong adaptability across various application scenarios, accuracy requirements, and system performance, enabling efficient LLM inference across a wide range of deployment scenarios.

==> 0-archive.tex <==
\section{Archive}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/precision_mapping_on_LLM_block.png}
%     \caption{Precision mapping for an LLM blocks.}
%     \label{fig:prec_map}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/dpu_pattern.png}
    \caption{(a) first-bit-plane-then-element reduction pattern; (b) first-element-then-bit-plane reduction pattern.}
    \label{fig:archive_dpu_pattern}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/mapping_gemm_to_mxu.png}
    \caption{Mapping GEMM into the MXU.}
    \label{fig:mapping_mxu}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/concept_fig_flexible.png}
%     \caption{[Concept Figure] Our arch strengths over the others.}
%     \label{fig:concept_flexible}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs. Key Metrics: Perplexity (Black, lower is better), OPS Reduction (Red), and Activation Tensor Size Compression Ratio (Blue).}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccccccc@{}}
% \toprule
% \multicolumn{2}{c|}{}                  & OPT-1.3B & OPT-6.7B & LLaMA-7B & LLaMA2-7B & OPT-13B & LLaMA-13B  & LLaMA2-13B & OPT-30B & LLaMA-30B  \\ \midrule
% \multirow{7}{*}{WikiText2} & Omniquant & 14.88    & 10.96    & 5.77     & 5.59      & 10.20   & 5.17       & 4.95       & 9.62    & 4.19       \\
%                            & AWQ       & 14.94    & 10.93    & 5.81     & 5.62      & 10.21   & 5.20       & 4.97       & 9.59    & 4.21       \\
%                            & GPTQ      & 14.89    & 10.93    & 5.85     & 5.61      & 10.17   & 5.20       & 4.98       & 9.58    & 4.23       \\
%                            & RTN       & 15.29    & 11.15    & 5.96     & 5.72      & 10.30   & 5.25       & 4.98       & 9.94    & 4.23       \\
%                            & FIGNA     & 14.90    & 10.96    & 5.78     & 5.60      & 10.22   & 5.18       & 4.96       & 9.61    & 4.20       \\
%                            & VSQuant   & 19.04    & 12.24    & 7.45     & 8.26      & 11.63   & 6.36       & 6.43       & 10.67   & 5.10       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \midrule
% \multirow{7}{*}{PTB}       & Omniquant & 17.40    & 13.25    & 8.97     & 21.52     & 12.46   & 8.14       & 30.19      & 11.94   & 7.39       \\
%                            & AWQ       & 17.46    & 13.28    & -        & -         & 12.46   & \textbf{-} & \textbf{-} & 11.90   & \textbf{-} \\
%                            & GPTQ      & 17.41    & 13.21    & -        & -         & 12.42   & \textbf{-} & \textbf{-} & 11.89   & \textbf{-} \\
%                            & RTN       & 33.63    & 16.05    & -        & -         & 15.40   & \textbf{-} & \textbf{-} & 14.17   & \textbf{-} \\
%                            & FIGNA     & 17.41    & 13.26    & 8.98     & 21.52     & 12.47   & 8.15       & 30.19      & 11.95   & 7.40       \\
%                            & VSQuant   & 25.64    & 15.50    & 15.78    & 53.46     & 14.47   & 12.54      & 49.91      & 13.47   & 9.92       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \midrule
% \multirow{7}{*}{C4}        & Omniquant & 15.03    & 11.85    & 7.21     & 7.12      & 11.29   & 6.69       & 6.56       & 10.75   & 6.06       \\
%                            & AWQ       & 15.04    & 11.87    & 7.21     & 7.13      & 11.28   & 6.70       & 6.56       & 10.75   & 6.05       \\
%                            & GPTQ      & 15.05    & 11.87    & 7.21     & 7.12      & 11.26   & 6.69       & 6.56       & 10.74   & 6.06       \\
%                            & RTN       & 15.71    & 12.31    & 7.37     & 7.24      & 11.51   & 6.69       & 6.58       & 10.94   & 6.06       \\
%                            & FIGNA     & 15.04    & 11.86    & 7.22     & 7.12      & 11.29   & 6.70       & 6.57       & 10.75   & 6.06       \\
%                            & VSQuant   & 19.00    & 13.13    & 8.89     & 10.36     & 12.64   & 7.85       & 8.35       & 11.91   & 6.85       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \bottomrule 
% \end{tabular}%
% }
% \end{table*}

==> 1-intro-v0.tex <==
% \rOneFC{Some writing references to learn from:}
% \begin{itemize}
%     \item \rOneFC{[MICRO'16] Stripes \cite{judd2016stripes}: the first work to leverage bit-serial computing in DNNs.}
%     \item \rOneFC{[HPCA'22] FAST \cite{zhang2022fast}: exploit DNN training with variable precision block floating point (BFP) numbers, and its BFP numbers are on-the-fly converted as well.}
%     \item \rOneFC{[HPCA'24] BitWave \cite{shi2024bitwave}: bit-serial computing with bit-column sparsity. Learn how to orchestra each part of the paper.}
%     \item \rOneFC{[HPCA'24] FIGNA \cite{jang2024figna}: the first work to focus on FP-INT GEMM optimizations with shared exponents. Our highly relevant baseline.}
%     \item \rOneFC{[JSSC'23] VS-Quant \cite{keller202395}: the two-level per-vector scaling quantization but requires retraining to recover accuracy. Our highly relevant baseline.}
% \end{itemize}

\section{Introduction} \label{sec:intro}

% \rOneFC{[Chao: I think the current intro is too lengthy. Maybe we need to discuss further how to build an attractive intro based on our claimed contributions.]}

% \rOneFC{[Goal: LLM's brief intro. Focus on challenges for LLM deployment.]}
The recent emergence of large language models (LLMs) has a profound impact on the world and is followed by a rapid, widespread adoption. Though highly in demand, their deployment is challenging due to their immense computational and storage demands. 
For example, GPT-3's 175 billion parameters require approximately 350GB of FP16 storage, surpassing the memory capacity of current commodity GPUs. For cloud environments, their deployment is facilitated by energy-hungry, purpose-built GPUs. In contrast, deployment on edge devices remains infeasible.

% \rOneFC{[Goal: Weight-only quantized LLMs have become a prevalent choice for deploying LLM models on edge devices.]}
Quantization serves as an effective technique to lower storage and computational demands by reducing the model's precision. Post-training Quantization (PTQ) stands out as a practical choice due to its lower training data dependency, shorter optimization time, and comparable model performance compared to Quantization-aware Training (QAT). Within PTQ, weight-only quantization has gained prominence in edge device deployment scenarios. 
% Unlike weight-activation quantization, which quantizes both weights and activations, weight-only quantization preserves activation data in FP16 precision, leading to reduced storage requirements.
In contrast to weight-activation quantization where both weights and activations are quantized, weight-only quantization maintains activations in FP16 precision and quantizes weights exclusively. 
This enables weight quantization to 4-bit integers while preserving model accuracy, achieving significant reductions in the model's storage cost. 
Consequently, weight-only quantization has become a prevalent choice for deploying LLM models on edge devices.

\rOneRG{[This should move to Motivation]}
% \rOneFC{[Goal: FP-INT operations are dominated in weight-only quantized LLMs, which requires further optimizations.]}
To further optimize the deployment of weight-only quantized LLMs, we first need to understand the distribution of their computational operations. We explored the proportion of FP-INT operations in text generation tasks for different context length ratios across a range of weight-quantized LLMs. As shown in the figure, when the generation length is 25\% of the maximum length, FP-INT operations account for an average of 97\%, and even when the generation length reaches 100\% of the maximum length, FP-INT operations still average over 90\%, demonstrating their significant dominance.
This implies that FP-INT operations account for the vast majority of the computational workload in text generation tasks, making them crucial for further deployment optimization. Therefore, we focus our optimization efforts on FP-INT operations.

% \rOneFC{[Goal: Activaitons in FP-INT GEMMs take the majority of energy consumption, including off-chip footprints, on-chip footprints, as well as computational costs. And therefore, it is essential to exploit optimizations towards activations for energy-efficient LLM inference.]}
In edge deployment scenarios, energy efficiency is paramount beyond storage constraints. While weight-only quantization reduces storage overhead, it fails to address the large energy cost of LLM inference. For edge devices, energy efficiency is a more stringent constraint than storage cost.
% with activations during FP-INT operations, which form the core computational workload in large models.
The activations remain in a high-precision format, incurring high energy consumption due to (1) frequent off-chip accesses due to limited on-chip space for storing entire next-layer FP16 activations, and (2) substantial on-chip memory access overhead compared to INT4 weights.


\rOneFC{[Goal: Summarize our work with focus on what techniques we leverage to solve what challenges mentioned above.]}
% The inference of large language models (LLMs) is bottlenecked by the computation and storage of floating-point (FP) activations, which incur significant energy overheads. 
To address the high energy cost associated with data movements of activations in weight-only quantization schemes, we conducted extensive experiments and made the following key observations:
\begin{enumerate}
    \item Nearby activations can be grouped to share the exponent part, which helps simplify the computation in the FP-INT units, while the appropriate group size has a negligible impact on model accuracy.
    \item There exists substantial redundancy in the mantissa part of FP activations, and different mantissa bitwidths trade off accuracy for different application scenarios, enabling flexible adjustment.
    \item Different modules in LLMs exhibit varying sensitivity of activation precision to model accuracy, necessitating a finer-grained exploration of the precision-bitwidth balance.
\end{enumerate}

Based on these findings, we propose Anda, a novel numerical format that enables energy-efficient and performance-scalable LLM inference. Anda dynamically shares exponents at runtime and automatically adjusts the variable-length mantissas based on user requirements. This design significantly reduces the data movement and computation overheads of the activations while supporting flexible precision tuning for different deployment scenarios, thereby achieving energy-efficient and performance-scalable LLM inference.
To efficiently process data in the Anda format, we further develop corresponding arithmetic units that leverage bit-serial operations to perform efficient FP-INT dot-product computations within shared-exponent groups. Additionally, to reduce the overhead of frequent memory accesses, we propose an on-the-fly compression engine to convert FP output activations to the Anda format. We also design an efficient online data orchestration scheme to improve the memory access efficiency of the Anda format.
Finally, we integrate the Anda format and aforementioned components into a single system and conduct comprehensive evaluations, demonstrating its superior performance in enabling energy-efficient and performance-scalable LLM inference.
% The contribution of this paper can be summarized as follows:
The major highlights of this work are as follows:
\begin{itemize}
    \item \textbf{Anda data format.} We propose a novel data format to reduce memory access overhead and computational complexity involved in FP activations, enabling online precision adjustment for better energy-performance-accuracy trade-offs. It achieves a xx\% reduction in memory access overhead and a xx\% reduction in required operations (OPS) within only 1\% negligible accuracy trade-off. (Sec.~\ref{sec:algo})
    % We propose a novel data representation format, Anda, specifically designed for optimizing activation data in FP-INT quantized LLMs. Anda format effectively reduces both storage and computation costs of activation data, leading to significant improvement in model energy efficiency.
    \item \textbf{Efficient arithmetic unit.} We design an efficient dot-product processing unit for activations in Anda format, achieving high area efficiency and energy efficiency with flexible precision adjustment. Compared to other equivalent units, it achieves a xx\% improvement in area efficiency and a xx\% improvement in energy efficiency at xx mantissa precision. (Sec.~\ref{subsec:dpu})
    \item \textbf{On-the-fly compression support.} We propose an on-the-fly compression engine to efficiently convert FP format to Anda format, significantly reducing off-chip and on-chip traffic and memory energy consumption. Moreover, we design a bit-plane data storage scheme for Anda format to improve storage utilization and reduce data movement costs. The compression efforts, with the cost of area overhead of xx\%, achieve xx\% reduction in memory access overhead, and xx\% energy saving compared to the original FP-INT format. (Sec.~\ref{subsec:comp} \& \ref{subsec:scheme})
    \item \textbf{System integration.} We build a computing system based on Anda format and conduct comprehensive experiments on nine popular LLMs. The results demonstrate that Anda format can significantly improve the area efficiency and energy efficiency of models with flexible energy-performance-accuracy trade-off. Specifically, with no loss in accuracy, Anda format achieves an average improvement of XX\% in area efficiency and XX\% in energy efficiency. When allowing a 1\% accuracy loss, the average improvements are XX\% in area efficiency and XX\% in energy efficiency. (Sec.~\ref{subsec:overall})


\end{itemize}

\textbf{=== Below is OUTLINE ===}
\begin{itemize}
    \item Why do we focus on weight-only quantized LLMs?
        \begin{itemize}
            \item Near-lossless model accuracy...
            \item Its unique benefits on memory consumption...
            % Also because of the benefit of ASIC compared to FPGA? We can more easily deal with the datatype conversions, so there is more to gain
            \item \rOneRG{We take weight-only quantization as a given}
        \end{itemize}
    \item What issues still exist in weight-only quantized LLMs?
        \begin{itemize}
            \item FP16 activations dominate energy consumption from two sides: memory access \& computation... (Here we need Robin \& Arne's help!) [Fig.~\ref{fig:zigzag}]
            \item FIGNA's \cite{jang2024figna} shortcomings in these two aspects: 1) memory access, FP16 in full precision storage plus repeated access consumes more energy... 2) computation, INT multiplier with high bitwidth preserving numerical accuracy consumes more energy... [Fig.~\ref{fig:2}]
        \end{itemize}
    \item What interesting findings do we have found?
        \begin{itemize}
            \item We don't need to maintain numerical accuracy due to the robustness of LLMs...Aggressive cutting mantissa bits within a shared exponent element group is feasible within 1\% negligible accuracy loss...
            \item Layer-wise sensitivity to mantissa bit cutting is near-uniform, while module-wise sensitivity is quite different, motivating us to explore flexible activation precision across modules...
        \end{itemize}
    \item How to resolve the above challenges based on our findings?
        \begin{itemize}
            \item From algorithm aspects, we propose a heuristic post-training algorithm to determine the bitwidth of each module of LLMs... (computation \& memory access)
            \item From architecture aspects, we design an energy-efficient accelerator with several features: 
                \begin{enumerate}
                    \item activation-bit-serial with shared exponent group PEs to enable flexible mantissa bit precision... (computation)
                    \item online bit-plane compression engine to reduce the memory access consumption... (memory access)
                    \item bit-plane data orchestration scheme to enable efficient storage utilization and transfer cost... (computation \& memory access)
                \end{enumerate}
        \end{itemize}
\end{itemize}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{(a) Concept of these two issues; (b) Concept of our findings; (c) Our Anda solution.}
%     \label{fig:2}
% \end{figure}

==> 1-intro-v1.tex <==
\section{Introduction} \label{sec:intro}

Large language models (LLMs) \cite{chowdhery2023palm, zhang2022opt, touvron2023llama, team2024gemma} have demonstrated remarkable proficiency in a wide array of natural language processing tasks, including text generation, question answering, and automatic summarization. %, \ms{and so on}. 
The extraordinary success of LLMs can be attributed to the scaling law \cite{bahri2024explaining}, which posits that performance improves dramatically with %increases in 
\ms{the ever-increased} model size, training data volume, and computational resources. 
%\ms{For instance,} t
\mv{T}he evolution of the GPT series \cite{achiam2023gpt, kalyan2023survey, bhattacharya2024demystifying} on model size strikingly illustrates this principle: while GPT-1 comprised a modest 117 million parameters in 2018, its successor GPT-4 is speculated to encompass over a trillion parameters \ms{along with considerable enhanced language understanding and generation capabilities}. 
% This exponential growth in scale has substantially enhanced the capacity of LLMs to tackle intricate and multifaceted tasks, pushing the boundaries of artificial intelligence in language understanding and generation.
%\ms{I cut the following sentence. feel it is redundant with the previous one.}
%As groundbreaking applications like OpenAI's ChatGPT~\cite{openai2024chatgpt} and Microsoft's Copilot~\cite{microsoft2024copilot} gain widespread popularity, LLM inference has emerged as a significant workload across various computing platforms \cite{hu2024characterization, yu2022orca, dhar2024empirical, yin2024llm}, from cloud infrastructures to edge devices. 
However, the exponential growth in LLM model sizes has created substantial deployment challenges, imposing enormous demands on storage and computational resources. 
% This escalating resource requirement underscores the critical need for efficient model compression techniques, particularly quantization, to optimize LLM performance and facilitate wider deployment.

Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} is one of the most popular techniques to %tackle resource issues.
\ms{reduce memory footprints and computation costs.}
%\ms{[I feel you don't need to talk about two different quantization methods. Focus on weight-only quantization as the most common quantization.]}
%Two primary quantization strategies are commonly employed \ms{for LLMs}: weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} and weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}. Weight-activation quantization quantizes both weight and activation parameters, while weight-only quantization focuses solely on weight parameters. 
\ms{To maximally shrink the model size, the most common quantization strategy \mv{for LLMs today} involves aggressively lowering the precision of the weights while typically maintaining high precision for activations due to the presence of outliers~\cite{dettmers2022gpt3, wei2022outlier}, a technique known as weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, zhao2024atom, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit}.} %Notably, weight-only quantization, particularly 
\ms{For example, the W4A16 scheme \cite{shao2024omniquant}, where weights are represented using 4-bit fixed-point integers (INT4) and activations are represented using 16-bit floating-point numbers (FP16), has gained substantial traction in LLM \mv{because of its significant impact on} %. This approach is effective because INT4 weights significantly reduce storage requirements during deployment \cite{yuan2024llm}, as weight parameters typically dominate 
the model's memory footprint during deployment \cite{yuan2024llm}.}
%However, the energy bottleneck shifts toward activation movements when weights are aggressively quantized, which raises the demand for the optimization of the FP16 activation. [Can we have a figure to show this shifting??]
%the W4A16 scheme \cite{shao2024omniquant}, where weights are represented using 4-bit fixed-point integers (INT4) and activations are represented using 16-bit floating-point numbers (FP16), has gained significant traction in LLM serving due to several compelling advantages: 1) Weight parameters typically account for the majority of a model's storage footprint. Weight-only quantization allows for aggressive quantization of weights to lower bitwidths, effectively alleviating storage constraints during deployment \cite{yuan2024llm}. 2) Activation values exhibit a wider dynamic range compared to weights, making them more challenging to quantize effectively. By retaining activations in FP16 format, weight-only quantization preserves the expressive power of activations while minimizing storage requirements \cite{lin2024awq}. 3) Limiting quantization to weights while keeping activations in FP16, eliminates frequent and complicated quantization-dequantization overhead and boosts inference speed compared to weight-activation quantization~\cite{lin2024qserve}.

% As weight-only quantization becomes increasingly important, NVIDIA introduced a new FP-INT GEMM kernel in CUDA’s CUTLASS and other researchers proposed specialized GPU kernels for this purpose. However, these kernels still rely on existing FP units for FP-INT GEMM computations, which involves dequantizing INT weights to FP values and incurs additional computational overhead. While this approach effectively reduces storage requirements and memory bandwidth, it does not fully address the increased computation costs. To further alleviate these costs, there have been explorations into transforming FP units into dedicated FP-INT arithmetic cores. Despite these efforts, the benefits are limited due to the inherent complexities of floating-point operations, such as exponent alignment and normalization. To simplify FP-INT operations in weight-only quantization, the FIGNA framework proposes a novel approach. FIGNA maintains activation values in FP16 format and employs a pre-alignment method to convert traditional FP operations into INT operations, significantly enhancing computational efficiency while preserving numerical precision comparable to FP arithmetic.

% As weight-only quantization becomes increasingly crucial, NVIDIA has introduced a new FP-INT GEMM kernel in CUDA’s CUTLASS, and other researchers have proposed specialized GPU kernels for this purpose. 
% While these kernels reduce memory footprint and bandwidth usage, they rely on existing FP units for FP-INT GEMM, which introduces additional computational overhead due to the need for dequantizing INT weights to FP values. 
% To further reduce computational costs, there has been exploration into converting FP units into dedicated FP-INT arithmetic units. 
% However, the complexity of operations like exponent alignment and normalization limits the potential gains. 
% To simplify FP-INT operations in weight-only quantization, the FIGNA framework proposes a novel approach. 
% FIGNA maintains activation values in FP16 format and employs a pre-alignment method to convert traditional FP operations into INT operations, achieving significant computational efficiency while maintaining precision. 
% Nevertheless, FIGNA’s approach does not optimize activation storage, leading to increased energy consumption due to redundant activation data access compared to weight data.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/ops_breakdown.pdf}
    \caption{FP-INT operations are dominated in weight-only quantized LLMs.}
    \label{fig:fp_int}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     % \subfigure[]{%
%     % }\hfill
%     % \subfigure[]{%
%     \includegraphics[width=0.46\columnwidth]{figs/memory_consumption.png}
%     \includegraphics[width=0.46\columnwidth]{figs/energy_weight_act.png}
%     \caption{Energy distribution of various LLM models on a typical cloud accelerator.}
%     \label{fig:zigzag}
% \end{figure}

% \ms{[feel the following para is not well connected with the previous para...should we say that the bottleneck of LLMs switches from memory-bound to computation-bound with the weight-only quantization, then say the optimization on the computation is necessary? or the energy bottleneck shifts to activation data movements? Anyway, we should mention the optimization target is activation and the reason before introduce our work.]} \mv{[I gave it a try]\\}
With the rising importance of weight-only quantization, \mv{initiates an interesting shift in the LLM inference bottlenecks. The burden now shifts to the activation data movements, and new optimized operators for FP-INT operations become indispensable.} 
Fig.~\ref{fig:fp_int} illustrates the relative distribution of operations for various W4A16 LLMs across different token lengths in text generation tasks. 
Notably, FP-INT operations consistently dominate, accounting for over 90\% of the total computational workload across all models and scenarios examined. 
This overwhelming prevalence underscores the critical importance of optimizing FP-INT GEMM operations to achieve efficient inference deployment for W4A16 LLMs. 

NVIDIA’s new FP-INT GEMM kernel \cite{nvidia2024cutlass}, \mv{as well} specialized GPU kernels \mv{optimizing activation memory bandwidth} \cite{jeon2020biqgemm, xia2024fp6, frantar2023optq} \mv{are a consequence of this evolution}. %have been introduced to manage memory and bandwidth more effectively. 
\mv{However, these optimized GPU kernels all} %While these kernels are beneficial for reducing storage, they 
still rely on FP units \mv{by} converting the INT weights to FP values for \mv{execution in FP} GeMM \mv{operatiors} \cite{lin2024qserve}. %, which adds computational overhead from converting INT weights to FP values. 
% \mv{In literature,} there have been efforts to develop dedicated FP-INT arithmetic units, \mv{in which the challenge lies in reducing the overhead stemming from the} exponent alignment and normalization. % limits performance improvements.
\rOneFC{In the literature \cite{jang2024figna}, efforts have been made to develop dedicated FP-INT arithmetic units, with the challenge lying in reducing the hardware overhead stemming from exponent alignment and normalization.}
\rOneFC{In addition to developing dedicated FP-INT computing units, another optimization approach is %to attempt 
to convert FP activations to a block floating point (BFP) data format for computation.}
\rOneFC{Since in BFP \mv{adjacent elements} share and exponent, the overhead of exponent alignment and normalization \mv{within a group disappears}, simplifying the operation to fixed-point arithmetic. 
However, directly applying previously proposed BFP formats \mv{to a pre-trained network} significantly impacts model accuracy. \mv{As a result, this is only possible in combination with} costly retraining \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock}, or \mv{with the usage of} a large mantissa field to preserve precision during conversion, resulting in substantial memory access and computational overhead \cite{jang2024figna, kim2023winning}.}
% FIGNA~\cite{jang2024figna} %represents a step forward by using FP16 for storage and 
% \mv{exploits} a grouped pre-alignment method to streamline computations with preserved numerical accuracy. % to FP arithmetic, 
% Yet, it falls short in optimizing \mv{the storage and energy footprint of the} activation data, \mv{which is still represented as FP16}. % , leading to increased energy consumption from inefficient activation data access. 
% \mv{[Can we discuss one more, besides FIGNA?]]}

% In this paper, we propose Anda, a novel data format as a drop-in replacement of FP16 activation for performance-scalable efficient LLM inference.

%Building upon these prior works and addressing their limitations 
\mv{The overcome these limitations of the SotA}, we propose Anda, a novel activation-oriented data format designed to directly replace FP16 without incurring any retraining overhead, which is \mv{important for LLMs due to their enormous} %impractical in LLM era due to the drastic 
training cost. 
\ms{Compared to the traditional FP16 data format, the Anda data type} \ms{reduces both} storage requirements  and computational costs, \mv{due to its shared exponent and adjustable mantissa bit-width. Moreover, Anda} allows a flexible trade-off between model accuracy and performance.
%Anda significantly reduces both storage requirements and computational costs associated with activation data and enables a flexible trade-off between model accuracy and performance through precision adjustments. 
% \mv{[I am not sure whether you should keep the following two sentences here. In my view, people can not understand them at this stage of the paper yet, and it is also not something that we deeply explpore in the paper. Not the core idea. I would first explain the rest, and add this rather a bit later.]}
% \mv{[[[} This feature holds substantial promise for LLM \mv{deployment}, particularly in scenarios with strict \mv{latency} constraints where applications may prioritize timely responses over maximum accuracy. 
% By offering this adaptability, Anda addresses a critical need in real-world LLM deployments, where the balance between accuracy and speed can be dynamically optimized based on specific use-case requirements. \mv{]]]}
% \mv{Towards this goal}, we \mv{in this paper} first identify the energy bottleneck associated with activations in LLM inference. Our analysis reveals that activations become the primary energy consumption in compute-bound LLM inference scenarios, particularly for quantized W4A16 LLMs. 
% This is due to their higher bit width and more frequent memory accesses compared to weights. 
% Consequently, approaches like FIGNA \cite{jang2024figna, kim2023winning}, which only transform data during computation while maintaining FP16 format for storage, show limited potential for energy optimization. 
% This observation motivates our exploration of a more efficient data representation for activations, aimed at simultaneously optimizing storage, memory access, and computational costs. 
% By addressing these multiple aspects, we seek to achieve comprehensive efficiency improvements in LLM inference, particularly in energy-constrained environments.
% While FIGNA demonstrated the feasibility of dynamically sharing exponent segments among adjacent activation elements at runtime to simplify mantissa computations, they expanded the aligned mantissa width to maintain numerical precision equivalent to the original FP format. However, our research reveals that as LLM sizes increase, they exhibit a higher tolerance for numerical precision errors in the mantissa. This finding suggests that after sharing exponent segments, the aligned mantissa width not only doesn't require expansion but can actually undergo aggressive reduction. This reduction is particularly promising, offering the potential to significantly decrease both storage and computational costs while maintaining LLM accuracy. Furthermore, our exploration uncovers that in W4A16 LLMs, different key modules exhibit varying sensitivities to mantissa reduction. Consequently, adopting different mantissa widths for different modules under the same model accuracy constraints can lead to even greater reductions in computational and storage overheads. 
% This modular approach to precision optimization represents a novel strategy for enhancing LLM efficiency without compromising performance.
% Based on these findings, we propose the Anda data format to accommodate the varying sensitivity of mantissa width across different modules and models in LLM FP activations. Anda dynamically shares exponent segments between adjacent elements at runtime while featuring a variable-width mantissa. 
This adaptive, \mv{varibale-mantissa}-length format adjusts according to model \mv{sensitivities}, yet remains transparent to users during execution, serving as a direct replacement for FP16 activation. 
\mv{In this work, we assess optimize and demonstrate the benefits of the Anda data type in a complete system setting.}
% \\
% \\
% \mv{[(If out of space) I WOULD CUT EVERYTHING FROM HERE...]\\}
% To identify optimal mantissa widths for different LLM modules we develop a rapid search algorithm \ms{within tolerated accuracy constraints}. Through \ms{a} minimal iterative \ms{mantissa bit length} relaxation, this algorithm efficiently finds feasible solutions %on calibration datasets
% that minimize both accuracy error and operand count. %This approach effectively reduces model storage, memory access, and computational costs while maintaining model accuracy.
% To fully harness Anda's potential in LLM inference, we construct a comprehensive computing system with the following key features: 
% 1) An activation data layout scheme for the variable-length Anda format, significantly reducing storage overhead while enabling efficient data access, thus achieving substantial savings in memory access energy. 
% 2) A flexible and efficient mantissa dot-product computation unit designed using a bit-serial approach, adapting to efficient computation of various fixed-length Anda data and enhancing computational efficiency for Anda format data.
% 3) A runtime bit-plane compressor that compresses output activations into Anda format before writing back to memory, dramatically reducing activation storage and memory access overheads.
% This integrated system leverages the Anda format to optimize LLM inference across multiple dimensions, addressing the challenges of storage, computation, and energy efficiency in large-scale model deployment.
% Extensive evaluation on Anda format shows \TODO{}... 
% \mv{[(If out of space) ... UNTIL HERE]\\}
\mv{Therefore,} %In summary, 
this paper makes the following contributions:
\begin{itemize}
    \item We \mv{formalize} Anda, a variable-length data format with dynamically shared exponents and adjustable mantissa widths for activations, directly replacing FP16 activations and adapting to precision requirements across different LLM modules.
    \item We develop an efficient algorithm to identify optimal mantissa widths for various LLM modules within given accuracy tolerances, balancing model accuracy and efficiency.
    \item We design \mv{an Anda-compatible} accelerator \mv{down to the RTL level,} featuring 1.) an \mv{Anda-}optimized \mv{memory layout}, %data layout, 
2.) flexible \mv{widely-parallel} dot-product computation units, and a 3.) a runtime \mv{data} compressor \mv{in the memory interface}, significantly enhancing storage, memory access, and compute efficiency. % for the Anda format
    \item Extensive evaluation \mv{of the system-level energy and throughput savings from the} Anda format \mv{across various LLMs} shows ... 

\end{itemize}

\mv{The paper is organized as follows: Sec.~\ref{sec:bkg} reviews the benefits and remaining bottlenecks of weight-only quantization methods, and quantifies the sensitivity of LLM accuracy to the shared exponents and reduced mantissa lengths. Based on these findings, Sec.~\ref{sec:algo} formalizes the proposed Anda data format as well as the algorithm to find the most optimal mantissa lengths for an LLM. Next, an Anda-optimized hardware architecture is proposed in Sec.~\ref{sec:arch}, which allows to derive system-level efficiency gains in Sec.~\ref{sec:eval} and benchmark it against the SotA. Sec.~\ref{sec:concls} concludes the paper.}

==> 2-bkg-v0.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figs/LLM_blocks.png}
    \caption{Illustration of the architecture for a weight-only quantized LLM model.}
    % The blue boxes represent modules with quantized weights, while the green boxes denote modules that perform only floating-point operations. \mv{[and what is orange? I would add the meaning of the colors in the graph as a legend, rather than in the caption?]}}
    \label{fig:llm_blocks}
\end{figure}

\section{Background and Motivation}\label{sec:bkg}

% \begin{itemize}
%     \item Introduction of Transformer layers
%         \begin{itemize}
%             \item Transformer layers itself
%             \item Prefill stage: GEMM; Decode stage: GEMV + KV cache [Fig.~\ref{fig:3}]
%         \end{itemize}
%     \item Related works \rOneFC{[Chao: Maybe we need to move it to the last section? like QServe \cite{lin2024qserve}]} \rOneRG{I think this fits nicely here. We should definitely explain FIGNA.}
%         \begin{itemize}
%             \item Quantization of LLMs: Weight-only quantization, weight-activation quantization, KV cache quantization.
%             \item LLM-related accelerators
%         \end{itemize}
% \end{itemize}

\subsection{Weight-only Quantized LLMs}

% Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} in large language models (LLMs) is a crucial technique that reduces model size and computational complexity while maintaining performance, typically by converting FP16 numbers to lower-precision integers. Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}, which applies quantization solely to model weights while keeping activations in full precision, has gained popularity in the era of large models due to its simplicity, lower precision loss, and better hardware compatibility compared to weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3}. 

% Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} in large language models (LLMs) is a crucial technique that reduces model size and computational complexity while maintaining performance, typically by converting 16-bit floating-point numbers to lower-precision integers. 
% The massive number of LLM parameters poses significant challenges to deploying LLM on resource-constrained devices. Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}, compared to weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3}, substantially reduces memory overhead, thereby alleviating deployment platform costs while maintaining high model accuracy. 
% Its ease of adaptation to existing GPU platforms has led to widespread application and attention. 

% Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq} has become a widely adopted technique in large language models (LLMs), surpassing weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} in popularity.
Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq} has become a widely adopted technique in deploying LLMs. 
Unlike weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} which reduces precision for both model weights and activations, weight-only quantization focuses solely on compressing model parameters with a much more aggressive quantization scheme, which significantly reduces memory consumption, enabling the efficient deployment of LLMs on resource-constrained devices while maintaining high model accuracy. Consequently, weight-only quantization has become crucial in addressing the challenges posed by the massive number of LLM parameters.

% Fig.~\ref{fig:llm_blocks} illustrates the model architecture of a weight-only quantized LLM. 
% LLMs are composed of a series of Transformer blocks, each containing attention and feed-forward layers.
% The blue boxes in Fig.~\ref{fig:llm_blocks} represent the quantized weight matrices: query (Q), key (K), value (V), and output (O) in the attention Layer, and up-projection and down-projection matrices in the feed-forward layer. 
% These weight matrices dominate the storage requirements during LLM inference. 
% In a W4A16 quantized LLM, these weight matrices are quantized from FP16 to INT4, significantly reducing storage overhead, while the rest of the model computation remains in FP16. 
% As shown in Fig.~\ref{fig:llm_blocks}, the FP16 activations related to these weight computations are qkv\_proj, out\_proj, fc1, and fc2. Specifically, qkv\_proj computes with Q, K, and V weight matrices, out\_proj with the O weight matrix, and fc1 and fc2 with the up-projection and down-projection weight matrices, respectively. 
% This approach effectively balances model efficiency and performance, making weight-only quantized LLMs particularly suitable for deploying large language models in resource-constrained environments.

Fig.~\ref{fig:llm_blocks} illustrates the model architecture of a weight-only quantized LLM that is built from a series of Transformer blocks, each consisting of attention and feed-forward layers.
The blue boxes in Fig.~\ref{fig:llm_blocks} represent the quantized weight matrices: query (Q), key (K), value (V), and output (O) in the attention Layer, and up-projection and down-projection matrices in the feed-forward layer. 
For example, in the widely used W4A16 quantization scheme, these weight matrices are quantized from FP16 to INT4, which significantly reduces the storage overhead, while the remaining computations in the model are still performed in FP16.
In W4A16 quantized LLMs, FP-INT operations become the predominant computations during LLM inference. Specifically, the FP16 activations shown in the figure include qkv\_proj, out\_proj, fc1, and fc2, which are involved in computations with the quantized Q, K, V, and O weight matrices, as well as the up-projection and down-projection weight matrices, respectively.
Despite the significant storage efficiency gains achieved through INT4 weight quantization, the FP16 activations still contribute to a notable performance bottleneck in the FP-INT computations~\cite{huang2024isca}. \mv{Can I see this somewhere? If not, add a citation to prove this...}.

\subsection{Block Floating Point}

Reducing the computational overhead of FP16 activations is crucial for optimizing the efficiency of LLMs, and BFP~\cite{drumond2018training} strikes a balance between traditional floating-point and integer formats. 
By assigning a shared exponent to a group of values, BFP maintains dynamic range while simplifying computations, and as such achieves higher compression ratios than integer formats. % while \mv{avoiding significant accuracy losses}. %ensuring computational efficiency. 
However, like other quantization techniques, BFP may \mv{still} affect neural network accuracy. 
To address this, researchers have proposed two main approaches: \mv{On the one hand,} BFP-aware training \mv{fine tunes the network after quantization} \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock}, \mv{at the expense of a} %which faces challenges of model-specific optimization and 
costly training process, making it \mv{rather} impractical for LLMs. \mv{On the other hand,} direct conversion of pre-trained floating-point models to BFP formats~\cite{dai2021vs, keller202395, jang2024figna, kim2023winning}, significantly reduces deployment costs, \mv{but requires long mantissa lengths to avoid serious degradations in} model performance, as \mv{e.g. observed in the} VS-Quant \mv{scheme}~\cite{dai2021vs, keller202395}). 
\mv{To avoid the storage of these long mantissa lengths}, methods like FIGNA~\cite{jang2024figna, kim2023winning} propose dynamic conversion to BFP during computation. \mv{This allows them to store the activation data in memory in the traditional FP16 data format, while expanding to long mantissa lengths and shared exponents right before computations. As such, FIGNA} preserves numerical precision comparable to floating-point calculations and maintains model performance. \mv{However, this also prevents FIGNA to obtain activation memory footprint savings, or significant computational savings.} %but sacrifices some potential computational gains. 

%In the era of LLMs, the cost of retraining before deployment is prohibitively high; therefore, 
\mv{To avoid both costly retraining, as well as large activation footprints,} we seek a solution that can rapidly convert FP activations to BFP activations \mv{without retraining}, while also leveraging the computational and storage advantages of BFP \mv{for LLM inference}. % to achieve efficient LLM inference deployment.
To achieve this goal, it is necessary to explore opportunities for \mv{reduced mantissa length BFP under the} %simplifying FP16 activation computations by leveraging the 
unique characteristics of LLMs.


% \subsection{Challenges towards Activations in W4A16 quantized LLMs}

% % Due to significant reduced storage requirements, W4A16 quantized LLMs have been widely deployed on GPU devices. 
% % Within LLMs, both linear layers and attention mechanisms rely on general matrix multiplication (GEMM) operations, with the key distinction being the operands involved. 
% % Linear layers perform GEMM between weights and activations, while attention mechanisms compute GEMM between different activation matrices. 
% % Fig.~\ref{fig:fp_int} illustrates the relative distribution of operations for various W4A16 LLMs across different token lengths in text generation tasks. 
% % Notably, FP-INT operations consistently dominate, accounting for over 90\% of the total computational workload across all models and scenarios examined. 
% % This overwhelming prevalence underscores the critical importance of optimizing FP-INT GEMM operations to achieve efficient inference deployment for W4A16 LLMs. 
% % Consequently, our optimization efforts are primarily focused on enhancing the performance of these FP-INT GEMM operations, as they represent the most significant bottleneck in the inference process.

% % \begin{figure}[htbp]
% %     \centering
% %     % \subfigure[]{%
% %     \includegraphics[width=0.92\columnwidth]{figs/energy_weight_act.png}
% %     % }\hfill
% %     % \subfigure[]{%
% %     %     \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
% %     %     \label{fig:subfig2}
% %     % }\vskip\baselineskip
% %     % \caption{Energy distribution in Llama2-7B model on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations. \rOneFC{[Chao: Robin, I think here we show llama-7b is enough, since our experiment will not cover gpt-175b. Maybe we can also remove the attention parts, i.e., Q*K$^{T}$ and S*V because we focus on FP-INT operations. Or we can split the Linear operations into qkv\_proj, out\_proj, and denote MLP as fc, like Fig.~\ref{fig:value_dist_wrt_addi_bits}, and merge Q*K$^{T}$ and S*V into the others to show the dominated energy consumption of FP-INT operations.]}}
% %     \caption{Energy distribution of various LLM models on a typical cloud accelerator.}
% %     \label{fig:zigzag}
% % \end{figure}

% % \begin{figure}[htbp]
% %     \centering
% %     \includegraphics[width=0.92\columnwidth]{figs/memory_consumption.png}
% %     \caption{Relative memory consumption.}
% %     \label{fig:mem_consumption}
% % \end{figure}

% For linear layers with INT4-quantized weights (Q, K, V, O, up projection, down projection), current GPUs lack specialized computational units, necessitating a process where INT4 weights are loaded into GPU memory and converted to FP16 before computation with FP16 activations. This approach incurs additional computational overhead. To enhance FP-INT operations, FINGA initially explored dedicated floating-point units for FP-INT computations. However, while this effectively reduced multiplier complexity, the alignment and normalization operations in floating-point units still consumed significant area and power, resulting in only 22\% and 26\% savings for FP16-INT4 specialized hardware units, respectively.

% To further reduce computational costs, FINGA leverages block floating-point (BFP) format, converting complex floating-point multiplications to INT multiplications. However, to maintain numerical precision, FINGA still uses FP16 format for storage, decompressing to INT format before computation, and expanding the mantissa. This approach, while beneficial, somewhat impacts computational efficiency.
% Moreover, in W4A16 LLM inference, although weight storage costs are significantly reduced, activation storage remains substantial. Crucially, in terms of inference energy consumption, we found that accessing activation data in LLM inference is more costly than accessing unit weights, and activations are frequently read during computations. Consequently, memory access for activation data accounts for a significant, non-negligible portion of energy consumption.
% This insight reveals that optimizing FP-INT GEMM by solely reducing FP-INT computational costs at the computation level is insufficient. A more comprehensive approach, considering both memory access and computation aspects simultaneously, is necessary to achieve more substantial benefits. This realization guides our strategy towards a holistic optimization of W4A16 LLM inference, addressing both computational efficiency and memory access patterns to maximize performance gains and energy efficiency.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/shared_exp_eval_fp_int_merged.pdf}
    \caption{Group Size (\mv{GS}) Impact. \mv{[I would find it better to on all plots use the actual mantissa bits on the x-axis and not the number of cut bits. this is too relative and not insightful. I can cut 20bits if I start from FP32...]}}
    \label{fig:acc_wrt_gs}
\end{figure}

\subsection{Opportunities towards Activation Optimizations}

%FIGNA's approach to introducing BFP computations in W4A16 LLMs involves expanding the mantissa to maintain precision, which introduces additional computational overhead. 
%Questioning the necessity of this expansion, we explore reducing mantissa length in BFP formats across different group sizes. 
%This intuition stems from neural network computation redundancy and model robustness to minor precision changes. 

\mv{To explore the sensitivity of LLMs to reduced mantissa lengths in BFP formats across different group sizes \mv{[Where do I see the impact across group sizes? Figure 3 does not seem to be referenced? ?]},} we first replace all activations of the different FP-INT GEMM operations, being the qkv\_proj, o\_proj, fc1, and fc2 \mv{(see Fig.2)} with the BFP format \mv{with a parametrized group size and mantissa length}, and observe the model's perplexity (PPL) \mv{to assess the accuracy impact}.

\mv{\textbf{Sensitivity to group size:} Fig.~\ref{fig:acc_wrt_gs} shows the sensitivity to the shared exponent group size for two different LLM models across a wide range of mantissa lengths. The experiment shows a clear trade-off between the group size, and the minimally required mantissa length.} Larger activation group sizes allow more efficient \mv{parallel} computations, yet at a greater precision cost \mv{or increased mantissa lengths}. Based on the observations, we chose a group size of 64 for subsequent exploration, as it provides a good balance between computational efficiency, hardware compatibility, and precision loss.
%This trade-off between computational efficiency and model accuracy provides crucial insights for optimizing LLM deployment strategies.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/acc_wrt_mbits_gs64.pdf}
    % \caption{The relative accuracy when uniformly cutting mantissa bits on 9 popular LLMs.}
    \caption{The relative accuracy to mantissa reduction across various LLMs. \mv{[Always put figures at paper top of bottom, rather than not in the text.]}}
    \label{fig:acc_wrt_mbits}
\end{figure}

\mv{\textbf{Sensitivity to LLM variant:} With this group size of 64, we continue our exploration across a wider range of recent LLMs, to derive their sensitivity to reduced mantissa lengths.} %Fig.~\ref{fig:acc_wrt_mbits} shows, LLMs maintained good PPL, sufficient for normal deployment even without mantissa expansion and with some reduction. 
%After determining the BFP group size, we conducted experiments on reducing mantissa lengths across several popular LLM models. 
As shown in Fig.~\ref{fig:acc_wrt_mbits}, different LLms exhibit varying sensitivities to mantissa reduction. %we explored the impact of mantissa reduction on model accuracy across different models. 
Assuming a 1\% accuracy loss tolerance in practical deployment scenarios, we observed that models \mv{such as} opt-6.7b, opt-13b, and opt-30b were less sensitive to mantissa reduction, allowing for the direct removal of 5 mantissa bits, while other models could only tolerate the removal of 4 mantissa bits. Furthermore, as more mantissa bits were removed, we observed more pronounced differences in accuracy sensitivity among different models. This insight inspires us to consider \mv{a variable length BFP datatype,} %model-specific optimization strategies for BFP conversion, 
potentially allowing for more aggressive compression in less sensitive models while maintaining a more conservative approach for others. \mv{This moreover raised the question whether there is also a difference in sensitivities among different tensors within one LLM.} %It also suggests the possibility of developing adaptive BFP schemes that adjust mantissa lengths based on each model's specific characteristics and requirements, thereby maximizing both efficiency and accuracy in LLM deployment. 
\mv{[I have cut quite some sentences in previous paragraph, and you still had quite some redudant messages...]}

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figs/module_wise_acc_gs64.pdf}
    \caption{The relative accuracy of OPT-6.7B, LLaMA-7B, and LLaMA-2-7B when cutting mantissa bits on qkv\_proj, o\_proj, fc1, and fc2 modules only.}
    \label{fig:module_wise_acc}
\end{figure}

\textbf{Sensitivity to tensor type:} We \mv{finally} explore the impact of different mantissa lengths \mv{across various tensors within the same model. This information allows to derive whether it makes sense to use different mantissa lengths across the activation outputs of the} qkv\_proj, out\_proj, fc1, and fc2 \mv{modules of a network}. %As shown in Fig. 1, these activations participate in computations with different INT4 quantized weight network layers. Converting these activations to BFP computations leads to accumulated numerical errors, ultimately affecting model accuracy. 
We \mv{therefore} examine opt-6.7b, llama-7b, and llama-2-7b models, \mv{individually sweeping} the mantissa \mv{length of each type of} activations to observe their \mv{individual sensitivity to} model accuracy. \mv{[Make it clear what length you use for the other tensors while you sweep one of them...]]}
Fig.~\ref{fig:module_wise_acc} \mv{summarizes the results, revealing} that activations from different modules \mv{indeed} have varying impacts on model accuracy across all three models. qkv\_proj consistently shows the most significant influence, while fc2 demonstrates low sensitivity in opt-6.7b but has a more pronounced effect in the llama series models.


% Our three sets of experiments reveal crucial insights into BFP application in LLMs. First, we find that LLMs can maintain good performance with reduced mantissa lengths, challenging the need for full-precision computations. Second, different LLM models show varying sensitivities to mantissa reduction, suggesting the potential for model-specific optimizations. Third, within a single model, different modules exhibit distinct sensitivities to precision reduction. These findings highlight limitations in traditional BFP designs, which use fixed mantissa lengths across all modules and models. In response, we propose a novel BFP design that employs variable-length mantissas tailored to the specific characteristics of each model and module. This approach allows for more efficient utilization of computational resources and storage, potentially leading to improved inference speed and reduced memory footprint without significant accuracy loss. Furthermore, this adaptive BFP strategy enables fine-grained optimization of LLM deployments, balancing performance and efficiency in a more nuanced manner than traditional fixed-precision approaches. By leveraging these model-specific and module-specific insights, our proposed BFP design paves the way for more efficient and adaptable LLM inference deployments across a wide range of applications and hardware configurations.

Our experiments reveal key insights into BFP application in LLMs: 1) LLMs maintain good performance with reduced mantissa lengths. 2) Different LLM models have varying sensitivities to mantissa reduction. 3) Within an LLM, different modules show distinct sensitivities to precision reduction.
These observations inspire us to \mv{introduce the new Anda data format, together with an methodology for post-training quantization, and rapid selection of the tolerable reduced mantissa lengths for any LLM. These will be introduced in the next section.} %pre-measure the sensitivity of different module activations to model accuracy. This insight enables efficient allocation of mantissa widths across modules during deployment, optimizing storage and computation while maintaining model performance.

%Traditional BFP designs, using fixed mantissa lengths, have limitations. We propose Anda BFP, employing variable-length mantissas tailored to each model and module. This approach improves efficiency, potentially increasing inference speed and reducing memory usage without significant accuracy loss. Anda BFP enables fine-grained optimization of LLM deployments, balancing performance and efficiency better than fixed-precision approaches.



==> 2.1-motivation.tex <==
\section{Motivation}\label{sec:motiv}

\rOneRG{[Goal: 1) show that in weight-only quantization, the activations take the majority of the energy. 2) weigt*act $>>$ act*act 3) mention we do only prefill + give arguments   ]}

Weight-only quantization alleviates the enormous storage requirements for contemporary LLMs, but it does not address the requirement of high energy-efficiency posed by edge computation environments. In order to gain insight into the energy bottlenecks, we simulate the performance of two well-known LLMs on a generalized but representative hardware architecture, for cloud and edge scenarios. By using a generalized architecture, the results conclusions with regards to energy bottlenecks are widely applicable. 

% HW info
The architecture is shown in Figure \ref{fig:generic-arch}. The cloud and edge accelerator have the same layout, but different dimensions and parameters. For the cloud scenario, the architecture is identical to the one used by \rOneRG{FLAT paper} for similar modelling purposes. To prevent becoming lost in the details, we generalize the energy cost of hardware transactions to a representative order of magnitude, given in Table \ref{tab:energy-cost}. \rOneRG{The values are justified by ...}

% Model info
The models chosen for simulation are Llama1-7B and GPT3-175B. We use a realistic batch size of 8 and only simulate the pre-fill phase, since this phase is the most energy intensive \rOneRG{[Is this the case?]}. The sequence length is set to half of the maximal context window. The tool used for simulation is ZigZag \rOneRG{[Cite, more info]}. The layers are mapped in an output-stationary way onto the architecture.

The simulation results are shown in Figrue \ref{fig:zigzag}. The figure show the total energy cost of a single inference of the LLM for the five major modules. Other modules such the non-linear operations or (de-)tokenization are omitted for simplicity. The energy costs are further categorized according to the type (compute or memory access at different levels) and the operand. The two main conclusions are that 1) the modules that embody weight $\times$ activation operations (and benefit from weight-only quantization) are dominant in terms of energy and 2) the data movement of the high-precision activations is the main contributor to the overall energy cost. \rOneRG{[This is not the case for the edge platform!]} Therefore, optimizing and compressing FP activations is necessary for achieving high-energy-efficient LLM inference deployment on edge devices.


% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{Hardware diagram of the target platform to model LLM inference.}
%     \label{fig:generic-arch}
% \end{figure}

% \begin{table}[h!]
%     \centering
%     \caption{Energy costs assumed in generic hardware architecture}
%     \begin{tabular}{lcc}
%         \toprule
%         \textbf{Energy cost per bit [pJ/bit]} & \textbf{Cloud scenario} & \textbf{Edge scenario} \\
%         \midrule
%         Off-chip DRAM read  & 10    & 10    \\
%         Off-chip DRAM write & 15    & 15    \\
%         On-chip SRAM read   & 1     & 1     \\
%         On-chip SRAM write  & 1.5   & 1.5   \\
%         Register file read  & 0.01  & 0.01  \\
%         Register file write & 0.015 & 0.015 \\
%         MAC operation       & 0.01  & 0.01  \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:energy-cost}
% \end{table}

\begin{figure}[htbp]
    \centering
    \subfigure[Subfigure 1]{%
        \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array.png}
        \label{fig:subfig1}
    }\hfill
    \subfigure[Subfigure 2]{%
        \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
        \label{fig:subfig2}
    }\vskip\baselineskip
    % \subfigure[Subfigure 3]{%
    %     \includegraphics[width=0.48\columnwidth]{figs/GPT3-175B_B=8_generic_array.png}
    %     \label{fig:subfig3}
    % }\hfill
    % \subfigure[Subfigure 4]{%
    %     \includegraphics[width=0.48\columnwidth]{figs/GPT3-175B_B=8_generic_array_edge.png}
    %     \label{fig:subfig4}
    % }
    \caption{Energy distribution in Llama1-7B and GPT3-175B models on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations. \rOneFC{[Chao: Robin, I think here we show llama-7b is enough, since our experiment will not cover gpt-175b. Maybe we can also remove the attention parts, i.e., Q*K$^{T}$ and S*V because we focus on FP-INT operations. Or we can split the Linear operations into qkv\_proj, out\_proj, and denote MLP as fc, like Fig.~\ref{fig:value_dist_wrt_addi_bits}, and merge Q*K$^{T}$ and S*V into the others to show the dominated energy consumption of FP-INT operations.]}
}
    \label{fig:zigzag}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \subfigure[]{%
%         \includegraphics[width=0.9\columnwidth]{figs/Llama1-7B_B=8_generic_array.png}
%         % \label{fig:subfig1}
%     }\hfill
%     \subfigure[Subfigure 2]{%
%         \includegraphics[width=0.9\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
%         % \label{fig:subfig2}
%     }\vskip\baselineskip
%     \subfigure[Subfigure 3]{%
%         \includegraphics[width=0.9\columnwidth]{figs/GPT3-175B_B=8_generic_array.png}
%         % \label{fig:subfig3}
%     }\hfill
%     \subfigure[Subfigure 4]{%
%         \includegraphics[width=0.9\columnwidth]{figs/GPT3-175B_B=8_generic_array_edge.png}
%         % \label{fig:subfig4}
%     }
%     \caption{Energy distribution in Llama1-7B and GPT3-175B models on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations}
%     \label{fig:zigzag}
% \end{figure}




% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{(a) Memory storage of W4A16 scheme compared to others (LLM-viewer); (b) FP16 takes majority energy consumption (Maybe from Zigzag?).}
%     \label{fig:1}
% \end{figure}

==> archive/0-abstr.tex <==
\begin{abstract}

% \rOneFC{The widely-used weight-only quantized large language models (LLMs), which leverage low-bit integer weights and retain floating-point (FP) activations, maintain accuracy while reducing storage requirements.}
% \rOneFC{However, FP activations contribute significantly to energy overhead due to high memory access costs, while the need for faster inference remains a pressing concern across various deployment scenarios.}
% \rOneFC{Our key finding is that FP activations contain redundant information, varying across different models and modules within LLMs.}
% \rOneFC{Leveraging this, we propose Anda, an adaptive data representation format for FP activations. Anda employs online grouping of shared exponent bits and dynamic mantissa bit allocation, substantially reducing memory access overhead and computational complexity.}
% % enabling aggressive bit-width reduction under inference accuracy constraints under deployment scenarios.}
% \rOneFC{We also develop a post-training adaptive precision combination search algorithm that iteratively optimizes the bit-width allocation for different modules, balancing model accuracy, energy efficiency, and inference speed within specified constraints.}
% % \rOneFC{To fully harness the advantages of Anda and further enhance system performance, we propose a suite of complementary hardware optimization techniques.}
% \rOneFC{To fully harness the advantages of Anda and further enhance system performance, we propose a suite of complementary hardware optimization techniques. These include a bit-plane-based data organization scheme, Anda-compatible processing units with bit-serial computation, and a runtime bit-plane Anda compressor, collectively optimizing storage, computation, and memory access efficiency.}
% \rOneFC{Evaluations on popular LLM families including OPT, LLaMA, and LLaMA-2 show that Anda achieves a 2.428× speedup and 3.148× energy efficiency improvement on average over existing GPU-based solutions. Anda demonstrates strong adaptability across various precision requirements and application scenarios, enabling efficient LLM inference in diverse environments.}

% \TODO{Check Arne's abstract rewrite.}

The widely-used, weight-only quantized large language models (LLMs), which leverage low-bit integer weights and retain floating-point (FP) activations, reduce storage requirements while maintaining accuracy. However, this shifts the energy and latency bottlenecks %overhead 
towards the FP activations that are associated with costly memory accesses and computations. %due to high memory access costs.} 
\ms{Existing LLM accelerators focus on optimizing energy-hungry FP computations, yet they do not effectively reduce data movements for FP activations and fail to provide any speedup in inference performance.}
%\ms{They also not optimize the memory accesses of FP, how to add this into the sentence? Arne, feel a bit redundant with the first one, let me think}
%\as{I took an attempt to add that information.}
%\todo{Add sentence on previous work that addresses energy bot doesn't tackle speedup.}

\as{\ms{To fill this gap,} we investigate the sensitivity of activation precision across various LLM modules and its impact on overall model accuracy. % in this work. 
%\ms{This achieves a reduction in memory footprints and computation by leveraging a lower activation precision with minimal accuracy impact.} 
Based on %this
%\ms{the investigation}
\rg{our findings}, we first propose the Anda data type: an adaptive data format with %online grouping of 
group-shared exponent bits and dynamic mantissa bit allocation. Secondly, we develop an iterative post-training adaptive precision search algorithm that optimizes the bit-width for different LLM modules to balance model accuracy, energy efficiency, and inference speed. Lastly, a suite of hardware optimization techniques is proposed to
\rg{maximally exploit}
% further boost
the benefits of the Anda format. 
These include a bit-plane-based data organization scheme, Anda-enhanced processing units with bit-serial computation, and a runtime bit-plane Anda compressor to \ms{simultaneously} optimize storage, computation, and memory footprints.}
% These include Anda-compatible processing units with bit-serial computation, a runtime bit-plane Anda compressor, and a bit-plane-based data organization scheme to \ms{simultaneously} optimize storage, computation and memory footprints.}
\as{Our evaluations show that Anda achieves 3.1$\times$ energy efficiency improvement and a 2.4$\times$ speedup on average for popular LLMs including OPT, LLaMA, and LLaMA-2 series over existing GPU-based solutions. Anda demonstrates strong adaptability across various application scenarios, accuracy requirements, and system performance, enabling efficient LLM inference across a wide range of deployment scenarios.}


% \rOneFC{First, we design a bit-plane-based data organization scheme for Anda format to optimize storage utilization and access efficiency. Second, we develop Anda-compatible hardware processing units that utilize bit-serial computation for multi-precision dot-product operations, enhancing computational flexibility and efficiency. Finally, we introduce an online bit-plane compression engine that efficiently converts FP numbers to the Anda format, further reducing memory access overhead.}
% === The origin version ===
% The widely-used weight-only quantized large language models (LLMs) leverage low-bit quantized weights and retain floating-point activations, aiming to maintain model accuracy while significantly reducing storage footprint. However, these floating-point activations are responsible for the majority of energy consumption during inference, including their costly memory access. In this paper, however, we will demonstrate that the FP activations contain redundant information, allowing for aggressive online bit reduction while preserving high model accuracy. As different modules exhibit varying sensitivities to quantization, we introduce Anda, an adaptive data representation method for floating-point activations in LLMs. Anda employs online group-shared exponents and dynamic mantissa allocation to reduce memory access overhead significantly. To demonstrate and quantify the benefits of Anda in an LLM accelerator, we design Anda-compatible hardware processing units using bit-serial computation for multi-precision dot-product calculations. Furthermore, we incorporate an online bit-plane compression
% engine and a bit-plane-based data organization scheme to improve storage utilization and further reduce memory access overhead. Evaluation of multiple popular LLMs, including the
% OPT, LLaMA, and LLaMA-2 series, demonstrates that ..

% % Weight-only quantization is a prevalent technique in large language models (LLMs) to reduce storage requirements. 
% The widely-used weight-only quantized large language models (LLMs) leverage low-bit quantized weights and retain floating-point activations, \mv{aiming to maintain} model accuracy while significantly reducing storage footprint.
% % However, floating-point activations significantly contribute to energy consumption during inference. 
% % \rOneFC{The weight-only quantized large language models (LLMs) that leverage low-bit quantized weights and retain floating-point activations, have gained widespread adoption for their ability to maintain model accuracy while significantly reducing storage requirements.}
% % \rOneFC{However, these models still face critical challenges in energy consumption and inference speed across various deployment scenarios. Floating-point activations, in particular, contribute significantly to the energy overhead due to their high memory access cost, while the need for faster inference times remains a pressing concern.}
% However, \mv{these} floating-point activations \mv{are responsible} for the majority of energy consumption during inference, including \mv{their costly} memory access.
% % and computation. 
% % Reducing this energy overhead is crucial for energy-constrained edge deployment of LLMs. %\rOneRG{[With the low-bit weights, the majority of the energy is spent on on-chip and off-chip activation memory access (computation energy is negligible)]}
% \mv{In this paper, however, we will demonstrate that the} %We find that 
% FP activations contain redundant information, allowing for aggressive online %quantization \rOneRG{[
% bit reduction %? - this is not really quantization]}
% while preserving high model accuracy. \mv{As} different modules exhibit varying sensitivities to quantization, we introduce Anda, an adaptive data representation method for floating-point activations in LLMs.
% Anda employs online group-shared exponents and dynamic mantissa allocation to reduce memory access overhead significantly. 
% \mv{To demonstrate and quantify the benefits of Anda in an LLM accelerator,} %Additionally, 
% we design \mv{Anda-compatible} hardware processing units using bit-serial computation for %flexible 
% multi-precision %activation 
% dot-product calculations. %, enhancing computational efficiency. 
% Furthermore, we incorporate an online bit-plane compression engine and a bit-plane-based data organization scheme to improve storage utilization and further reduce memory access overhead.
% Evaluation of multiple popular LLMs, including the OPT, LLaMA, and LLaMA-2 series, demonstrates that ...

% Weight-only quantized large language models (LLMs) leverage low-bit quantized weights while retaining floating-point activations. This approach maintains model accuracy and significantly reduces storage footprint, making it widely adopted in deployments.
% Despite the reduced storage from fixed-point quantized weights, floating-point activations account for the majority of energy consumption during inference, including memory access and computation. Reducing this energy overhead is crucial for energy-constrained edge deployment of LLMs.
% To optimize energy consumption in LLM deployment, we focus on floating-point activations. We found that they contain redundant information, allowing for aggressive online quantization while maintaining highly-preserved accuracy. Different modules exhibit varying sensitivities to quantization.
% Based on these findings, we propose a new adaptive data representation method for floating-point activations, called Anda. This format uses online grouped exponents and dynamic allocation of variable mantissas, significantly reducing memory access overhead for activations.
% We design efficient hardware processing units for the Anda data format, leveraging bit-serial computation to enable flexible multi-precision activation dot product calculations, enhancing computational efficiency.
% Additionally, we design an online bit-plane compression engine and a bit-plane-based data organization strategy for the Anda format, improving storage utilization and significantly reducing memory access overhead.
% We validate the Anda system on popular LLMs ranging from the OPT, LLaMA, and LLaMA-2 series.
% Experimental results show...
\end{abstract}

==> archive/0-archive.tex <==
\section{Archive}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/precision_mapping_on_LLM_block.png}
%     \caption{Precision mapping for an LLM blocks.}
%     \label{fig:prec_map}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/dpu_pattern.png}
    \caption{(a) first-bit-plane-then-element reduction pattern; (b) first-element-then-bit-plane reduction pattern.}
    \label{fig:archive_dpu_pattern}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/mapping_gemm_to_mxu.png}
    \caption{Mapping GEMM into the MXU.}
    \label{fig:mapping_mxu}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/concept_fig_flexible.png}
%     \caption{[Concept Figure] Our arch strengths over the others.}
%     \label{fig:concept_flexible}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs. Key Metrics: Perplexity (Black, lower is better), OPS Reduction (Red), and Activation Tensor Size Compression Ratio (Blue).}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccccccc@{}}
% \toprule
% \multicolumn{2}{c|}{}                  & OPT-1.3B & OPT-6.7B & LLaMA-7B & LLaMA2-7B & OPT-13B & LLaMA-13B  & LLaMA2-13B & OPT-30B & LLaMA-30B  \\ \midrule
% \multirow{7}{*}{WikiText2} & Omniquant & 14.88    & 10.96    & 5.77     & 5.59      & 10.20   & 5.17       & 4.95       & 9.62    & 4.19       \\
%                            & AWQ       & 14.94    & 10.93    & 5.81     & 5.62      & 10.21   & 5.20       & 4.97       & 9.59    & 4.21       \\
%                            & GPTQ      & 14.89    & 10.93    & 5.85     & 5.61      & 10.17   & 5.20       & 4.98       & 9.58    & 4.23       \\
%                            & RTN       & 15.29    & 11.15    & 5.96     & 5.72      & 10.30   & 5.25       & 4.98       & 9.94    & 4.23       \\
%                            & FIGNA     & 14.90    & 10.96    & 5.78     & 5.60      & 10.22   & 5.18       & 4.96       & 9.61    & 4.20       \\
%                            & VSQuant   & 19.04    & 12.24    & 7.45     & 8.26      & 11.63   & 6.36       & 6.43       & 10.67   & 5.10       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \midrule
% \multirow{7}{*}{PTB}       & Omniquant & 17.40    & 13.25    & 8.97     & 21.52     & 12.46   & 8.14       & 30.19      & 11.94   & 7.39       \\
%                            & AWQ       & 17.46    & 13.28    & -        & -         & 12.46   & \textbf{-} & \textbf{-} & 11.90   & \textbf{-} \\
%                            & GPTQ      & 17.41    & 13.21    & -        & -         & 12.42   & \textbf{-} & \textbf{-} & 11.89   & \textbf{-} \\
%                            & RTN       & 33.63    & 16.05    & -        & -         & 15.40   & \textbf{-} & \textbf{-} & 14.17   & \textbf{-} \\
%                            & FIGNA     & 17.41    & 13.26    & 8.98     & 21.52     & 12.47   & 8.15       & 30.19      & 11.95   & 7.40       \\
%                            & VSQuant   & 25.64    & 15.50    & 15.78    & 53.46     & 14.47   & 12.54      & 49.91      & 13.47   & 9.92       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \midrule
% \multirow{7}{*}{C4}        & Omniquant & 15.03    & 11.85    & 7.21     & 7.12      & 11.29   & 6.69       & 6.56       & 10.75   & 6.06       \\
%                            & AWQ       & 15.04    & 11.87    & 7.21     & 7.13      & 11.28   & 6.70       & 6.56       & 10.75   & 6.05       \\
%                            & GPTQ      & 15.05    & 11.87    & 7.21     & 7.12      & 11.26   & 6.69       & 6.56       & 10.74   & 6.06       \\
%                            & RTN       & 15.71    & 12.31    & 7.37     & 7.24      & 11.51   & 6.69       & 6.58       & 10.94   & 6.06       \\
%                            & FIGNA     & 15.04    & 11.86    & 7.22     & 7.12      & 11.29   & 6.70       & 6.57       & 10.75   & 6.06       \\
%                            & VSQuant   & 19.00    & 13.13    & 8.89     & 10.36     & 12.64   & 7.85       & 8.35       & 11.91   & 6.85       \\
%                            & Ours      &          &          &          &           &         &            &            &         &            \\ \bottomrule 
% \end{tabular}%
% }
% \end{table*}

==> archive/1-intro-v0.tex <==
% \rOneFC{Some writing references to learn from:}
% \begin{itemize}
%     \item \rOneFC{[MICRO'16] Stripes \cite{judd2016stripes}: the first work to leverage bit-serial computing in DNNs.}
%     \item \rOneFC{[HPCA'22] FAST \cite{zhang2022fast}: exploit DNN training with variable precision block floating point (BFP) numbers, and its BFP numbers are on-the-fly converted as well.}
%     \item \rOneFC{[HPCA'24] BitWave \cite{shi2024bitwave}: bit-serial computing with bit-column sparsity. Learn how to orchestra each part of the paper.}
%     \item \rOneFC{[HPCA'24] FIGNA \cite{jang2024figna}: the first work to focus on FP-INT GEMM optimizations with shared exponents. Our highly relevant baseline.}
%     \item \rOneFC{[JSSC'23] VS-Quant \cite{keller202395}: the two-level per-vector scaling quantization but requires retraining to recover accuracy. Our highly relevant baseline.}
% \end{itemize}

\section{Introduction} \label{sec:intro}

% \rOneFC{[Chao: I think the current intro is too lengthy. Maybe we need to discuss further how to build an attractive intro based on our claimed contributions.]}

% \rOneFC{[Goal: LLM's brief intro. Focus on challenges for LLM deployment.]}
The recent emergence of large language models (LLMs) has a profound impact on the world and is followed by a rapid, widespread adoption. Though highly in demand, their deployment is challenging due to their immense computational and storage demands. 
For example, GPT-3's 175 billion parameters require approximately 350GB of FP16 storage, surpassing the memory capacity of current commodity GPUs. For cloud environments, their deployment is facilitated by energy-hungry, purpose-built GPUs. In contrast, deployment on edge devices remains infeasible.

% \rOneFC{[Goal: Weight-only quantized LLMs have become a prevalent choice for deploying LLM models on edge devices.]}
Quantization serves as an effective technique to lower storage and computational demands by reducing the model's precision. Post-training Quantization (PTQ) stands out as a practical choice due to its lower training data dependency, shorter optimization time, and comparable model performance compared to Quantization-aware Training (QAT). Within PTQ, weight-only quantization has gained prominence in edge device deployment scenarios. 
% Unlike weight-activation quantization, which quantizes both weights and activations, weight-only quantization preserves activation data in FP16 precision, leading to reduced storage requirements.
In contrast to weight-activation quantization where both weights and activations are quantized, weight-only quantization maintains activations in FP16 precision and quantizes weights exclusively. 
This enables weight quantization to 4-bit integers while preserving model accuracy, achieving significant reductions in the model's storage cost. 
Consequently, weight-only quantization has become a prevalent choice for deploying LLM models on edge devices.

\rOneRG{[This should move to Motivation]}
% \rOneFC{[Goal: FP-INT operations are dominated in weight-only quantized LLMs, which requires further optimizations.]}
To further optimize the deployment of weight-only quantized LLMs, we first need to understand the distribution of their computational operations. We explored the proportion of FP-INT operations in text generation tasks for different context length ratios across a range of weight-quantized LLMs. As shown in the figure, when the generation length is 25\% of the maximum length, FP-INT operations account for an average of 97\%, and even when the generation length reaches 100\% of the maximum length, FP-INT operations still average over 90\%, demonstrating their significant dominance.
This implies that FP-INT operations account for the vast majority of the computational workload in text generation tasks, making them crucial for further deployment optimization. Therefore, we focus our optimization efforts on FP-INT operations.

% \rOneFC{[Goal: Activaitons in FP-INT GEMMs take the majority of energy consumption, including off-chip footprints, on-chip footprints, as well as computational costs. And therefore, it is essential to exploit optimizations towards activations for energy-efficient LLM inference.]}
In edge deployment scenarios, energy efficiency is paramount beyond storage constraints. While weight-only quantization reduces storage overhead, it fails to address the large energy cost of LLM inference. For edge devices, energy efficiency is a more stringent constraint than storage cost.
% with activations during FP-INT operations, which form the core computational workload in large models.
The activations remain in a high-precision format, incurring high energy consumption due to (1) frequent off-chip accesses due to limited on-chip space for storing entire next-layer FP16 activations, and (2) substantial on-chip memory access overhead compared to INT4 weights.


\rOneFC{[Goal: Summarize our work with focus on what techniques we leverage to solve what challenges mentioned above.]}
% The inference of large language models (LLMs) is bottlenecked by the computation and storage of floating-point (FP) activations, which incur significant energy overheads. 
To address the high energy cost associated with data movements of activations in weight-only quantization schemes, we conducted extensive experiments and made the following key observations:
\begin{enumerate}
    \item Nearby activations can be grouped to share the exponent part, which helps simplify the computation in the FP-INT units, while the appropriate group size has a negligible impact on model accuracy.
    \item There exists substantial redundancy in the mantissa part of FP activations, and different mantissa bitwidths trade off accuracy for different application scenarios, enabling flexible adjustment.
    \item Different modules in LLMs exhibit varying sensitivity of activation precision to model accuracy, necessitating a finer-grained exploration of the precision-bitwidth balance.
\end{enumerate}

Based on these findings, we propose Anda, a novel numerical format that enables energy-efficient and performance-scalable LLM inference. Anda dynamically shares exponents at runtime and automatically adjusts the variable-length mantissas based on user requirements. This design significantly reduces the data movement and computation overheads of the activations while supporting flexible precision tuning for different deployment scenarios, thereby achieving energy-efficient and performance-scalable LLM inference.
To efficiently process data in the Anda format, we further develop corresponding arithmetic units that leverage bit-serial operations to perform efficient FP-INT dot-product computations within shared-exponent groups. Additionally, to reduce the overhead of frequent memory accesses, we propose an on-the-fly compression engine to convert FP output activations to the Anda format. We also design an efficient online data orchestration scheme to improve the memory access efficiency of the Anda format.
Finally, we integrate the Anda format and aforementioned components into a single system and conduct comprehensive evaluations, demonstrating its superior performance in enabling energy-efficient and performance-scalable LLM inference.
% The contribution of this paper can be summarized as follows:
The major highlights of this work are as follows:
\begin{itemize}
    \item \textbf{Anda data format.} We propose a novel data format to reduce memory access overhead and computational complexity involved in FP activations, enabling online precision adjustment for better energy-performance-accuracy trade-offs. It achieves a xx\% reduction in memory access overhead and a xx\% reduction in required operations (OPS) within only 1\% negligible accuracy trade-off. (Sec.~\ref{sec:algo})
    % We propose a novel data representation format, Anda, specifically designed for optimizing activation data in FP-INT quantized LLMs. Anda format effectively reduces both storage and computation costs of activation data, leading to significant improvement in model energy efficiency.
    \item \textbf{Efficient arithmetic unit.} We design an efficient dot-product processing unit for activations in Anda format, achieving high area efficiency and energy efficiency with flexible precision adjustment. Compared to other equivalent units, it achieves a xx\% improvement in area efficiency and a xx\% improvement in energy efficiency at xx mantissa precision. (Sec.~\ref{subsec:dpu})
    \item \textbf{On-the-fly compression support.} We propose an on-the-fly compression engine to efficiently convert FP format to Anda format, significantly reducing off-chip and on-chip traffic and memory energy consumption. Moreover, we design a bit-plane data storage scheme for Anda format to improve storage utilization and reduce data movement costs. The compression efforts, with the cost of area overhead of xx\%, achieve xx\% reduction in memory access overhead, and xx\% energy saving compared to the original FP-INT format. (Sec.~\ref{subsec:comp} \& \ref{subsec:scheme})
    \item \textbf{System integration.} We build a computing system based on Anda format and conduct comprehensive experiments on nine popular LLMs. The results demonstrate that Anda format can significantly improve the area efficiency and energy efficiency of models with flexible energy-performance-accuracy trade-off. Specifically, with no loss in accuracy, Anda format achieves an average improvement of XX\% in area efficiency and XX\% in energy efficiency. When allowing a 1\% accuracy loss, the average improvements are XX\% in area efficiency and XX\% in energy efficiency. (Sec.~\ref{subsec:overall})


\end{itemize}

\textbf{=== Below is OUTLINE ===}
\begin{itemize}
    \item Why do we focus on weight-only quantized LLMs?
        \begin{itemize}
            \item Near-lossless model accuracy...
            \item Its unique benefits on memory consumption...
            % Also because of the benefit of ASIC compared to FPGA? We can more easily deal with the datatype conversions, so there is more to gain
            \item \rOneRG{We take weight-only quantization as a given}
        \end{itemize}
    \item What issues still exist in weight-only quantized LLMs?
        \begin{itemize}
            \item FP16 activations dominate energy consumption from two sides: memory access \& computation... (Here we need Robin \& Arne's help!) [Fig.~\ref{fig:zigzag}]
            \item FIGNA's \cite{jang2024figna} shortcomings in these two aspects: 1) memory access, FP16 in full precision storage plus repeated access consumes more energy... 2) computation, INT multiplier with high bitwidth preserving numerical accuracy consumes more energy... [Fig.~\ref{fig:2}]
        \end{itemize}
    \item What interesting findings do we have found?
        \begin{itemize}
            \item We don't need to maintain numerical accuracy due to the robustness of LLMs...Aggressive cutting mantissa bits within a shared exponent element group is feasible within 1\% negligible accuracy loss...
            \item Layer-wise sensitivity to mantissa bit cutting is near-uniform, while module-wise sensitivity is quite different, motivating us to explore flexible activation precision across modules...
        \end{itemize}
    \item How to resolve the above challenges based on our findings?
        \begin{itemize}
            \item From algorithm aspects, we propose a heuristic post-training algorithm to determine the bitwidth of each module of LLMs... (computation \& memory access)
            \item From architecture aspects, we design an energy-efficient accelerator with several features: 
                \begin{enumerate}
                    \item activation-bit-serial with shared exponent group PEs to enable flexible mantissa bit precision... (computation)
                    \item online bit-plane compression engine to reduce the memory access consumption... (memory access)
                    \item bit-plane data orchestration scheme to enable efficient storage utilization and transfer cost... (computation \& memory access)
                \end{enumerate}
        \end{itemize}
\end{itemize}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{(a) Concept of these two issues; (b) Concept of our findings; (c) Our Anda solution.}
%     \label{fig:2}
% \end{figure}

==> archive/1-intro-v1.tex <==
\section{Introduction} \label{sec:intro}

Large language models (LLMs) \cite{chowdhery2023palm, zhang2022opt, touvron2023llama, team2024gemma} have demonstrated remarkable proficiency in a wide array of natural language processing tasks, including text generation, question answering, and automatic summarization. %, \ms{and so on}. 
The extraordinary success of LLMs can be attributed to the scaling law \cite{bahri2024explaining}, which posits that performance improves dramatically with %increases in 
\ms{the ever-increased} model size, training data volume, and computational resources. 
%\ms{For instance,} t
\mv{T}he evolution of the GPT series \cite{achiam2023gpt, kalyan2023survey, bhattacharya2024demystifying} on model size strikingly illustrates this principle: while GPT-1 comprised a modest 117 million parameters in 2018, its successor GPT-4 is speculated to encompass over a trillion parameters \ms{along with considerable enhanced language understanding and generation capabilities}. 
% This exponential growth in scale has substantially enhanced the capacity of LLMs to tackle intricate and multifaceted tasks, pushing the boundaries of artificial intelligence in language understanding and generation.
%\ms{I cut the following sentence. feel it is redundant with the previous one.}
%As groundbreaking applications like OpenAI's ChatGPT~\cite{openai2024chatgpt} and Microsoft's Copilot~\cite{microsoft2024copilot} gain widespread popularity, LLM inference has emerged as a significant workload across various computing platforms \cite{hu2024characterization, yu2022orca, dhar2024empirical, yin2024llm}, from cloud infrastructures to edge devices. 
However, the exponential growth in LLM model sizes has created substantial deployment challenges, imposing enormous demands on storage and computational resources. 
% This escalating resource requirement underscores the critical need for efficient model compression techniques, particularly quantization, to optimize LLM performance and facilitate wider deployment.

Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} is one of the most popular techniques to %tackle resource issues.
\ms{reduce memory footprints and computation costs.}
%\ms{[I feel you don't need to talk about two different quantization methods. Focus on weight-only quantization as the most common quantization.]}
%Two primary quantization strategies are commonly employed \ms{for LLMs}: weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} and weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}. Weight-activation quantization quantizes both weight and activation parameters, while weight-only quantization focuses solely on weight parameters. 
\ms{To maximally shrink the model size, the most common quantization strategy \mv{for LLMs today} involves aggressively lowering the precision of the weights while typically maintaining high precision for activations due to the presence of outliers~\cite{dettmers2022gpt3, wei2022outlier}, a technique known as weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, zhao2024atom, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit}.} %Notably, weight-only quantization, particularly 
\ms{For example, the W4A16 scheme \cite{shao2024omniquant}, where weights are represented using 4-bit fixed-point integers (INT4) and activations are represented using 16-bit floating-point numbers (FP16), has gained substantial traction in LLM \mv{because of its significant impact on} %. This approach is effective because INT4 weights significantly reduce storage requirements during deployment \cite{yuan2024llm}, as weight parameters typically dominate 
the model's memory footprint during deployment \cite{yuan2024llm}.}
%However, the energy bottleneck shifts toward activation movements when weights are aggressively quantized, which raises the demand for the optimization of the FP16 activation. [Can we have a figure to show this shifting??]
%the W4A16 scheme \cite{shao2024omniquant}, where weights are represented using 4-bit fixed-point integers (INT4) and activations are represented using 16-bit floating-point numbers (FP16), has gained significant traction in LLM serving due to several compelling advantages: 1) Weight parameters typically account for the majority of a model's storage footprint. Weight-only quantization allows for aggressive quantization of weights to lower bitwidths, effectively alleviating storage constraints during deployment \cite{yuan2024llm}. 2) Activation values exhibit a wider dynamic range compared to weights, making them more challenging to quantize effectively. By retaining activations in FP16 format, weight-only quantization preserves the expressive power of activations while minimizing storage requirements \cite{lin2024awq}. 3) Limiting quantization to weights while keeping activations in FP16, eliminates frequent and complicated quantization-dequantization overhead and boosts inference speed compared to weight-activation quantization~\cite{lin2024qserve}.

% As weight-only quantization becomes increasingly important, NVIDIA introduced a new FP-INT GEMM kernel in CUDA’s CUTLASS and other researchers proposed specialized GPU kernels for this purpose. However, these kernels still rely on existing FP units for FP-INT GEMM computations, which involves dequantizing INT weights to FP values and incurs additional computational overhead. While this approach effectively reduces storage requirements and memory bandwidth, it does not fully address the increased computation costs. To further alleviate these costs, there have been explorations into transforming FP units into dedicated FP-INT arithmetic cores. Despite these efforts, the benefits are limited due to the inherent complexities of floating-point operations, such as exponent alignment and normalization. To simplify FP-INT operations in weight-only quantization, the FIGNA framework proposes a novel approach. FIGNA maintains activation values in FP16 format and employs a pre-alignment method to convert traditional FP operations into INT operations, significantly enhancing computational efficiency while preserving numerical precision comparable to FP arithmetic.

% As weight-only quantization becomes increasingly crucial, NVIDIA has introduced a new FP-INT GEMM kernel in CUDA’s CUTLASS, and other researchers have proposed specialized GPU kernels for this purpose. 
% While these kernels reduce memory footprint and bandwidth usage, they rely on existing FP units for FP-INT GEMM, which introduces additional computational overhead due to the need for dequantizing INT weights to FP values. 
% To further reduce computational costs, there has been exploration into converting FP units into dedicated FP-INT arithmetic units. 
% However, the complexity of operations like exponent alignment and normalization limits the potential gains. 
% To simplify FP-INT operations in weight-only quantization, the FIGNA framework proposes a novel approach. 
% FIGNA maintains activation values in FP16 format and employs a pre-alignment method to convert traditional FP operations into INT operations, achieving significant computational efficiency while maintaining precision. 
% Nevertheless, FIGNA’s approach does not optimize activation storage, leading to increased energy consumption due to redundant activation data access compared to weight data.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/ops_breakdown.pdf}
    \caption{FP-INT operations are dominated in weight-only quantized LLMs.}
    \label{fig:fp_int}
\end{figure}

% \begin{figure}[htbp]
%     \centering
%     % \subfigure[]{%
%     % }\hfill
%     % \subfigure[]{%
%     \includegraphics[width=0.46\columnwidth]{figs/memory_consumption.png}
%     \includegraphics[width=0.46\columnwidth]{figs/energy_weight_act.png}
%     \caption{Energy distribution of various LLM models on a typical cloud accelerator.}
%     \label{fig:zigzag}
% \end{figure}

% \ms{[feel the following para is not well connected with the previous para...should we say that the bottleneck of LLMs switches from memory-bound to computation-bound with the weight-only quantization, then say the optimization on the computation is necessary? or the energy bottleneck shifts to activation data movements? Anyway, we should mention the optimization target is activation and the reason before introduce our work.]} \mv{[I gave it a try]\\}
With the rising importance of weight-only quantization, \mv{initiates an interesting shift in the LLM inference bottlenecks. The burden now shifts to the activation data movements, and new optimized operators for FP-INT operations become indispensable.} 
Fig.~\ref{fig:fp_int} illustrates the relative distribution of operations for various W4A16 LLMs across different token lengths in text generation tasks. 
Notably, FP-INT operations consistently dominate, accounting for over 90\% of the total computational workload across all models and scenarios examined. 
This overwhelming prevalence underscores the critical importance of optimizing FP-INT GEMM operations to achieve efficient inference deployment for W4A16 LLMs. 

NVIDIA’s new FP-INT GEMM kernel \cite{nvidia2024cutlass}, \mv{as well} specialized GPU kernels \mv{optimizing activation memory bandwidth} \cite{jeon2020biqgemm, xia2024fp6, frantar2023optq} \mv{are a consequence of this evolution}. %have been introduced to manage memory and bandwidth more effectively. 
\mv{However, these optimized GPU kernels all} %While these kernels are beneficial for reducing storage, they 
still rely on FP units \mv{by} converting the INT weights to FP values for \mv{execution in FP} GeMM \mv{operatiors} \cite{lin2024qserve}. %, which adds computational overhead from converting INT weights to FP values. 
% \mv{In literature,} there have been efforts to develop dedicated FP-INT arithmetic units, \mv{in which the challenge lies in reducing the overhead stemming from the} exponent alignment and normalization. % limits performance improvements.
\rOneFC{In the literature \cite{jang2024figna}, efforts have been made to develop dedicated FP-INT arithmetic units, with the challenge lying in reducing the hardware overhead stemming from exponent alignment and normalization.}
\rOneFC{In addition to developing dedicated FP-INT computing units, another optimization approach is %to attempt 
to convert FP activations to a block floating point (BFP) data format for computation.}
\rOneFC{Since in BFP \mv{adjacent elements} share and exponent, the overhead of exponent alignment and normalization \mv{within a group disappears}, simplifying the operation to fixed-point arithmetic. 
However, directly applying previously proposed BFP formats \mv{to a pre-trained network} significantly impacts model accuracy. \mv{As a result, this is only possible in combination with} costly retraining \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock}, or \mv{with the usage of} a large mantissa field to preserve precision during conversion, resulting in substantial memory access and computational overhead \cite{jang2024figna, kim2023winning}.}
% FIGNA~\cite{jang2024figna} %represents a step forward by using FP16 for storage and 
% \mv{exploits} a grouped pre-alignment method to streamline computations with preserved numerical accuracy. % to FP arithmetic, 
% Yet, it falls short in optimizing \mv{the storage and energy footprint of the} activation data, \mv{which is still represented as FP16}. % , leading to increased energy consumption from inefficient activation data access. 
% \mv{[Can we discuss one more, besides FIGNA?]]}

% In this paper, we propose Anda, a novel data format as a drop-in replacement of FP16 activation for performance-scalable efficient LLM inference.

%Building upon these prior works and addressing their limitations 
\mv{The overcome these limitations of the SotA}, we propose Anda, a novel activation-oriented data format designed to directly replace FP16 without incurring any retraining overhead, which is \mv{important for LLMs due to their enormous} %impractical in LLM era due to the drastic 
training cost. 
\ms{Compared to the traditional FP16 data format, the Anda data type} \ms{reduces both} storage requirements  and computational costs, \mv{due to its shared exponent and adjustable mantissa bit-width. Moreover, Anda} allows a flexible trade-off between model accuracy and performance.
%Anda significantly reduces both storage requirements and computational costs associated with activation data and enables a flexible trade-off between model accuracy and performance through precision adjustments. 
% \mv{[I am not sure whether you should keep the following two sentences here. In my view, people can not understand them at this stage of the paper yet, and it is also not something that we deeply explpore in the paper. Not the core idea. I would first explain the rest, and add this rather a bit later.]}
% \mv{[[[} This feature holds substantial promise for LLM \mv{deployment}, particularly in scenarios with strict \mv{latency} constraints where applications may prioritize timely responses over maximum accuracy. 
% By offering this adaptability, Anda addresses a critical need in real-world LLM deployments, where the balance between accuracy and speed can be dynamically optimized based on specific use-case requirements. \mv{]]]}
% \mv{Towards this goal}, we \mv{in this paper} first identify the energy bottleneck associated with activations in LLM inference. Our analysis reveals that activations become the primary energy consumption in compute-bound LLM inference scenarios, particularly for quantized W4A16 LLMs. 
% This is due to their higher bit width and more frequent memory accesses compared to weights. 
% Consequently, approaches like FIGNA \cite{jang2024figna, kim2023winning}, which only transform data during computation while maintaining FP16 format for storage, show limited potential for energy optimization. 
% This observation motivates our exploration of a more efficient data representation for activations, aimed at simultaneously optimizing storage, memory access, and computational costs. 
% By addressing these multiple aspects, we seek to achieve comprehensive efficiency improvements in LLM inference, particularly in energy-constrained environments.
% While FIGNA demonstrated the feasibility of dynamically sharing exponent segments among adjacent activation elements at runtime to simplify mantissa computations, they expanded the aligned mantissa width to maintain numerical precision equivalent to the original FP format. However, our research reveals that as LLM sizes increase, they exhibit a higher tolerance for numerical precision errors in the mantissa. This finding suggests that after sharing exponent segments, the aligned mantissa width not only doesn't require expansion but can actually undergo aggressive reduction. This reduction is particularly promising, offering the potential to significantly decrease both storage and computational costs while maintaining LLM accuracy. Furthermore, our exploration uncovers that in W4A16 LLMs, different key modules exhibit varying sensitivities to mantissa reduction. Consequently, adopting different mantissa widths for different modules under the same model accuracy constraints can lead to even greater reductions in computational and storage overheads. 
% This modular approach to precision optimization represents a novel strategy for enhancing LLM efficiency without compromising performance.
% Based on these findings, we propose the Anda data format to accommodate the varying sensitivity of mantissa width across different modules and models in LLM FP activations. Anda dynamically shares exponent segments between adjacent elements at runtime while featuring a variable-width mantissa. 
This adaptive, \mv{varibale-mantissa}-length format adjusts according to model \mv{sensitivities}, yet remains transparent to users during execution, serving as a direct replacement for FP16 activation. 
\mv{In this work, we assess optimize and demonstrate the benefits of the Anda data type in a complete system setting.}
% \\
% \\
% \mv{[(If out of space) I WOULD CUT EVERYTHING FROM HERE...]\\}
% To identify optimal mantissa widths for different LLM modules we develop a rapid search algorithm \ms{within tolerated accuracy constraints}. Through \ms{a} minimal iterative \ms{mantissa bit length} relaxation, this algorithm efficiently finds feasible solutions %on calibration datasets
% that minimize both accuracy error and operand count. %This approach effectively reduces model storage, memory access, and computational costs while maintaining model accuracy.
% To fully harness Anda's potential in LLM inference, we construct a comprehensive computing system with the following key features: 
% 1) An activation data layout scheme for the variable-length Anda format, significantly reducing storage overhead while enabling efficient data access, thus achieving substantial savings in memory access energy. 
% 2) A flexible and efficient mantissa dot-product computation unit designed using a bit-serial approach, adapting to efficient computation of various fixed-length Anda data and enhancing computational efficiency for Anda format data.
% 3) A runtime bit-plane compressor that compresses output activations into Anda format before writing back to memory, dramatically reducing activation storage and memory access overheads.
% This integrated system leverages the Anda format to optimize LLM inference across multiple dimensions, addressing the challenges of storage, computation, and energy efficiency in large-scale model deployment.
% Extensive evaluation on Anda format shows \TODO{}... 
% \mv{[(If out of space) ... UNTIL HERE]\\}
\mv{Therefore,} %In summary, 
this paper makes the following contributions:
\begin{itemize}
    \item We \mv{formalize} Anda, a variable-length data format with dynamically shared exponents and adjustable mantissa widths for activations, directly replacing FP16 activations and adapting to precision requirements across different LLM modules.
    \item We develop an efficient algorithm to identify optimal mantissa widths for various LLM modules within given accuracy tolerances, balancing model accuracy and efficiency.
    \item We design \mv{an Anda-compatible} accelerator \mv{down to the RTL level,} featuring 1.) an \mv{Anda-}optimized \mv{memory layout}, %data layout, 
2.) flexible \mv{widely-parallel} dot-product computation units, and a 3.) a runtime \mv{data} compressor \mv{in the memory interface}, significantly enhancing storage, memory access, and compute efficiency. % for the Anda format
    \item Extensive evaluation \mv{of the system-level energy and throughput savings from the} Anda format \mv{across various LLMs} shows ... 

\end{itemize}

\mv{The paper is organized as follows: Sec.~\ref{sec:bkg} reviews the benefits and remaining bottlenecks of weight-only quantization methods, and quantifies the sensitivity of LLM accuracy to the shared exponents and reduced mantissa lengths. Based on these findings, Sec.~\ref{sec:algo} formalizes the proposed Anda data format as well as the algorithm to find the most optimal mantissa lengths for an LLM. Next, an Anda-optimized hardware architecture is proposed in Sec.~\ref{sec:arch}, which allows to derive system-level efficiency gains in Sec.~\ref{sec:eval} and benchmark it against the SotA. Sec.~\ref{sec:concls} concludes the paper.}

==> archive/1-intro.tex <==
\section{Introduction} \label{sec:intro}
Large language models (LLMs) \cite{chowdhery2023palm, zhang2022opt, touvron2023llama, team2024gemma, achiam2023gpt} have demonstrated remarkable proficiency in a wide array of natural language processing tasks, including text generation, question answering, and automatic summarization.
The extraordinary success of LLMs can be attributed to the scaling law \cite{bahri2024explaining}, which posits that performance improves dramatically with 
the ever-increased model size, training data volume, and computational resources. 
The evolution of the GPT series \cite{achiam2023gpt, kalyan2023survey, bhattacharya2024demystifying} on model size strikingly illustrates the scaling law: while GPT-1 comprised a modest 117 million parameters, its successor GPT-4 is speculated to encompass over a trillion parameters.
% along with considerably enhanced language understanding and generation capabilities. 
However, the exponential growth in LLM model sizes has created substantial deployment challenges, imposing enormous demands on storage and computational resources. 

% Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} is one of the most popular techniques to reduce memory footprints and computation costs.
\rOneFC{To address these challenges, quantization techniques \cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq, xia2024fp6} have been widely adopted in LLMs to reduce memory footprint and lower deployment costs.}
% To maximally shrink the model size, the most common quantization strategy for LLMs today involves aggressively lowering the precision of the weights while typically maintaining high precision for activations due to the presence of outliers~\cite{dettmers2022gpt3, wei2022outlier}, a technique known as weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, zhao2024atom, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit}.
\rOneFC{To maximally shrink the model size, the most common strategy for LLMs today is weight-only quantization~\cite{park2024lutgemm, dettmers2023case, chee2024quip, lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit}, which aggressively lowers the precision of the weights while maintaining high precision for activations due to the presence of outliers \cite{dettmers2022gpt3, wei2022outlier}.}
% For example, the W4A16 scheme \cite{shao2024omniquant}, where weights are represented using 4-bit fixed-point integers (INT4) and activations are represented using 16-bit floating-point numbers (FP16), has gained substantial traction in LLM because of its significant impact on the model's memory footprint during deployment \cite{yuan2024llm}.
\rOneFC{In particular, the widely adopted W4A16 scheme~\cite{shao2024omniquant, frantar2023optq}, which quantizes weights into 4-bit integers (INT4) while retaining activations in 16-bit floating-point format (FP16), significantly reduces memory requirements and bandwidth, lowering GPU memory usage by nearly 4$\times$~\cite{yuan2024llm} and facilitating deployment to smaller devices~\cite{lin2024awq, nvidia2024cutlass}.}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/anda_concept.pdf}
    \caption{Overview of the drop-in replacement process for FP activations using the variable-length grouped Anda data type. This achieves significant energy efficiency improvement and speedup through the proposed adaptive precision combination search algorithm and the Anda-aware architecture.}
    \label{fig:anda_concept}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/ops_breakdown_v4.pdf}
    % \caption{FP-INT operations are dominated in weight-only quantized LLMs.}
    \caption{FP-INT GeMM operations dominate in weight-only quantized LLMs with different context lengths and model sizes for text generation tasks.
    % \TODO{If time permits, we may replace or add a sub-group experiment using CUTLASS half-precision GeMM. Step out of this comfort zone may cost a week: \url{https://github.com/NVIDIA/FasterTransformer/tree/main/src/fastertransformer/kernels/cutlass_kernels/fpA_intB_gemm}}
    }
    \label{fig:fp_int}
\end{figure}

% With the rising importance of weight-only quantization, initiates an interesting shift in the LLM inference bottlenecks. The burden now shifts to the activation data movements, and new optimized operators for FP-INT operations become indispensable.
% \rOneFC{With the rising importance of weight-only quantization, FP-INT GeMM operations have become indispensable in LLM inference.}
% % Fig.~\ref{fig:fp_int} illustrates the relative distribution of operations for various W4A16 LLMs across different token lengths in text generation tasks. 
% % Notably, FP-INT operations consistently dominate, accounting for over 90\% of the total computational workload across all models and scenarios examined. 
% \rOneFC{As shown in Fig.~\ref{fig:fp_int}, FP-INT GeMM operations dominate the computational workload, accounting for over 90\% of the total workload across various W4A16 LLMs and context token lengths in text generation tasks.}
% \rOneFC{The relative OPs are independent of batch size since the OPs linearly scale with batch size both in LLMs.}
% This overwhelming prevalence underscores the critical importance of optimizing FP-INT GeMM operations to achieve efficient inference deployment for W4A16 LLMs. 

% \rOneFC{The widespread adoption of weight-only quantization has made FP-INT GeMM operations crucial in LLM inference. Fig.~\ref{fig:fp_int} illustrates the dominance of these operations across various W4A16 LLMs and context token lengths in text generation tasks. FP-INT GeMM consistently accounts for over 90\% of the total computational workload, regardless of batch size due to the linear scaling of operations in LLMs. This prevalence highlights the critical need to optimize FP-INT GeMM operations for efficient W4A16 LLM inference deployment.}

\rOneFC{With the increasing importance of weight-only quantization, FP-INT GeMM operations~\cite{jang2024figna} have become indispensable in LLM inference.}
\rOneFC{As illustrated in Fig.~\ref{fig:fp_int}, FP-INT GeMMs dominate the computational workload, making up over 90\% of the total number of operations across various weight-only quantized LLMs and context token lengths in text generation tasks.}
% \rOneFC{This dominance remains consistent regardless of batch size, as operations scale linearly with it.} 
\rOneFC{Such prevalence highlights the urgent need to optimize FP-INT GeMM operations for efficient LLM inference.}


% \TODO{} 
% NVIDIA’s new FP-INT GeMM kernel~\cite{nvidia2024cutlass}, as well as other specialized GPU kernels~\cite{jeon2020biqgemm, xia2024fp6, frantar2023optq} optimizing weight memory bandwidth are a consequence of this evolution. 
NVIDIA’s new FP-INT GeMM kernel~\cite{nvidia2024cutlass}, as well as some specialized GPU kernels~\cite{jeon2020biqgemm, xia2024fp6, frantar2023optq}, are a consequence of this evolution.
However, these optimized GPU kernels still rely on using FP units by converting the INT weights to FP values for execution in FP GeMM operators~\cite{lin2024qserve}. 
% In the literature \cite{jang2024figna}, efforts have been made to develop dedicated FP-INT arithmetic units, with the challenge lying in reducing the hardware overhead stemming from exponent alignment and normalization.
\rOneFC{Efforts have been made to develop dedicated FP-INT arithmetic units~\cite{jang2024figna}, while the additional costs of exponent alignment and normalization persist, resulting in complicated hardware implementation.}
% \as{Efforts have been made to develop dedicated FP-INT arithmetic units~\cite{jang2024figna}, which incurs additional exponent alignment and normalization costs, and results in a complicated hardware implementation.}
% In addition to developing dedicated FP-INT computing units, 
\rOneFC{To reduce hardware cost,}
another optimization approach is to convert the FP activations to a block floating point (BFP) data format for computation~\cite{koster2017flexpoint, drumond2018training, darvish2020pushing}.
Since grouped BFP elements share an exponent, the overhead of exponent alignment and normalization within a group disappears, simplifying the operation to \rOneFC{INT} 
arithmetic. 
% However, directly applying previously proposed BFP formats to a pre-trained network significantly impacts model accuracy. 
% \rOneFC{However, to mitigate accuracy loss when converting FP activations to BFP format on a pre-trained network, this is only possible in combination with costly retraining \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock, guo2023boost}, which is impractical for agile 
% % % and out-of-the-box 
% LLM deployment, or with the usage of a large mantissa field to preserve precision during conversion~\cite{jang2024figna, kim2023winning}, leading to significant energy consumption due to computational overhead and heavy memory accesses.}
However, to mitigate accuracy loss when converting FP activations to BFP format on a pre-trained network, costly retraining \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock, guo2023boost} is required, hindering agile LLM deployment. Alternatively, accuracy can be preserved by using a large mantissa field conversion~\cite{jang2024figna, kim2023winning}, but this significantly increases the energy consumption due to computational and memory access overhead of the additional bits.


% \as{However, applying BFP activations to a pre-trained network significantly degrades model accuracy and thus needs to be combined with costly retraining~\cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock, guo2023boost}. This is impractical for agile LLM inference, and the usage of a large mantissa field to preserve accuracy~\cite{jang2024figna, kim2023winning} leads to a large energy overhead.}

\rOneFC{In summary, processing
%involved with 
FP activations remains a major bottleneck in weight-only quantized LLM inference, and existing methods struggle to balance model accuracy, computational efficiency, and energy consumption.}
% \TODO{Please brainstorm how to reduce the redundancy from the following paragraphs to the contributions.} \rg{[The text know has non-overlapping technical info in both the main section and the bullet point, it's a good idea to reduce this. I would propose to keep the motivation and outline sentences in the section's full text, and fold all details into the bullet points.]}
% \as{I would completely merge the paragraphs below and the bullet points (except for maybe one or two very high-level sentences). I have made an attempt below.}
% % To overcome these limitations of the SotA, we propose Anda, a novel activation-oriented data format designed to directly replace FP16 without incurring any retraining overhead, which is important for LLMs due to their enormous training cost. 
% \rOneFC{To overcome these limitations of state-of-the-art (SotA) hardware, we propose Anda, a variable-length grouped data representation format tailored for FP activations \rg{[}, based on our key insight that FP activations exist \rg{[exhibit?]} substantial redundant information, varying across different LLM models and modules.}
% % Compared to the traditional FP16 data format, the Anda data type reduces both storage requirements and computational costs, due to its shared exponent and adjustable mantissa bit-width. Moreover, Anda allows a flexible trade-off between model accuracy and performance.
% % This adaptive, variable-mantissa-length format adjusts according to model sensitivities, yet remains transparent to users during execution, serving as a direct replacement for FP16 activation. 
% % \rOneFC{By dynamically adjusting data representation to minimize redundancy, Anda significantly reduces memory access overhead and computational complexity while maintaining model accuracy.
% % \rOneFC{Anda minimizes redundancy by dynamically adjusting data representation, significantly reducing memory access overhead and computational complexity while maintaining model accuracy.
% \rOneFC{Specifically, Anda employs online grouping of shared exponent and dynamic mantissa bit allocation strategies, greatly reducing storage and computational costs.} \rg{]}
% % \rOneFC{To fully realize Anda's potential, we develop complementary algorithms and hardware optimization techniques. These include a post-training adaptive precision search algorithm that determines the optimal Anda format for each module, striking a balance between model accuracy and computational efficiency.}
% \rOneFC{To unleash the full potential of Anda, we develop a suite of 
% complementary 
% optimization techniques from both algorithm and hardware perspectives.}
% % \rOneFC{These include a post-training adaptive precision search algorithm that determines the optimal Anda format for each module, striking a balance between model accuracy and computational efficiency.}
% % \rOneFC{Additionally, we propose hardware optimization techniques such as a bit-plane-based data organization scheme, processing units adapted to the Anda format, and an online bit-plane compression engine. 
% % These techniques collectively enable the efficient hardware deployment of LLMs, maximizing system performance and the benefits of the Anda format in practical applications.}
% \rg{[} \rOneFC{An adaptive precision search algorithm is proposed to determine the optimal Anda format for each module without retraining, balancing model accuracy and computational efficiency. 
% Furthermore, we introduce hardware optimizations, including a bit-plane-based data organization scheme, Anda-compatible bit-serial processing units, and a runtime bit-plane Anda compressor, collectively 
% % enabling efficient LLM hardware deployment and 
% maximizing the benefits of Anda for practical applications.} \rg{]}
% \rOneFC{Anda, as an innovative variable-length grouped activation data format, provides significant improvements in LLM inference efficiency by maintaining model accuracy while reducing computational and storage overheads.}
% % , providing a novel solution for efficient LLM deployment.}
% % In this work, we assess optimize, and demonstrate the benefits of the Anda data type in a complete system setting.
% \rg{More concretely,} Therefore, this paper makes the following contributions:
% \begin{itemize}
%     \item \rg{Based on our key observation that FP activations exhibit substantial redundant information, varying across different LLM models and modules,} We formalize \rg{[propose]} Anda,\rg{:} a variable-length data format \rg{[I think it is a good idea to describe what anda is in simple terms in this sentence, without all of the other adjectives. Let this sink in with the reader, then continue with the technical details]} \rg{. Anda...} with dynamically shared exponents and adjustable mantissa widths for activations, directly replacing FP16 activations and adapting to precision requirements across different LLM modules.
%     % \item We develop an efficient algorithm to identify optimal mantissa widths for various LLM modules within given accuracy tolerances, balancing model accuracy and efficiency.
%     \item \rOneFC{We develop an adaptive precision search algorithm to optimize mantissa widths for various LLM modules within given accuracy tolerances without retraining, balancing model accuracy, energy efficiency, and inference speed.}
%     % \item We design an Anda-compatible accelerator down to the RTL level, featuring 1.) an Anda-optimized memory layout, 2.) flexible widely-parallel dot-product computation units, and 3.) a runtime data compressor in the memory interface, significantly enhancing storage, memory access, and compute efficiency.
%     \item \rOneFC{We design an Anda-compatible accelerator down to the RTL level, featuring 1) a bit-plane-based memory layout scheme, 2) Anda-compatible bit-serial processing units, and 3) a runtime data compressor, significantly enhancing storage, computation, and memory access efficiency.}
%     % \item Extensive evaluation of the system-level energy and throughput savings from the Anda format across various LLMs shows ... 
%     \item \rOneFC{We conduct extensive evaluations of the Anda format across various LLMs, demonstrating an average speedup of 2.428$\times$ and a 2.062$\sim$3.148$\times$ improvement in energy efficiency compared to existing SotA solutions.}
% \end{itemize}
\as{
% To overcome the limitations of SotA hardware for LLM inference, 
% we propose Anda: a novel data format \rg{to replace} for FP activations with limited accuracy loss, combined with \rg{low-level hardware} optimizations at the hardware level to exploit its benefits. 
\rTwoFC{To overcome the above limitations, we propose Anda to unlock efficient LLM inference. Anda introduces a novel variable-length grouped activation data format, coupled with 
% an adaptive precision search algorithm 
\rTwoFC{the algorithm innovation}
and specialized hardware optimizations. As illustrated in Fig.~\ref{fig:anda_concept}, Anda first employs an adaptive precision combination search algorithm to determine optimal bit configurations across different LLM modules, considering user-desired accuracy requirements towards diverse LLM architectures and applications. It then leverages this optimized Anda format in conjunction with Anda-aware hardware architecture to efficiently replace FP16 activations during inference, achieving significant time-saving and energy-efficient LLM inference.}
More concretely, our contributions are as follows:
\begin{itemize}
    \item We investigate the potential of BFP activation quantization across popular LLM models within different modules. Based on these insights, we propose Anda: a variable-length grouped data format with shared exponents and adjustable mantissa widths for activations.
    \item We develop an adaptive search algorithm to optimize the mantissa widths for different LLM modules without retraining. 
    % This algorithm includes a tunable accuracy loss to balance model accuracy, energy efficiency and inference speed.
    \rTwoFC{This algorithm balances model accuracy, energy efficiency, and inference speed based on a user-defined accuracy loss tolerance.}
    \item We design 
    % an LLM accelerator 
    an efficient Anda-aware hardware architecture
    featuring (1) a bit-plane-based data layout scheme in~memory, (2) Anda-enhanced bit-serial processing units, and (3) a runtime bit-plane data compressor. 
    Extensive evaluations of the Anda system across popular LLMs demonstrate a 2.1$\sim$3.1$\times$ improvement in energy efficiency and an average speedup of 2.4$\times$ compared to existing SotA hardware.
    % We conduct extensive evaluations of the Anda format across popular LLMs, demonstrating a 2.0$\sim$3.1$\times$ improvement in energy efficiency and an average speedup of 2.4$\times$ compared to existing SotA hardware.
\end{itemize}
}

% \TODO{Attention! Rewrite this paper organization.}

The paper is organized as follows: Sec.~\ref{sec:bkg} reviews the~benefits and remaining bottlenecks of weight-only quantized~LLMs and BFP formats, and quantifies the sensitivity of LLM~inference accuracy to the shared exponents and reduced mantissas sizes. Based on these findings, Sec.~\ref{sec:algo} features the proposed Anda data format and presents the algorithm to rapidly optimize mantissa length under given accuracy constraints. Next, an Anda-optimized hardware architecture is proposed in Sec.~\ref{sec:arch}, which allows us to derive system-level gains in Sec.~\ref{sec:eval} and benchmark it against the SotA solutions. Sec.~\ref{sec:concls} concludes the paper.




==> archive/2-bkg-v0.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figs/LLM_blocks.png}
    \caption{Illustration of the architecture for a weight-only quantized LLM model.}
    % The blue boxes represent modules with quantized weights, while the green boxes denote modules that perform only floating-point operations. \mv{[and what is orange? I would add the meaning of the colors in the graph as a legend, rather than in the caption?]}}
    \label{fig:llm_blocks}
\end{figure}

\section{Background and Motivation}\label{sec:bkg}

% \begin{itemize}
%     \item Introduction of Transformer layers
%         \begin{itemize}
%             \item Transformer layers itself
%             \item Prefill stage: GEMM; Decode stage: GEMV + KV cache [Fig.~\ref{fig:3}]
%         \end{itemize}
%     \item Related works \rOneFC{[Chao: Maybe we need to move it to the last section? like QServe \cite{lin2024qserve}]} \rOneRG{I think this fits nicely here. We should definitely explain FIGNA.}
%         \begin{itemize}
%             \item Quantization of LLMs: Weight-only quantization, weight-activation quantization, KV cache quantization.
%             \item LLM-related accelerators
%         \end{itemize}
% \end{itemize}

\subsection{Weight-only Quantized LLMs}

% Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} in large language models (LLMs) is a crucial technique that reduces model size and computational complexity while maintaining performance, typically by converting FP16 numbers to lower-precision integers. Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}, which applies quantization solely to model weights while keeping activations in full precision, has gained popularity in the era of large models due to its simplicity, lower precision loss, and better hardware compatibility compared to weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3}. 

% Quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, lin2024awq, shao2024omniquant, frantar2023optq} in large language models (LLMs) is a crucial technique that reduces model size and computational complexity while maintaining performance, typically by converting 16-bit floating-point numbers to lower-precision integers. 
% The massive number of LLM parameters poses significant challenges to deploying LLM on resource-constrained devices. Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq}, compared to weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3}, substantially reduces memory overhead, thereby alleviating deployment platform costs while maintaining high model accuracy. 
% Its ease of adaptation to existing GPU platforms has led to widespread application and attention. 

% Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq} has become a widely adopted technique in large language models (LLMs), surpassing weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} in popularity.
Weight-only quantization~\cite{lin2024awq, shao2024omniquant, frantar2023optq} has become a widely adopted technique in deploying LLMs. 
Unlike weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3} which reduces precision for both model weights and activations, weight-only quantization focuses solely on compressing model parameters with a much more aggressive quantization scheme, which significantly reduces memory consumption, enabling the efficient deployment of LLMs on resource-constrained devices while maintaining high model accuracy. Consequently, weight-only quantization has become crucial in addressing the challenges posed by the massive number of LLM parameters.

% Fig.~\ref{fig:llm_blocks} illustrates the model architecture of a weight-only quantized LLM. 
% LLMs are composed of a series of Transformer blocks, each containing attention and feed-forward layers.
% The blue boxes in Fig.~\ref{fig:llm_blocks} represent the quantized weight matrices: query (Q), key (K), value (V), and output (O) in the attention Layer, and up-projection and down-projection matrices in the feed-forward layer. 
% These weight matrices dominate the storage requirements during LLM inference. 
% In a W4A16 quantized LLM, these weight matrices are quantized from FP16 to INT4, significantly reducing storage overhead, while the rest of the model computation remains in FP16. 
% As shown in Fig.~\ref{fig:llm_blocks}, the FP16 activations related to these weight computations are qkv\_proj, out\_proj, fc1, and fc2. Specifically, qkv\_proj computes with Q, K, and V weight matrices, out\_proj with the O weight matrix, and fc1 and fc2 with the up-projection and down-projection weight matrices, respectively. 
% This approach effectively balances model efficiency and performance, making weight-only quantized LLMs particularly suitable for deploying large language models in resource-constrained environments.

Fig.~\ref{fig:llm_blocks} illustrates the model architecture of a weight-only quantized LLM that is built from a series of Transformer blocks, each consisting of attention and feed-forward layers.
The blue boxes in Fig.~\ref{fig:llm_blocks} represent the quantized weight matrices: query (Q), key (K), value (V), and output (O) in the attention Layer, and up-projection and down-projection matrices in the feed-forward layer. 
For example, in the widely used W4A16 quantization scheme, these weight matrices are quantized from FP16 to INT4, which significantly reduces the storage overhead, while the remaining computations in the model are still performed in FP16.
In W4A16 quantized LLMs, FP-INT operations become the predominant computations during LLM inference. Specifically, the FP16 activations shown in the figure include qkv\_proj, out\_proj, fc1, and fc2, which are involved in computations with the quantized Q, K, V, and O weight matrices, as well as the up-projection and down-projection weight matrices, respectively.
Despite the significant storage efficiency gains achieved through INT4 weight quantization, the FP16 activations still contribute to a notable performance bottleneck in the FP-INT computations~\cite{huang2024isca}. \mv{Can I see this somewhere? If not, add a citation to prove this...}.

\subsection{Block Floating Point}

Reducing the computational overhead of FP16 activations is crucial for optimizing the efficiency of LLMs, and BFP~\cite{drumond2018training} strikes a balance between traditional floating-point and integer formats. 
By assigning a shared exponent to a group of values, BFP maintains dynamic range while simplifying computations, and as such achieves higher compression ratios than integer formats. % while \mv{avoiding significant accuracy losses}. %ensuring computational efficiency. 
However, like other quantization techniques, BFP may \mv{still} affect neural network accuracy. 
To address this, researchers have proposed two main approaches: \mv{On the one hand,} BFP-aware training \mv{fine tunes the network after quantization} \cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock}, \mv{at the expense of a} %which faces challenges of model-specific optimization and 
costly training process, making it \mv{rather} impractical for LLMs. \mv{On the other hand,} direct conversion of pre-trained floating-point models to BFP formats~\cite{dai2021vs, keller202395, jang2024figna, kim2023winning}, significantly reduces deployment costs, \mv{but requires long mantissa lengths to avoid serious degradations in} model performance, as \mv{e.g. observed in the} VS-Quant \mv{scheme}~\cite{dai2021vs, keller202395}). 
\mv{To avoid the storage of these long mantissa lengths}, methods like FIGNA~\cite{jang2024figna, kim2023winning} propose dynamic conversion to BFP during computation. \mv{This allows them to store the activation data in memory in the traditional FP16 data format, while expanding to long mantissa lengths and shared exponents right before computations. As such, FIGNA} preserves numerical precision comparable to floating-point calculations and maintains model performance. \mv{However, this also prevents FIGNA to obtain activation memory footprint savings, or significant computational savings.} %but sacrifices some potential computational gains. 

%In the era of LLMs, the cost of retraining before deployment is prohibitively high; therefore, 
\mv{To avoid both costly retraining, as well as large activation footprints,} we seek a solution that can rapidly convert FP activations to BFP activations \mv{without retraining}, while also leveraging the computational and storage advantages of BFP \mv{for LLM inference}. % to achieve efficient LLM inference deployment.
To achieve this goal, it is necessary to explore opportunities for \mv{reduced mantissa length BFP under the} %simplifying FP16 activation computations by leveraging the 
unique characteristics of LLMs.


% \subsection{Challenges towards Activations in W4A16 quantized LLMs}

% % Due to significant reduced storage requirements, W4A16 quantized LLMs have been widely deployed on GPU devices. 
% % Within LLMs, both linear layers and attention mechanisms rely on general matrix multiplication (GEMM) operations, with the key distinction being the operands involved. 
% % Linear layers perform GEMM between weights and activations, while attention mechanisms compute GEMM between different activation matrices. 
% % Fig.~\ref{fig:fp_int} illustrates the relative distribution of operations for various W4A16 LLMs across different token lengths in text generation tasks. 
% % Notably, FP-INT operations consistently dominate, accounting for over 90\% of the total computational workload across all models and scenarios examined. 
% % This overwhelming prevalence underscores the critical importance of optimizing FP-INT GEMM operations to achieve efficient inference deployment for W4A16 LLMs. 
% % Consequently, our optimization efforts are primarily focused on enhancing the performance of these FP-INT GEMM operations, as they represent the most significant bottleneck in the inference process.

% % \begin{figure}[htbp]
% %     \centering
% %     % \subfigure[]{%
% %     \includegraphics[width=0.92\columnwidth]{figs/energy_weight_act.png}
% %     % }\hfill
% %     % \subfigure[]{%
% %     %     \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
% %     %     \label{fig:subfig2}
% %     % }\vskip\baselineskip
% %     % \caption{Energy distribution in Llama2-7B model on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations. \rOneFC{[Chao: Robin, I think here we show llama-7b is enough, since our experiment will not cover gpt-175b. Maybe we can also remove the attention parts, i.e., Q*K$^{T}$ and S*V because we focus on FP-INT operations. Or we can split the Linear operations into qkv\_proj, out\_proj, and denote MLP as fc, like Fig.~\ref{fig:value_dist_wrt_addi_bits}, and merge Q*K$^{T}$ and S*V into the others to show the dominated energy consumption of FP-INT operations.]}}
% %     \caption{Energy distribution of various LLM models on a typical cloud accelerator.}
% %     \label{fig:zigzag}
% % \end{figure}

% % \begin{figure}[htbp]
% %     \centering
% %     \includegraphics[width=0.92\columnwidth]{figs/memory_consumption.png}
% %     \caption{Relative memory consumption.}
% %     \label{fig:mem_consumption}
% % \end{figure}

% For linear layers with INT4-quantized weights (Q, K, V, O, up projection, down projection), current GPUs lack specialized computational units, necessitating a process where INT4 weights are loaded into GPU memory and converted to FP16 before computation with FP16 activations. This approach incurs additional computational overhead. To enhance FP-INT operations, FINGA initially explored dedicated floating-point units for FP-INT computations. However, while this effectively reduced multiplier complexity, the alignment and normalization operations in floating-point units still consumed significant area and power, resulting in only 22\% and 26\% savings for FP16-INT4 specialized hardware units, respectively.

% To further reduce computational costs, FINGA leverages block floating-point (BFP) format, converting complex floating-point multiplications to INT multiplications. However, to maintain numerical precision, FINGA still uses FP16 format for storage, decompressing to INT format before computation, and expanding the mantissa. This approach, while beneficial, somewhat impacts computational efficiency.
% Moreover, in W4A16 LLM inference, although weight storage costs are significantly reduced, activation storage remains substantial. Crucially, in terms of inference energy consumption, we found that accessing activation data in LLM inference is more costly than accessing unit weights, and activations are frequently read during computations. Consequently, memory access for activation data accounts for a significant, non-negligible portion of energy consumption.
% This insight reveals that optimizing FP-INT GEMM by solely reducing FP-INT computational costs at the computation level is insufficient. A more comprehensive approach, considering both memory access and computation aspects simultaneously, is necessary to achieve more substantial benefits. This realization guides our strategy towards a holistic optimization of W4A16 LLM inference, addressing both computational efficiency and memory access patterns to maximize performance gains and energy efficiency.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs/shared_exp_eval_fp_int_merged.pdf}
    \caption{Group Size (\mv{GS}) Impact. \mv{[I would find it better to on all plots use the actual mantissa bits on the x-axis and not the number of cut bits. this is too relative and not insightful. I can cut 20bits if I start from FP32...]}}
    \label{fig:acc_wrt_gs}
\end{figure}

\subsection{Opportunities towards Activation Optimizations}

%FIGNA's approach to introducing BFP computations in W4A16 LLMs involves expanding the mantissa to maintain precision, which introduces additional computational overhead. 
%Questioning the necessity of this expansion, we explore reducing mantissa length in BFP formats across different group sizes. 
%This intuition stems from neural network computation redundancy and model robustness to minor precision changes. 

\mv{To explore the sensitivity of LLMs to reduced mantissa lengths in BFP formats across different group sizes \mv{[Where do I see the impact across group sizes? Figure 3 does not seem to be referenced? ?]},} we first replace all activations of the different FP-INT GEMM operations, being the qkv\_proj, o\_proj, fc1, and fc2 \mv{(see Fig.2)} with the BFP format \mv{with a parametrized group size and mantissa length}, and observe the model's perplexity (PPL) \mv{to assess the accuracy impact}.

\mv{\textbf{Sensitivity to group size:} Fig.~\ref{fig:acc_wrt_gs} shows the sensitivity to the shared exponent group size for two different LLM models across a wide range of mantissa lengths. The experiment shows a clear trade-off between the group size, and the minimally required mantissa length.} Larger activation group sizes allow more efficient \mv{parallel} computations, yet at a greater precision cost \mv{or increased mantissa lengths}. Based on the observations, we chose a group size of 64 for subsequent exploration, as it provides a good balance between computational efficiency, hardware compatibility, and precision loss.
%This trade-off between computational efficiency and model accuracy provides crucial insights for optimizing LLM deployment strategies.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/acc_wrt_mbits_gs64.pdf}
    % \caption{The relative accuracy when uniformly cutting mantissa bits on 9 popular LLMs.}
    \caption{The relative accuracy to mantissa reduction across various LLMs. \mv{[Always put figures at paper top of bottom, rather than not in the text.]}}
    \label{fig:acc_wrt_mbits}
\end{figure}

\mv{\textbf{Sensitivity to LLM variant:} With this group size of 64, we continue our exploration across a wider range of recent LLMs, to derive their sensitivity to reduced mantissa lengths.} %Fig.~\ref{fig:acc_wrt_mbits} shows, LLMs maintained good PPL, sufficient for normal deployment even without mantissa expansion and with some reduction. 
%After determining the BFP group size, we conducted experiments on reducing mantissa lengths across several popular LLM models. 
As shown in Fig.~\ref{fig:acc_wrt_mbits}, different LLms exhibit varying sensitivities to mantissa reduction. %we explored the impact of mantissa reduction on model accuracy across different models. 
Assuming a 1\% accuracy loss tolerance in practical deployment scenarios, we observed that models \mv{such as} opt-6.7b, opt-13b, and opt-30b were less sensitive to mantissa reduction, allowing for the direct removal of 5 mantissa bits, while other models could only tolerate the removal of 4 mantissa bits. Furthermore, as more mantissa bits were removed, we observed more pronounced differences in accuracy sensitivity among different models. This insight inspires us to consider \mv{a variable length BFP datatype,} %model-specific optimization strategies for BFP conversion, 
potentially allowing for more aggressive compression in less sensitive models while maintaining a more conservative approach for others. \mv{This moreover raised the question whether there is also a difference in sensitivities among different tensors within one LLM.} %It also suggests the possibility of developing adaptive BFP schemes that adjust mantissa lengths based on each model's specific characteristics and requirements, thereby maximizing both efficiency and accuracy in LLM deployment. 
\mv{[I have cut quite some sentences in previous paragraph, and you still had quite some redudant messages...]}

\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figs/module_wise_acc_gs64.pdf}
    \caption{The relative accuracy of OPT-6.7B, LLaMA-7B, and LLaMA-2-7B when cutting mantissa bits on qkv\_proj, o\_proj, fc1, and fc2 modules only.}
    \label{fig:module_wise_acc}
\end{figure}

\textbf{Sensitivity to tensor type:} We \mv{finally} explore the impact of different mantissa lengths \mv{across various tensors within the same model. This information allows to derive whether it makes sense to use different mantissa lengths across the activation outputs of the} qkv\_proj, out\_proj, fc1, and fc2 \mv{modules of a network}. %As shown in Fig. 1, these activations participate in computations with different INT4 quantized weight network layers. Converting these activations to BFP computations leads to accumulated numerical errors, ultimately affecting model accuracy. 
We \mv{therefore} examine opt-6.7b, llama-7b, and llama-2-7b models, \mv{individually sweeping} the mantissa \mv{length of each type of} activations to observe their \mv{individual sensitivity to} model accuracy. \mv{[Make it clear what length you use for the other tensors while you sweep one of them...]]}
Fig.~\ref{fig:module_wise_acc} \mv{summarizes the results, revealing} that activations from different modules \mv{indeed} have varying impacts on model accuracy across all three models. qkv\_proj consistently shows the most significant influence, while fc2 demonstrates low sensitivity in opt-6.7b but has a more pronounced effect in the llama series models.


% Our three sets of experiments reveal crucial insights into BFP application in LLMs. First, we find that LLMs can maintain good performance with reduced mantissa lengths, challenging the need for full-precision computations. Second, different LLM models show varying sensitivities to mantissa reduction, suggesting the potential for model-specific optimizations. Third, within a single model, different modules exhibit distinct sensitivities to precision reduction. These findings highlight limitations in traditional BFP designs, which use fixed mantissa lengths across all modules and models. In response, we propose a novel BFP design that employs variable-length mantissas tailored to the specific characteristics of each model and module. This approach allows for more efficient utilization of computational resources and storage, potentially leading to improved inference speed and reduced memory footprint without significant accuracy loss. Furthermore, this adaptive BFP strategy enables fine-grained optimization of LLM deployments, balancing performance and efficiency in a more nuanced manner than traditional fixed-precision approaches. By leveraging these model-specific and module-specific insights, our proposed BFP design paves the way for more efficient and adaptable LLM inference deployments across a wide range of applications and hardware configurations.

Our experiments reveal key insights into BFP application in LLMs: 1) LLMs maintain good performance with reduced mantissa lengths. 2) Different LLM models have varying sensitivities to mantissa reduction. 3) Within an LLM, different modules show distinct sensitivities to precision reduction.
These observations inspire us to \mv{introduce the new Anda data format, together with an methodology for post-training quantization, and rapid selection of the tolerable reduced mantissa lengths for any LLM. These will be introduced in the next section.} %pre-measure the sensitivity of different module activations to model accuracy. This insight enables efficient allocation of mantissa widths across modules during deployment, optimizing storage and computation while maintaining model performance.

%Traditional BFP designs, using fixed mantissa lengths, have limitations. We propose Anda BFP, employing variable-length mantissas tailored to each model and module. This approach improves efficiency, potentially increasing inference speed and reducing memory usage without significant accuracy loss. Anda BFP enables fine-grained optimization of LLM deployments, balancing performance and efficiency better than fixed-precision approaches.



==> archive/2-bkg.tex <==
\section{Background and Motivation}\label{sec:bkg}

\subsection{Weight-only Quantized LLMs}

% Weight-only quantization~\cite{park2024lutgemm, dettmers2023case, chee2024quip, lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit} has become a widely adopted technique for efficient LLM deployment. 
% Unlike weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, xiao2023smoothquant, zhao2024atom} which reduces precision for both model weights and activations, weight-only quantization focuses solely on compressing model parameters with a much more aggressive quantization scheme, which significantly reduces memory consumption, enabling the efficient deployment of LLMs on resource-constrained devices while maintaining high model accuracy. Consequently, weight-only quantization has become crucial in addressing the challenges posed by the massive number of LLM parameters.
% \rOneFC{Weight-only quantization~\cite{park2024lutgemm, dettmers2023case, chee2024quip, lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit} has emerged as a pivotal technique for efficient LLM inference. Unlike weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, xiao2023smoothquant, zhao2024atom}, which reduces precision for both weights and activations, weight-only quantization focuses solely on compressing model parameters with a much more aggressive quantization scheme, which constitute the vast majority of an LLM's storage requirements.}
% \rOneFC{By dramatically reducing the bits needed to represent weights, this method significantly decreases overall memory consumption while maintaining model accuracy, enabling LLM deployment on resource-constrained devices.}
% \rOneFC{This approach allows for aggressive weight quantization, significantly reducing memory consumption while preserving accuracy. As a result, it enables LLM deployment on resource-constrained devices without performance loss.}

\rOneFC{Weight-only quantization~\cite{park2024lutgemm, dettmers2023case, chee2024quip, lin2024awq, shao2024omniquant, frantar2023optq, li2024norm, jeon2022mr, jeon2020biqgemm, xia2024fp6, xu2024onebit} has emerged as a pivotal technique for efficient LLM inference.}
\rOneFC{Unlike weight-activation quantization~\cite{dai2021vs, lin2024qserve, dettmers2022gpt3, xiao2023smoothquant, zhao2024atom}, which reduces precision for both weights and activations, weight-only quantization focuses solely on compressing model parameters using a much more aggressive quantization scheme.}
\rOneFC{This approach addresses the predominant storage requirements of LLMs, thereby enabling LLM deployment on resource-constrained devices while maintaining model accuracy~\cite{nvidia2024cutlass,shao2024omniquant}.}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.96\linewidth]{figs/LLM_blocks.pdf}
    \caption{Illustration of the architecture for a weight-only quantized LLM model.}
    \label{fig:llm_blocks}
\end{figure}

\rOneFC{Fig.~\ref{fig:llm_blocks} illustrates the architecture of a weight-only quantized LLM, composed of a series of Transformer blocks that each contains an attention layer and a feed-forward layer.}
\rOneFC{The light blue background highlights the dominant computational modules involving FP-INT GeMM operations of weight-only quantized LLMs.}
\rOneFC{The dark blue blocks represent the quantized INT weights, while the orange arrows indicate the FP activations.}
\rOneFC{As shown in Fig.~\ref{fig:llm_blocks}, these FP-INT GeMM operations can be categorized into four module types based on the positions of the FP activations: the first type involves $A_{qkv}$ interacting with $W_q$, $W_k$, and $W_v$ to compute the query ($Q$), key ($K$), value ($V$) matrices, respectively; the second type involves $A_o$ multiplying with $W_o$ to compute the output matrix;}
\rTwoFC{the other two types are up-projection and down-projection modules of the feed-forward layer, respectively, involving $A_u$ and $A_d$ with interacting to corresponding weights.}
% the other two types involve $A_u$ and $A_d$ interacting with the weights in the up projection and down projection modules of the feed-forward layer, respectively.}
% The blue boxes in Fig.~\ref{fig:llm_blocks} represent the quantized weight matrices: query ($Q$), key ($K$), value ($V$), and output ($O$) in the attention Layer, and up-projection ($U$) and down-projection ($D$) matrices in the feed-forward layer. 
% For example, in the widely used W4A16 quantization scheme~\cite{nvidia2024cutlass,lin2024awq,shao2024omniquant,jang2024figna}, these weight matrices are quantized from FP16 to INT4, which significantly reduces the storage overhead, while the remaining computations in the model are still performed in FP16.
% In W4A16 quantized LLMs, FP-INT operations become the predominant computations during LLM inference~\cite{jang2024figna, kim2023winning}. Specifically, the FP16 activations shown in Fig.~\ref{fig:llm_blocks} include $A_{qkv}$, $A_{o}$, $A_{u}$, and $A_{d}$, which are involved in computations with the quantized Q, K, V, and O weight matrices, as well as the up-projection and down-projection weight matrices, respectively.
% Despite the significant storage efficiency gains achieved through INT4 weight quantization, the FP16 activations still contribute to a notable performance bottleneck in the FP-INT computations~\cite{huang2024isca, yuan2024llm}. 
% \rOneFC{Despite the significant storage efficiency gains, FP activations remain a critical performance bottleneck of weight-only quantized LLMs.}
% \rOneFC{Compared to INT weights, accessing FP activations for FP-INT GeMMs incurs higher energy costs, and FP-INT operations require more complicated hardware implementations.}

\rOneFC{Despite the significant storage efficiency gains of weight-only quantized LLMs, to perform FP-INT GeMMs, accessing FP activations incurs higher energy costs than INT weights~\cite{huang2024isca}, and FP-INT operations require complicated hardware implementations~\cite{jang2024figna}.}
\rOneFC{Hence, optimizing FP activations emerges as a key opportunity to improve the overall efficiency of weight-only quantized LLMs.}
% \mv{Can I see this somewhere? If not, add a citation to prove this...}.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.96\linewidth]{figs/fp_bfp_convert_process.pdf}
    \caption{The process of converting a set of FP16 numbers into different BFP numbers. BFP format is regulated by two key parameters: group size (GS) and mantissa length (M).}
    % \as{Are the mantissa bits in case 2 of correct length?}}
    \label{fig:fp_bfp_convert_process}
    % \vspace{-1em}
\end{figure}

\subsection{Block Floating Point}

Reducing the computation and storage overhead of FP16 activations is crucial for optimizing the efficiency of LLMs.
% BFP~\cite{drumond2018training} strikes an ingenious balance between conventional FP and INT numbers.
% \rOneFC{BFP~\cite{drumond2018training} offers a promising solution by balancing the advantages of FP and INT formats. By sharing exponents within groups of values, BFP preserves dynamic range while mitigating the impact of outliers and simplifying computations.}
\rOneFC{BFP~\cite{drumond2018training} offers a promising solution by sharing exponents within groups of values, preserving dynamic range while mitigating the impact of outliers and simplifying computations.}
\rOneFC{The BFP format can characterized by two key parameters: group size and mantissa length.}
\rOneFC{Fig.~\ref{fig:fp_bfp_convert_process} shows the process of converting FP16 tensors to BFP numbers using two different instances of the BFP format.}
\rOneFC{Initially, FP16 tensors are divided into groups. Within each group, the largest exponent is selected as the shared exponent and other mantissas are right-shifted based on their exponent differences. Bits exceeding the specified mantissa length are truncated, and zero is represented by all mantissa bits being 0.}
% \rOneFC{Notably, this process can lead to precision loss, as evidenced in Fig.~\ref{fig:fp_bfp_convert_process}, where some elements become zero due to mantissa truncation. This precision loss poses a significant challenge to maintaining model accuracy.}
\rOneFC{As illustrated in Fig.~\ref{fig:fp_bfp_convert_process}, this conversion process can lead to precision loss due to mantissa truncation, with some elements becoming zero, thereby posing a significant challenge to maintaining model accuracy.}

% \rOneFC{It not only preserves dynamic range but also simplifies computations while mitigating the impact of outliers. By sharing exponents, BFP effectively reduces both storage and computational costs.}
% By assigning a shared exponent to a group of values, BFP maintains dynamic range while simplifying computations, and as such achieves higher compression ratios than integer formats. % while \mv{avoiding significant accuracy losses}. %ensuring computational efficiency. 
% However, like other quantization techniques, BFP may \mv{still} affect neural network accuracy. 
\rOneFC{Current approaches to address this fall into two categories.}
% To address this, researchers have proposed two main approaches: 
On the one hand, BFP-aware training fine-tunes the model after the quantization~\cite{dai2021vs, darvish2023shared, darvish2020pushing, keller202395, zhang2022fast, koster2017flexpoint, noh2023flexblock, guo2023boost, kim2024isca, fan2019static}, at the expense of a
costly training process, making it rather impractical for agile LLM deployment. 
% \TODO{On the other hand, direct conversion of pre-trained FP models to BFP formats~\cite{dai2021vs, keller202395, jang2024figna, kim2023winning, fan2018reconfigurable, lian2019high} reduces deployment costs but faces a dilemma \rg{trade-off}: short mantissa lengths lead to performance degradation, as observed in VS-Quant~\cite{dai2021vs, keller202395}, while long mantissas increase computation and storage overhead, diminishing the advantages of BFP.}
% \rTwoFC{On the other hand, direct conversion of pre-trained FP models to BFP formats~\cite{fan2018reconfigurable, lian2019high, koster2017flexpoint, fan2019static, noh2023flexblock} requires long mantissas to maintain accuracy, which increases computation and storage overhead, since using short mantissas results in significant accuracy loss.}
\rTwoFC{On the other hand, direct conversion of pre-trained FP models to BFP formats~\cite{fan2018reconfigurable, lian2019high, koster2017flexpoint, fan2019static, noh2023flexblock} requires long mantissas to avoid the significant accuracy loss, which increases computation and storage overhead, diminishing the advantages of BFP.}
\rOneFC{To avoid the storage of these long mantissas, methods like FIGNA~\cite{jang2024figna} and~\cite{kim2023winning} propose dynamic conversion to BFP during computation.
This approach stores activations in FP16 format and expands to long mantissas with shared exponents before computations to maintain model accuracy.}
However, this also prevents FIGNA from obtaining activation memory footprint savings.

To avoid both costly retraining and large activation memory footprints, we seek a solution that can rapidly convert FP activations to BFP activations without retraining, while also leveraging the computational and storage advantages of BFP for LLM inference.
To achieve this goal, it is necessary to explore opportunities for reduced mantissa length BFP under the unique characteristics of LLMs.

\subsection{Opportunities towards Activation Optimizations}

% \rOneFC{We explore opportunities for LLM activation optimization by systematically investigating the sensitivity of model accuracy to reduced mantissa lengths in BFP formats.}
% \rOneFC{This study converts the activation tensors of FP-INT GeMM operations, including $A_{qkv}$, $A_{o}$, $A_{u}$, and $A_{d}$, directly from FP16 to BFP format for computation, as illustrated in Fig.~\ref{fig:fp_bfp_convert_process}.}
% \rOneFC{Model accuracy is evaluated using perplexity (PPL) on the wikitext2 dataset, with lower PPL indicating higher accuracy.}
% \rOneFC{While the first set of experiments uses absolute PPL, for ease of comparison in subsequent experiments, we uniformly adopt relative accuracy as our metric.}
% \rOneFC{Through this approach, we aim to uncover the potential for more efficient activation representations while maintaining LLM performance.}

% \rOneFC{We explore LLM activation optimization by systematically investigating the sensitivity of model accuracy to reduced mantissa lengths in BFP formats. This study converts FP-INT GeMM activation tensors, including $A_{qkv}$, $A_{o}$, $A_{u}$, $A_{d}$, directly from FP16 to BFP format for computation, as shown in Fig.~\ref{fig:fp_bfp_convert_process}. Model accuracy is evaluated using perplexity (PPL) on the wikitext2 dataset, with lower PPL indicating higher accuracy. Assuming a 1\% accuracy loss tolerance in practical deployment scenarios, we examine various BFP configurations. While our initial set of experiments uses absolute PPL values, for ease of comparison across different settings, subsequent experiments uniformly adopt relative accuracy as the metric. Through this comprehensive approach, we aim to uncover the potential for more efficient activation representations while carefully maintaining LLM performance within acceptable limits.}

\rOneFC{We explore opportunities for LLM activation optimization by investigating the sensitivity of model accuracy to reduced mantissa lengths in BFP formats. This study converts FP-INT GeMM activation tensors ($A_{qkv}$, $A_{o}$, $A_{u}$, $A_{d}$) from FP16 to BFP format, as shown in Fig.~\ref{fig:fp_bfp_convert_process}. Model accuracy is evaluated using perplexity (PPL) on the wikitext2 dataset, with lower PPL indicating higher accuracy. We assume a 1\% accuracy loss tolerance in practical scenarios. 
% While initial experiments use absolute PPL, subsequent ones adopt relative accuracy for ease of comparison across different settings. 
We aim to uncover efficient activation representations while maintaining LLM performance within acceptable limits.}

% \mv{To explore the sensitivity of LLMs to reduced mantissa lengths in BFP formats across different group sizes \mv{[Where do I see the impact across group sizes? Figure 3 does not seem to be referenced? ?]},} we first replace all activations of the different FP-INT GEMM operations, being the $A_{qkv}$, $A_{o}$, $A_{u}$, and $A_{d}$ \mv{(see Fig.2)} with the BFP format \mv{with a parametrized group size and mantissa length}, and observe the model's perplexity (PPL) \mv{to assess the accuracy impact}.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/shared_exp_eval_fp_int_merged.pdf}
    % \caption{Group Size (\mv{GS}) Impact.}
    \caption{LLM sensitivity to BFP group size (GS) and preserved mantissa bits.}
    % \mv{[I would find it better to on all plots use the actual mantissa bits on the x-axis and not the number of cut bits. this is too relative and not insightful. I can cut 20bits if I start from FP32...]}}
    \label{fig:acc_wrt_gs}
\end{figure}


\mv{\textbf{Sensitivity to group size:}} 
% Fig.~\ref{fig:acc_wrt_gs} shows the sensitivity to the shared exponent group size for two different LLM models across a wide range of mantissa lengths. The experiment shows a clear trade-off between the group size, and the minimally required mantissa length.} Larger activation group sizes allow more efficient \mv{parallel} computations, yet at a greater precision cost \mv{or increased mantissa lengths}. 
\rOneFC{Fig.~\ref{fig:acc_wrt_gs} illustrates the sensitivity to shared exponent group size for two different LLM models across various mantissa lengths. The experiments reveal a clear trade-off between group size and the minimum required mantissa length to maintain model accuracy.}
\rOneFC{Larger activation group sizes allow more efficient parallel computations, yet at a greater accuracy tolerance or increased mantissa lengths.}
\rOneFC{Based on these observations, we select a group size of 64 for subsequent experiments, as it offers a good balance between computational efficiency and accuracy tolerance.}


\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figs/acc_wrt_mbits_gs64.pdf}
    % \caption{The relative accuracy when uniformly cutting mantissa bits on 9 popular LLMs.}
    % \caption{The relative accuracy to mantissa reduction across various LLMs.}
    \caption{The relative accuracy to preserved mantissa bits across various LLMs.}
    % \mv{[Always put figures at paper top of bottom, rather than not in the text.]}}
    \label{fig:acc_wrt_mbits}
\end{figure}

\mv{\textbf{Sensitivity to LLM model:}} With this group size of 64, we continue our exploration across a wider range of recent LLMs, to derive their sensitivity to reduced mantissa lengths.
\rOneFC{Fig.~\ref{fig:acc_wrt_mbits} reveals varying sensitivities among different models.}
Notably, models such as OPT-2.7B, OPT-6.7B, OPT-13B, and OPT-30B are less sensitive to mantissa reduction, allowing for the direct removal of 5 mantissa bits, while other models could only tolerate the removal of 4 mantissa bits. 
% Furthermore, as more mantissa bits are removed, we observe more pronounced differences in accuracy sensitivity among different models. 
\rOneFC{As more mantissa bits are removed, differences in accuracy sensitivity become more pronounced.}
This insight inspires us to consider a variable-length BFP datatype, potentially enabling more aggressive compression in less sensitive models while employing a more conservative one for others. 
\rOneFC{It also prompts us to explore whether activations in different modules within one LLM have varying sensitivities.}
% Moreover, this raises the question of whether there is also a difference in sensitivities among different activation tensors within one LLM.

\mv{\textbf{Sensitivity to LLM inner module:}}
% We \mv{finally} explore the impact of different mantissa lengths \mv{across various tensors within the same model. This information allows us to derive whether it makes sense to use different mantissa lengths across the activation outputs of the} $A_{qkv}$, $A_{o}$, $A_{u}$, and $A_{d}$ \mv{modules of a network}. 
% We \mv{therefore} examine opt-6.7b, llama-7b, and llama-2-7b models, \mv{individually sweeping} the mantissa \mv{length of each type of} activations to observe their \mv{individual sensitivity to} model accuracy. \mv{[Make it clear what length you use for the other tensors while you sweep one of them...]]}
% Fig.~\ref{fig:module_wise_acc} \mv{summarizes the results, revealing} that activations from different modules \mv{indeed} have varying impacts on model accuracy across all three models. $A_{qkv}$ consistently shows the most significant influence, while $A_{d}$ demonstrates low sensitivity in opt-6.7b but has a more pronounced effect in the llama series models.
\rOneFC{We finally explore the impact of different mantissa lengths of the activations of different modules within the same LLM. More specifically, we examine the $A_{qkv}$, $A_{o}$, $A_{u}$, and $A_{d}$ modules of the OPT-6.7B, LLaMA-7B, and LLaMA2-7B models. The mantissa length of each module is swept while keeping the lengths of other modules fixed at 13 bits. Fig.~\ref{fig:module_wise_acc} summarizes the results, revealing that activations from different modules have varying impacts on model accuracy across all three models. $A_{qkv}$ consistently shows the most significant influence, while $A_{d}$ demonstrates low sensitivity in OPT-6.7B but has a more pronounced effect in the LLaMA series models.}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figs/module_wise_acc_gs64.pdf}
    \caption{The relative accuracy of OPT-6.7B, LLaMA-7B, and LLaMA2-7B when cutting mantissa bits on either $A_{qkv}$, $A_{o}$, $A_{u}$, or $A_{d}$ activation only.}
    \label{fig:module_wise_acc}
\end{figure}

\rOneFC{Our study reveals several key insights into the application of BFP in LLMs:
1) LLMs can maintain good performance with reduced mantissa lengths. 
2) Different LLM models exhibit varying sensitivities to mantissa reduction. 
3) Within a single LLM, different modules have distinct sensitivities to precision reduction.
These observations motivate us to introduce the new variable-length grouped data format for FP activations, along with a methodology for post-training quantization and rapid selection of tolerable reduced mantissa lengths for any LLM.}
% \TODO{This last paragraph could be removed and the key insights could be put in bold in the previous paragraphs to save space.}
% The details of this approach will be introduced in the next section.}

% Our experiments reveal key insights into BFP application in LLMs: 1) LLMs maintain good performance with reduced mantissa lengths. 2) Different LLM models have varying sensitivities to mantissa reduction. 3) Within an LLM, different modules show distinct sensitivities to precision reduction.
% These observations inspire us to \mv{introduce the new Anda data format, together with a methodology for post-training quantization, and rapid selection of the tolerable reduced mantissa lengths for any LLM. These will be introduced in the next section.} 
%pre-measure the sensitivity of different module activations to model accuracy. This insight enables efficient allocation of mantissa widths across modules during deployment, optimizing storage and computation while maintaining model performance.



==> archive/2.1-motivation.tex <==
\section{Motivation}\label{sec:motiv}

\rOneRG{[Goal: 1) show that in weight-only quantization, the activations take the majority of the energy. 2) weigt*act $>>$ act*act 3) mention we do only prefill + give arguments   ]}

Weight-only quantization alleviates the enormous storage requirements for contemporary LLMs, but it does not address the requirement of high energy-efficiency posed by edge computation environments. In order to gain insight into the energy bottlenecks, we simulate the performance of two well-known LLMs on a generalized but representative hardware architecture, for cloud and edge scenarios. By using a generalized architecture, the results conclusions with regards to energy bottlenecks are widely applicable. 

% HW info
The architecture is shown in Figure \ref{fig:generic-arch}. The cloud and edge accelerator have the same layout, but different dimensions and parameters. For the cloud scenario, the architecture is identical to the one used by \rOneRG{FLAT paper} for similar modelling purposes. To prevent becoming lost in the details, we generalize the energy cost of hardware transactions to a representative order of magnitude, given in Table \ref{tab:energy-cost}. \rOneRG{The values are justified by ...}

% Model info
The models chosen for simulation are Llama1-7B and GPT3-175B. We use a realistic batch size of 8 and only simulate the pre-fill phase, since this phase is the most energy intensive \rOneRG{[Is this the case?]}. The sequence length is set to half of the maximal context window. The tool used for simulation is ZigZag \rOneRG{[Cite, more info]}. The layers are mapped in an output-stationary way onto the architecture.

The simulation results are shown in Figrue \ref{fig:zigzag}. The figure show the total energy cost of a single inference of the LLM for the five major modules. Other modules such the non-linear operations or (de-)tokenization are omitted for simplicity. The energy costs are further categorized according to the type (compute or memory access at different levels) and the operand. The two main conclusions are that 1) the modules that embody weight $\times$ activation operations (and benefit from weight-only quantization) are dominant in terms of energy and 2) the data movement of the high-precision activations is the main contributor to the overall energy cost. \rOneRG{[This is not the case for the edge platform!]} Therefore, optimizing and compressing FP activations is necessary for achieving high-energy-efficient LLM inference deployment on edge devices.


% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{Hardware diagram of the target platform to model LLM inference.}
%     \label{fig:generic-arch}
% \end{figure}

% \begin{table}[h!]
%     \centering
%     \caption{Energy costs assumed in generic hardware architecture}
%     \begin{tabular}{lcc}
%         \toprule
%         \textbf{Energy cost per bit [pJ/bit]} & \textbf{Cloud scenario} & \textbf{Edge scenario} \\
%         \midrule
%         Off-chip DRAM read  & 10    & 10    \\
%         Off-chip DRAM write & 15    & 15    \\
%         On-chip SRAM read   & 1     & 1     \\
%         On-chip SRAM write  & 1.5   & 1.5   \\
%         Register file read  & 0.01  & 0.01  \\
%         Register file write & 0.015 & 0.015 \\
%         MAC operation       & 0.01  & 0.01  \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:energy-cost}
% \end{table}

\begin{figure}[htbp]
    \centering
    \subfigure[Subfigure 1]{%
        \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array.png}
        \label{fig:subfig1}
    }\hfill
    \subfigure[Subfigure 2]{%
        \includegraphics[width=0.48\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
        \label{fig:subfig2}
    }\vskip\baselineskip
    % \subfigure[Subfigure 3]{%
    %     \includegraphics[width=0.48\columnwidth]{figs/GPT3-175B_B=8_generic_array.png}
    %     \label{fig:subfig3}
    % }\hfill
    % \subfigure[Subfigure 4]{%
    %     \includegraphics[width=0.48\columnwidth]{figs/GPT3-175B_B=8_generic_array_edge.png}
    %     \label{fig:subfig4}
    % }
    \caption{Energy distribution in Llama1-7B and GPT3-175B models on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations. \rOneFC{[Chao: Robin, I think here we show llama-7b is enough, since our experiment will not cover gpt-175b. Maybe we can also remove the attention parts, i.e., Q*K$^{T}$ and S*V because we focus on FP-INT operations. Or we can split the Linear operations into qkv\_proj, out\_proj, and denote MLP as fc, like Fig.~\ref{fig:value_dist_wrt_addi_bits}, and merge Q*K$^{T}$ and S*V into the others to show the dominated energy consumption of FP-INT operations.]}
}
    \label{fig:zigzag}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \subfigure[]{%
%         \includegraphics[width=0.9\columnwidth]{figs/Llama1-7B_B=8_generic_array.png}
%         % \label{fig:subfig1}
%     }\hfill
%     \subfigure[Subfigure 2]{%
%         \includegraphics[width=0.9\columnwidth]{figs/Llama1-7B_B=8_generic_array_edge.png}
%         % \label{fig:subfig2}
%     }\vskip\baselineskip
%     \subfigure[Subfigure 3]{%
%         \includegraphics[width=0.9\columnwidth]{figs/GPT3-175B_B=8_generic_array.png}
%         % \label{fig:subfig3}
%     }\hfill
%     \subfigure[Subfigure 4]{%
%         \includegraphics[width=0.9\columnwidth]{figs/GPT3-175B_B=8_generic_array_edge.png}
%         % \label{fig:subfig4}
%     }
%     \caption{Energy distribution in Llama1-7B and GPT3-175B models on a typical cloud and edge accelerator. \textbf{Bold} module names indicate weight $\times$ activation computations}
%     \label{fig:zigzag}
% \end{figure}




% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.25\linewidth]{TODO.pdf}
%     \caption{(a) Memory storage of W4A16 scheme compared to others (LLM-viewer); (b) FP16 takes majority energy consumption (Maybe from Zigzag?).}
%     \label{fig:1}
% \end{figure}

==> archive/3-algo.tex <==
% \begin{figure}[]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/overview_of_deployment_process.png}
%     \caption{Comparison of FIGNA and our Anda LLM deployment process.}
%     \label{fig:deployment}
% \end{figure}

\section{Anda Data Format} \label{sec:algo}
In this section, we present unique features of the Anda data format and demonstrate 
\rg{its benefits towards FP-INT operations}
% how to 
% seamlessly replace the FP16 activations with the Anda format 
% \rTwoFC{perform efficient FP-INT GeMM with the Anda format}
in weight-only quantized LLM inference. Furthermore, we introduce 
a \ms{mantissa bit-width search} method
%ms{driven by a tunable accuracy drop tolerance is introduced} 
to efficiently identify the optimized Anda precision combinations that satisfy a user-defined accuracy drop.
% , facilitating the efficient deployment of LLMs.

% \subsection{Motivation}

% \rOneFC{[Goal: We present experimental findings here.]}

% Finding 1: Nearby activations can be grouped to share the exponent part, which helps simplify the computation in the FP-INT units, while the appropriate group size has a negligible impact on model accuracy.

% By exploring the FP16 activations in large language models (LLMs), we discover that nearby activations can be grouped to share the exponent part, which helps simplify the computation in the FP-INT units. Taking LLaMA-7B as an example, in its four major modules, even when grouping 16 adjacent activations to share one exponent, the distribution of differences between these values and the shared exponent is highly concentrated, as shown by the red line in Fig.~\ref{fig:exp_diff_dist}. When the group size is increased to 64 or 256, the concentration level of the difference distribution remains largely unchanged. This suggests that we can implement efficient FP16 activation compression in hardware by storing only one shared exponent and multiple truncated mantissas, while the impact on model accuracy is negligible.

% \begin{figure}[]
%     \centering
%     \includegraphics[width=\linewidth]{figs/llama-7b.wikitext2_prealign_exp_diff_cdf.pdf}
%     \caption{The cumulative distribution of the difference between a shared-group exponent and the exponents of all other values in the group within a group size of 16, 64, and 256, respectively, for the four modules of FP activations in LLaMA-7b. The red dashed line represents the centroid of the distribution.}
%     \label{fig:exp_diff_dist}
% \end{figure}

% Finding 2: Substantial redundancy exists in the mantissa part of FP activations, and different mantissa bitwidths trade off accuracy for different application scenarios, enabling flexible adjustment.

% \begin{figure}[bp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/llama-7b.wikitext2_value_dist_wrt_addi_bits_gs64.pdf}
%     \caption{The value distribution of FP activations involved with the four modules with respect to varying preserved mantissa bits in LLaMA-7b within a shared group size of 64. \rOneFC{Or we just show some specific layer instead of all layers?}}
%     \label{fig:value_dist_wrt_addi_bits}
% \end{figure}

% We further find that substantial redundancy exists in the mantissa part of FP16 activations. Fig.~\ref{fig:value_dist_wrt_addi_bits} illustrates the activation value distributions of the four major modules in LLaMA-7B to varying preserved mantissa bitwidths, under a group size of 64. 
% It can be observed that as the number of preserved mantissa bits decreases, the distributions gradually converge towards zero. 
% This insight indicates that moderately reducing the mantissa bitwidth can significantly lower storage and computation overhead with a relatively small accuracy degradation. 
% Fig.~\ref{fig:acc_wrt_mbits} further quantifies this impact, showing that across 9 popular LLMs, a uniform reduction of 3-5 mantissa bits typically results in less than 5\% relative accuracy loss. Therefore, we can design flexible mantissa compression strategies in hardware according to different application scenarios, trading off efficiency and accuracy.


% Finding 3: Different modules in LLMs exhibit varying sensitivity of activation precision to model accuracy, necessitating a finer-grained exploration of the precision-bitwidth balance.

% Our study also reveals that different modules in LLMs exhibit varying sensitivity of activation precision to model accuracy. 
% As shown in Fig.~\ref{fig:module_wise_acc}, when reducing the mantissa bits only for the qkv\_proj module in OPT-1.3B and LLaMA-2-13B, the relative accuracy degradation can exceed 10\%. 
% However, if the mantissa bits are reduced for the fc2 module, the loss is controllable within 5\%. 
% This module-level discrepancy reflects the complexity and heterogeneity of the computational processes within LLMs. 
% To maximize the overall performance, we need to explore the optimal precision-bitwidth balance for different modules individually, rather than adopting a uniform strategy. 
% For instance, we can retain more mantissa bits for the qkv\_proj module while moderately reducing the mantissa bitwidth for the fc2 module to achieve better overall compression effectiveness.


\subsection{Anda Format Features}
% \TODO{Please skip this subsection until it is rebuilt.}

%\rOneFC{Our study in the previous section reveals that LLMs can maintain good performance with reduced mantissa lengths, albeit with varying sensitivities across different models and modules.}
%\rOneFC{These findings not only demonstrate the adaptability of LLMs to BFP formats but also highlight the limitations of existing BFP schemes.}

\rTwoFC{
% To address the limitations of existing BFP formats, 
% Innovated by our
\rg{Based on the} findings of our previous study, we propose the Anda format: an innovative variable-length mantissa BFP scheme designed for efficient LLM inference.}
% \rOneFC{Anda's definition process \ms{hence} resembles traditional BFP, as previously shown in Fig.~\ref{fig:fp_bfp_convert_process}, converting multiple FP16 tensors into a shared-exponent format \ms{at the first place}.}
% \rOneFC{Its basic structure comprises a sign bit, a shared exponent, and a variable-length mantissa.}
\rTwoFC{Anda's structure comprises a sign bit, a shared exponent, and a variable-length mantissa, building upon traditional BFP conversion processes as previously shown in Fig.~\ref{fig:fp_bfp_convert_process}.}
\rTwoFC{Its key feature is the ability to dynamically select mantissa lengths for different tensors based on their precision sensitivity, maintaining consistency within each tensor while optimizing the accuracy-efficiency trade-off.}
% \rOneFC{The distinguishing feature of Anda lies in its ability to dynamically select different mantissa lengths for different tensors based on their sensitivity to application precision. \ms{This allows for a mantissa bit width} range from 1 to 16 bits or even more while maintaining consistency within each tensor. \ms{Anda’s dynamic precision adjustment mechanism} %This dynamic adjustment mechanism enables Anda to 
% achieves an optimal balance between accuracy and efficiency across various application scenarios.}

\rTwoFC{Table~\ref{tab:bfp_cmp} compares Anda with prior BFP formats, categorizing them based on supported mantissa lengths.}
% Uni-length BFP formats, such as VS-Quant~\cite{dai2021vs} and FIGNA~\cite{jang2024figna}, use a fixed mantissa length for all operations. 
% Multi-length formats like FAST~\cite{zhang2022fast} and DaCapo~\cite{kim2024isca} offer limited flexibility with 2$\sim$3 predefined mantissa lengths. In contrast, Anda introduces a variable-length approach, supporting mantissa lengths from 1 to 16 bits or more.
\rTwoFC{Uni-length formats, such as VS-Quant~\cite{dai2021vs} and FIGNA~\cite{jang2024figna}, use fixed mantissa lengths, while multi-length formats like FAST~\cite{zhang2022fast} and DaCapo~\cite{kim2024isca} offer limited flexibility with 2$\sim$3 predefined lengths. Anda surpasses both by providing a continuous range of mantissa lengths, allowing fine-grained precision control across different LLM modules.}
\rg{Enabled by specialized hardware units, as detailed in Sec.~\ref{sec:arch}, smaller mantissa widths result in a lower inference latency, computational cost and memory storage cost. This allows Anda format to carefully balance model precision and computational efficiency, providing a more aggressive compression in less sensitive model
parts while preserving critical precision elsewhere.
} 
% \rg{[Below are hardware details, they are not relevant for the format yet! The key innovation is the precision flexibiilty, not the HW details.]}
% \rTwoFC{Moreover, Anda's \rg{intended} bit-serial computation enables efficient processing of variable-length mantissas, contrasting with the bit-parallel approach of most formats. Additionally, its bit-plane-based storage strategy optimizes memory access and utilization. These features, combined with shared exponents, allow Anda to balance precision flexibility and computational efficiency, enabling more aggressive compression in less sensitive model parts while preserving critical precision elsewhere.}
% \rTwoFC{Computation methods also differ significantly. While most formats use bit-parallel processing, Anda employs bit-serial computation, enabling more efficient processing of variable-length mantissas. Storage strategies vary as well, with Anda utilizing a bit-plane-based approach for optimal memory access and utilization.}
% \rTwoFC{Building upon these existing formats, Anda addresses their limitations by combining the precision flexibility of multi-length formats with the efficiency of shared exponents. It improves upon uni-length formats by allowing fine-grained precision control, and surpasses limited multi-length formats by offering a continuous range of mantissa lengths.}

% \rTwoFC{By enabling precision to be tailored for each tensor type within an LLM, Anda can optimize the trade-off between accuracy and efficiency at a granular level. This adaptability allows for more aggressive compression in less sensitive parts of the model while preserving precision where it's most critical.}

%As shown in 
% \rOneFC{Fig.~\ref{fig:datatype}(a) \ms{first} presents single-length mantissa BFP formats~\cite{dai2021vs, guo2023boost, lian2019high, jang2024figna, fan2018reconfigurable, koster2017flexpoint} \ms{which} struggle to accommodate the diverse precision requirements of different models and tasks.}
% \rOneFC{Multi-length mantissa BFP formats~\cite{zhang2022fast, kim2024isca, noh2023flexblock} offer \ms{certain} %some 
% flexibility, \ms{yet typically treat all components of LLM equally and fail to explore the potential performance improvement further.}} %their lengths are predetermined at design time, precluding dynamic adjustments during runtime.}

% \begin{table*}[t]
% \centering
% \caption{Anda format definition in contrast with prior BFP formats}
% \label{tab:anda}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lcccccccccc@{}}
% \toprule
% \textbf{Property} & \textbf{VS-Quant~\cite{dai2021vs}} & \textbf{BOOST~\cite{guo2023boost}} & \textbf{X. Lian et al.~\cite{lian2019high}} & \textbf{FIGNA~\cite{jang2024figna}} & \textbf{H. Fan et al.~\cite{fan2018reconfigurable}} & \textbf{Flexpoint~\cite{koster2017flexpoint}} & \textbf{FAST~\cite{zhang2022fast}} & \textbf{DaCapo~\cite{kim2024isca}} & \textbf{FlexBlock~\cite{noh2023flexblock}} & \textbf{Anda (Ours)} \\ \midrule
% BFP Type & Uni-Length & Uni-Length & Uni-Length & Uni-Length & Uni-Length & Uni-Length & Multi-Length & Multi-Length & Multi-Length & Variable-Length \\
% Mantissa Length during Computation & 4b & 5b & 8b & 14b & 15b & 16b & 2b/4b & 2b/4b/8b & 4b/8b/16b & 1b/2b/.../16b/... \\
% Computation & Bit-parallel & Bit-parallel & Bit-parallel & Bit-parallel & Bit-parallel & Bit-parallel & Chunk-serial & Bit-parallel & Bit-parallel & Bit-serial \\
% Storage & BFP Element-based & BFP Element-based & BFP Element-based & FP16 Element-based & BFP Element-based & BFP Element-based & BFP Chunk-based & BFP Element-based & BFP Element-based & BFP Bit-plane-based \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \caption{Anda format definition in contrast with prior BFP formats}
% \label{tab:anda}
% \resizebox{0.46\textwidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
%                & BFP Type        & \begin{tabular}[c]{@{}c@{}}Mantissa Length \\ during Computation\end{tabular} & Computation   & Storage             \\ \midrule
% VS-Quant~\cite{dai2021vs}       & Uni-Length      & 4b                                                                         & Bit-parallel & BFP Element-based   \\
% BOOST~\cite{guo2023boost}          & Uni-Length      & 5b                                                                         & Bit-parallel & BFP Element-based   \\
% X. Lian et al.~\cite{lian2019high} & Uni-Length      & 8b                                                                         & Bit-parallel & BFP Element-based   \\
% FIGNA~\cite{jang2024figna}          & Uni-Length      & 14b                                                                        & Bit-parallel & FP16 Element-based  \\
% H. Fan et al.~\cite{fan2018reconfigurable}  & Uni-Length      & 15b                                                                        & Bit-parallel & BFP Element-based   \\
% Flexpoint~\cite{koster2017flexpoint}      & Uni-Length      & 16b                                                                        & Bit-parallel & BFP Element-based   \\ \midrule
% FAST~\cite{zhang2022fast}           & Multi-Length    & 2b/4b                                                                      & Chunk-serial & BFP Chunk-based     \\
% DaCapo~\cite{kim2024isca}         & Multi-Length    & 2b/4b/8b                                                                   & Bit-parallel & BFP Element-based   \\
% FlexBlock~\cite{noh2023flexblock}      & Multi-Length    & 4b/8b/16b                                                                  & Bit-parallel & BFP Element-based   \\ \midrule
% \rowcolor[HTML]{FFFFC7} 
% \textbf{Anda (Ours)}    & \textbf{Variable-Length} & \textbf{1b/2b/.../16b/..}                                                           & \textbf{Bit-serial}   & \textbf{BFP Bit-plane-based} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[]
% \centering
% \caption{Anda format definition in contrast with prior BFP formats}
% \label{tab:my-table}
% \resizebox{0.46\textwidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
%                      & BFP Type                       & \begin{tabular}[c]{@{}c@{}}Mantissa Length \\ during Computation\end{tabular} & Compuation          & Storage                                    \\ \midrule
% VS-Quant             &                                & 4b                                                                            & Bit-parallel        & BFP Element-based                          \\
% BOOST                &                                & 5b                                                                            & Bit-parallel        & BFP Element-based                          \\
% X. Lian et al.       &                                & 8b                                                                            & Bit-parallel        & BFP Element-based                          \\
% FIGNA                &                                & 14b                                                                           & Bit-parallel        & \cellcolor[HTML]{FFFFFF}FP16 Element-based \\
% H. Fan et al.        &                                & 15b                                                                           & Bit-parallel        & BFP Element-based                          \\
% Flexpoint            & \multirow{-6}{*}{Uni-Length}   & 16b                                                                           & Bit-parallel        & BFP Element-based                          \\ \midrule
% FAST                 &                                & 2b/4b                                                                         & Chunk-serial        & BFP Chunk-based                            \\
% DaCapo               &                                & 2b/4b/8b                                                                      & Bit-parallel        & BFP Element-based                          \\
% FlexBlock            & \multirow{-3}{*}{Multi-Length} & 4b/8b/16b                                                                     & Bit-parallel        & BFP Element-based                          \\ \midrule
% \textbf{Anda (Ours)} & \textbf{Variable-Length}       & \textbf{1b/2b/.../16b/..}                                                     & \textbf{Bit-serial} & \textbf{BFP Bit-plane-based}               \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Anda format definition in contrast with prior BFP formats}
% \label{tab:my-table}
% \resizebox{0.46\textwidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
%                      & BFP Type                      & \begin{tabular}[c]{@{}c@{}}Mantissa Length \\ during Computation\end{tabular} & Compuation                    & Storage                      \\ \midrule
% VS-Quant             & \multirow{6}{*}{Uni-Length}   & 4b                                                                            & \multirow{6}{*}{Bit-parallel} & BFP Element-based            \\
% BOOST                &                               & 5b                                                                            &                               & BFP Element-based            \\
% X. Lian et al.       &                               & 8b                                                                            &                               & BFP Element-based            \\
% FIGNA                &                               & 14b                                                                           &                               & FP16 Element-based           \\
% H. Fan et al.        &                               & 15b                                                                           &                               & BFP Element-based            \\
% Flexpoint            &                               & 16b                                                                           &                               & BFP Element-based            \\ \midrule
% FAST                 & \multirow{3}{*}{Multi-Length} & 2b/4b                                                                         & Chunk-serial                  & BFP Chunk-based              \\
% DaCapo               &                               & 2b/4b/8b                                                                      & \multirow{2}{*}{Bit-parallel} & BFP Element-based            \\
% FlexBlock            &                               & 4b/8b/16b                                                                     &                               & BFP Element-based            \\ \midrule
% \textbf{Anda (Ours)} & \textbf{Variable-Length}      & \textbf{1b/2b/.../16b/..}                                                     & \textbf{Bit-serial}           & \textbf{BFP Bit-plane-based} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[t]
\centering
\caption{Anda format definition in contrast with prior BFP formats}
\label{tab:bfp_cmp}
\resizebox{0.46\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
                     & BFP Type                      & \begin{tabular}[c]{@{}c@{}}Mantissa Length \\ during Computation\end{tabular} & Computation                    & Storage                      \\ \midrule
VS-Quant~\cite{dai2021vs}             & \multirow{6}{*}{Uni-Length}   & 4b                                                                            & \multirow{6}{*}{Bit-parallel} & BFP Element-based            \\
BOOST~\cite{guo2023boost}                &                               & 5b                                                                            &                               & BFP Element-based            \\
X. Lian et al.~\cite{lian2019high}       &                               & 8b                                                                            &                               & BFP Element-based            \\
FIGNA~\cite{jang2024figna}                &                               & 14b                                                                           &                               & FP16 Element-based           \\
H. Fan et al.~\cite{fan2018reconfigurable}        &                               & 15b                                                                           &                               & BFP Element-based            \\
Flexpoint~\cite{koster2017flexpoint}            &                               & 16b                                                                           &                               & BFP Element-based            \\ \midrule
FAST~\cite{zhang2022fast}                 & \multirow{3}{*}{Multi-Length} & 2b/4b                                                                         & Chunk-serial                  & BFP Chunk-based              \\
DaCapo~\cite{kim2024isca}               &                               & 2b/4b/8b                                                                      & \multirow{2}{*}{Bit-parallel} & BFP Element-based            \\
FlexBlock~\cite{noh2023flexblock}            &                               & 4b/8b/16b                                                                     &                               & BFP Element-based            \\ \midrule
\rowcolor[HTML]{FFFFC7} \textbf{Anda (Ours)} & \textbf{Variable-Length}      & \textbf{1b/2b/.../16b}                                                     & \textbf{Bit-serial}           & \textbf{BFP Bit-plane-based} \\ \bottomrule
\end{tabular}%
}
\end{table}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figs/datatype.png}
%     % \caption{Representation of multiple tensor blocks using (a) conventional floating-point format, (b) block floating-point format, and (c) our proposed mantissa-scalable Anda format. \TODO{To be replaced.}}
%     \caption{(a) Anda format definition in contrast with prior BFP formats. (b) Drop-in replacement process for FP activations with Anda architecture during deployment.}
%     \label{fig:datatype}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.92\textwidth]{figs/workflow.pdf}
    \caption{Comparison of (a) the current computation scheme on GPU, (b) and that enhanced with dedicated FP-INT processing unit, (c) FIGNA scheme, and (d) our Anda scheme for FP-INT GeMM. Our Anda scheme significantly reduces memory space, access cost, and computation cost and enables energy-efficient precision-scalable operations.}
    \label{fig:workflow}
\end{figure*}
% \ms{Therefore, the Anda format (Fig.~\ref{fig:datatype}(a) bottom),} an innovative variable-length mantissa BFP scheme, \ms{is proposed} 
% \rOneFC{to address these constraints.} %\ms{as shown in Fig.~\ref{fig:datatype}(a) bottom. }}%, we propose the Anda format}, %an innovative variable-length mantissa BFP scheme.}
% \ms{Exsiting works \ms{[CITE]} have proved that sharing exponent strategy removes considerable overheads associated with computation and data movements, without sacrificing accuracy in LLM inference.}
% \rOneFC{Anda's definition process \ms{hence} resembles traditional BFP, converting multiple FP16 tensors into a shared-exponent format \ms{at the first place}.}
% \rOneFC{Its basic structure comprises a sign bit, a shared exponent, and a variable-length mantissa.}
% \rOneFC{The distinguishing feature of Anda lies in its ability to dynamically select different mantissa lengths for different tensors based on their sensitivity to application precision. \ms{This allows for a mantissa bit width} range from 1 to 16 bits or even more while maintaining consistency within each tensor. \ms{Anda’s dynamic precision adjustment mechanism} %This dynamic adjustment mechanism enables Anda to 
% achieves an optimal balance between accuracy and efficiency across various application scenarios.}

% \rOneFC{Fig.~\ref{fig:datatype}(b) %shows
% \ms{illustrates} the deployment of Anda \ms{which} involves two critical steps. Firstly, an adaptive precision combination search algorithm swiftly determines the optimal Anda format \ms{bit} configuration \ms{across different components of LLM}. This algorithm \ms{searches the possible candidates under the consideration of} %considers
% the given LLM architecture, task-specific data collected on-site, and a predefined accuracy tolerance. Importantly, this process occurs during the deployment phase, ensuring no impact on runtime performance. Secondly, leveraging the optimal Anda format configuration, the Anda-aware hardware architecture seamlessly replaces the original FP16 activations with Anda format during execution. This approach guarantees efficient inference, saving both time and energy, while maintaining transparency to the user.}

% \rOneFC{In the following sections, we will delve into Anda's workflow, precision search algorithm, and the design of Anda-aware hardware architecture. Through this comprehensive exploration, we aim to demonstrate Anda's potential in enhancing LLM inference efficiency.}

% % \rOneFC{[Goal: Present what Anda type is, and what is the difference and its benefits over the other datatypes. And how to use it in LLMs.]}
% Fig.~\ref{fig:datatype} \mv{introduces the Anda format and compares it to} conventional FP and BFP formats. %, and Anda Format, showcasing their respective schemes for representing multiple tensor blocks.
% All these numeric representations consist of three fields: sign, exponent, and mantissa. \ms{As} shown in Fig.~\ref{fig:datatype}(a), in conventional FP, %each 
% \ms{individual} element %possesses
% \ms{equips} its own set of these three fields. For instance, the commonly used FP16 format in W4A16 LLMs, as defined by the IEEE754 standard, comprises \ms{1-bit sign, 5-bit exponent as well as 10-bit mantissa.} \ms{This provides
% a wide \ms{data} dynamic range representation and maintains high numerical accuracy in a variety of computation applications}. %for individual elements. 
% %1 sign bit, 5 exponent bits, and 10 mantissa bits. 
% \ms{Yet, traditional FP representation falls short of effectiveness}
% %However, this format is computationally expensive 
% due to \ms{its costly} exponent alignment and normalization during MAC operations and \ms{associated}
% %It also has 
% higher storage and memory access overhead 
% compared to \ms{integer} %INT4 
% representation. %for weights
% BFP \ms{alleviates}
% %ddresses 
% the computational and storage overhead of FP16 by sharing the exponent field within each tensor block, simplifying multiply-accumulate operations. However, previous BFP formats used fixed-length mantissa fields, limiting their adaptability to different LLM tasks and architectures.

% An shown in Fig.~\ref{fig:datatype}(a), in conventional FP, each element possesses its own set of these three fields, allowing for a wide dynamic range representation for individual elements. For instance, the commonly used FP16 format in W4A16 LLMs, as defined by the IEEE754 standard, comprises 1 sign bit, 5 exponent bits, and 10 mantissa bits. However, this format incurs significant computational overhead during GEMM operations due to the need for exponent alignment and normalization for each multiply-accumulate operation, substantially increasing the computational cost. Moreover, compared to INT4 representation for weight parameters, using FP16 for activations also entails higher storage and memory access overhead.

% Fig.~\ref{fig:datatype}(c) presents our proposed Anda Format, which is motivated by our previous explorations of BFP in LLMs. 
% We observed that different modules in W4A16 LLMs exhibit varying sensitivity to the mantissa reduction of activations. 
% %Traditional BFP formats, which employ a length-static mantissa field and apply a uniform BFP across all activations, either risk compromising model accuracy or struggle to achieve efficient computation and storage benefits while maintaining accuracy. 
% To address this, we build upon the shared exponent field of BFP and \mv{additionally} introduce a \mv{variable-length} mantissa field within each tensor block. 
% This adaptability allows the Anda format to accommodate the diverse precision requirements of different modules in LLMs, optimizing storage and computational overhead while preserving model accuracy. 
%In Anda Format, the exponent field is shared within each block, while the mantissa field is determined based on the impact of data format conversion on the model accuracy of the corresponding LLM module.

%\subsection{Anda Format Workflow}
\subsection{Efficient FP-INT GeMM Using Anda Format}
% To further demonstrate the potential advantages of replacing FP16 activations with the Anda data format, we compare the workflow of W4A16 \mv{deployment for different SotA approaches}: (a) W4A16 GeMM execution on existing GPU platforms; (b) \mv{deployment on hardware with} dedicated FP16-INT4 computation units; (c) \mv{exploitation of} FIGNA's \mv{dynamic alignment} scheme; and (d) our proposed Anda approach. Fig.~\ref{fig:workflow} \mv{illustrates these different schemes, where the colors denote the data types used along the computational flow.}

\rOneFC{We then compare the workflows of \ms{GeMM workloads} of several SotA approaches %for deploying weight-only quantized LLMs 
to illustrate the advantages of replacing FP16 activations with the Anda data format. Taking the W4A16 quantization scheme as an example, we examine the FP-INT GeMM computation process (a) on existing GPU platforms~\cite{lin2024qserve}; (b) on GPU platforms with dedicated FP-INT processing units; (c) using FIGNA's dynamic conversion scheme~\cite{jang2024figna}; and (d) with our proposed Anda approach. Fig.~\ref{fig:workflow} depicts %these different
the \ms{four} schemes, with colors indicating the data types used throughout the computational process.}

% When deploying W4A16 LLMs on existing GPU platforms, as shown in Fig.~\ref{fig:workflow}(a), due to the lack of dedicated FP-INT computation units, the current computation scheme reads INT4 weights and FP16 activations from memory, converts INT4 weights to FP16 before computation, and then utilizes \mv{the tensor cores in FP16 mode} for calculation. This scheme not only \mv{brings} additional format conversion overheads, but also \mv{requires costly} FP computations.

% \rOneFC{When deploying W4A16 LLMs on existing GPU platforms, as shown in Fig.~\ref{fig:workflow}(a),
\ms{Fig.~\ref{fig:workflow}(a) shows the \rg{workflow of} W4A16 LLMs on common GPU platforms}. 
% The lack of dedicated FP-INT computation units \ms{in GPU} necessitates %reading INT4 weights and FP16 activations from memory, 
% converting INT4 weights to FP16 before computation. \ms{Tensor cores are active in an FP16 mode for calculations.}} 
\rTwoFC{The absence of dedicated FP-INT computation units in GPU necessitates converting INT4 weights to FP16 before processing, with tensor cores operating in FP16 mode.}
This scheme not only brings additional format conversion overheads, but requires costly FP computations.

% \mv{Equipping compute} platforms with dedicated FP-INT computation units, as illustrated in Fig.~\ref{fig:workflow}(b), can save the data conversion overhead from INT4 to FP16 and \mv{reduce the cost of the} computations.
% However, as pointed out by FIGNA~\cite{jang2024figna}, due to the high alignment and normalization overhead in FP-INT computation units, the computational cost of dedicated FP-INT computation units remains high.
\rOneFC{GPU platforms equipped with dedicated FP-INT processing units, as illustrated in Fig.~\ref{fig:workflow}(b), can eliminate the need for converting INT4 weights to FP16, thereby reducing data conversion overheads and computation costs.}
\rOneFC{However, as pointed out by FIGNA~\cite{jang2024figna}, the high alignment and normalization overhead associated with FP-INT processing units still results in high computational expenses.}

\rOneFC{To efficiently deploy W4A16 LLMs, FIGNA proposes a computation scheme using a BFP variant with corresponding hardware support to overcome the issues with dedicated FP-INT units.}
As \ms{depicted} in Fig.~\ref{fig:workflow}(c), activations are stored in FP16 format in memory, converted to the FIGNA format before computation, \mv{after which} a 14-bit \mv{mantissa is multiplied} with INT4 weights for GeMM computation. The final results are then converted \mv{again} to FP16 and written back to memory.
\rOneFC{This scheme reduces the computation overhead by converting costly FP GeMM to INT operations.}
However, since FP16 activations need to be repeatedly \mv{accessed} during computation, frequent data conversion from FP16 to FIGNA introduces additional overhead, affecting overall efficiency.

% \mv{Finally}, our proposed Anda format computation scheme offers some unique advantages. 

\rOneFC{As presented in Fig.~\ref{fig:workflow}(d), our proposed Anda format computation scheme offers some unique advantages in contrast with the previous approaches.}
% \mv{the activations are no longer stored in memory in FP16, but directly in the Anda data format. This directly} reduces storage overhead \mv{and} data access overhead, while avoiding frequent data conversion. 
% Moreover, due to the shared exponent, the \mv{multiplication of INT4 weights with} Anda activations \mv{results in pure} INT \mv{dot-product operations within a shared exponent group, followed by an FP32 accumulation across groups}, reducing computational overhead. 
\rOneFC{Firstly, the activations are no longer stored in memory in FP16 \rg{format}, but directly in the Anda data format, reducing storage overhead and data access overhead while avoiding frequent data conversion.}
\rOneFC{Secondly, the shared exponent enables INT dot-product operations within a group, followed by FP32 accumulation across groups, reducing the computational overhead of FP-INT GeMMs.}
\rOneFC{Thirdly, the variable-length mantissa \ms{considerably decreases} dot-product operations and memory accesses use the minimal necessary word length.}
\rOneFC{Finally, converting only the final FP32 results back to Anda format before writing to memory minimizes the storage \ms{requirement} %overhead 
and the additional overhead from switching data format.}
%\rOneFC{Combined, these features make the Anda format an efficient choice when deploying weight-only quantized LLMs.}
% We only need to convert \mv{the final accumulated} FP32 results \mv{once back} to the Anda format before writing them back to memory, reducing memory storage overhead while minimizing the additional overhead caused by frequent data switching. 
% \mv{Finally, the variable-length mantissa ensures that all dot-product operations and all memory access take place with the minimal word length necessary.}

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figs/representation.png}
%     \caption{The process of adaptive precision combination search. \TODO{The input and output of our algorithm. Also the termination.}}
%     \label{fig:rep}
% \end{figure}


% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figs/algo_process.png}
%     \caption{The process of adaptive precision combination search. \TODO{The input and output of our algorithm. Also the termination.}}
%     \label{fig:algo}
% \end{figure}

% \begin{algorithmic}[1]
% \REQUIRE LLM model $M$, calibration dataset $D$, accuracy tolerance $\delta$, max iterations $N$
% \ENSURE Optimal precision combination $[M_{qkv}, M_o, M_u, M_d]$

% \STATE Initialize priority queue $Q$ with combinations from $[4,4,4,4]$ to $[13,13,13,13]$
% \STATE $best \gets null$, $best\_bops \gets \infty$

% \FOR{$i = 1$ to $N$}
%     \STATE $c \gets Q.pop()$ \COMMENT{Extract combination with lowest BOPs}
%     \STATE $bops \gets \text{CalculateBOPs}(c)$
%     \STATE $acc \gets \text{EvaluateAccuracy}(M, D, c)$
    
%     \IF{$bops < best\_bops$ \AND $acc \geq (1-\delta) \cdot \text{BaselineAccuracy}(M, D)$}
%         \STATE $best \gets c$
%         \STATE $best\_bops \gets bops$
%         \STATE $neighbors \gets \text{GenerateNeighbors}(c)$
%         \FOR{$n \in neighbors$}
%             \STATE $Q.push(n)$
%         \ENDFOR
%     \ENDIF
    
%     \IF{$Q.empty()$ \OR $i = N$}
%         \STATE \textbf{break}
%     \ENDIF
% \ENDFOR

% \RETURN $best$
% \end{algorithmic}

% \begin{algorithm}[t]
% \caption{Adaptive Precision Search for Anda}
% \label{alg:anda_search}
% \SetAlgoLined
% \KwIn{LLM model $M$, calibration dataset $D$, \\ accuracy tolerance $\delta$, max iterations $N$}
% \KwOut{Optimal precision combination $[M_{qkv}, M_o, M_u, M_d]$}
% \BlankLine
% Initialize priority queue $Q$ with combinations from $[4,4,4,4]$ to $[13,13,13,13]$;

% $best \gets null$, $best_bops \gets \infty$;

% \While{\textnormal{not converged and iterations} $< N$}{
%     $c \gets Q.pop()$ \tcp*{Extract combination with lowest BOPs}
%     $bops \gets \text{CalculateBOPs}(c)$\;
%     $acc \gets \text{EvaluateAccuracy}(M, D, c)$\;
    
%     \If{$bops < best\_bops$ \textnormal{\textbf{and}} $acc \geq (1-\delta) \cdot \text{BaselineAccuracy}(M, D)$}{
%         $best \gets c$\;
%         $best\_bops \gets bops$\;
%         $neighbors \gets \text{GenerateNeighbors}(c)$\;
%         \ForEach{$n \in neighbors$}{
%             $Q.push(n)$\;
%         }
%     }
    
%     \If{$Q.empty()$}{
%         \textbf{break}\;
%     }
% }

% \Return $best$
% \end{algorithm}

% \begin{algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \caption{Adaptive Precision Search for Anda Format}
% \label{alg:anda_search}
% \begin{algorithmic}[1]
% \REQUIRE LLM model $M$, calibration dataset $D$, accuracy tolerance $\delta$, max iterations $N$
% \ENSURE Optimal precision combination $[M_{qkv}, M_o, M_u, M_d]$
% \STATE Initialize priority queue $Q$ with combinations from $[4,4,4,4]$ to $[13,13,13,13]$
% \STATE $best \gets null$, $best_bops \gets \infty$
% \WHILE{not converged and iterations $< N$}
% \STATE $c \gets Q.pop()$ \COMMENT{Extract combination with lowest BOPs}
% \STATE $bops \gets \text{CalculateBOPs}(c)$
% \STATE $acc \gets \text{EvaluateAccuracy}(M, D, c)$
% \IF{$bops < best_bops$ \textbf{and} $acc \geq (1-\delta) \cdot \text{BaselineAccuracy}(M, D)$}
% \STATE $best \gets c$
% \STATE $best_bops \gets bops$
% \STATE $neighbors \gets \text{GenerateNeighbors}(c)$
% \FORALL{$n \in neighbors$}
% \STATE $Q.push(n)$
% \ENDFOR
% \ENDIF
% \IF{$Q.empty()$}
% \STATE \textbf{break}
% \ENDIF
% \ENDWHILE
% \STATE \textbf{return} $best$
% \end{algorithmic}
% \end{algorithm}


% \usepackage[ruled,vlined,linesnumbered]{algorithm2e}

% \begin{algorithm}[t]
% \SetAlgoLined
% \caption{Adaptive Precision Combination Search}
% \label{alg:anda_search}
% \KwIn{LLM model $M$, calibration dataset $D$, accuracy tolerance $\delta$, max iterations $N$}
% \KwOut{Optimal precision combination $[M_{qkv}, M_o, M_u, M_d]$}

% Initialize priority queue $Q$ with combinations from $[4,4,4,4]$ to $[13,13,13,13]$\;
% $best \gets null$, $best\_bops \gets \infty$\;

% \While{not converged and iterations $< N$}{
%     $c \gets Q.pop()$ \tcp*{Extract combination with lowest BOPs}
%     $bops \gets \text{CalculateBOPs}(c)$\;
%     $acc \gets \text{EvaluateAccuracy}(M, D, c)$\;
    
%     \If{$bops < best\_bops$ \textnormal{\textbf{and}} $acc \geq (1-\delta) \cdot \text{BaselineAccuracy}(M, D)$}{
%         $best \gets c$\;
%         $best\_bops \gets bops$\;
%         $neighbors \gets \text{GenerateNeighbors}(c)$\;
%         \ForEach{$n \in neighbors$}{
%             $Q.push(n)$\;
%         }
%     }
    
%     \If{$Q.empty()$}{
%         \textbf{break}\;
%     }
% }

% \Return $best$
% \end{algorithm}

% \begin{algorithm}[t]
% \small
% \SetAlgoLined
% \caption{Adaptive Precision Combination Search}
% \label{alg:anda_search}
% \KwIn{LLM model $L$, calibration dataset $D$, \newline accuracy loss tolerance $\delta$, max iterations $N$}
% \KwOut{Optimized precision combination $best.comb$ denoted as a 4-tuple $[M_\text{qkv}, M_\text{o}, M_\text{u}, M_\text{d}]$}
% % \vspace{2pt}
% \tcp{S1: Initialize search starting points}
% {Initialize priority queue $Q$ with combinations \newline \hspace*{2em} from $[4,4,4,4]$ to $[13,13,13,13]$}\;
% $best.comb \gets \text{null}$, $best.bops \gets \infty$, \textit{iterations} $\gets$ 0\;
% $fp\_acc \gets \textbf{EvaluateAccuracy}(L, D)$\;
% $visited \gets \{\}$\;
% \While{iterations $< N$}{\tcp{S2: Check the promising combination}
%     Calculate BOPs for all combinations in $Q$\;
%     $curr \gets Q.\text{popMinBOPs}()$\;
%     $visited \gets visited \cup \{curr.comb\}$\;
%     $anda\_acc \gets \textbf{EvaluateAccuracy}(L, D, curr)$\;\tcp{S3: Update and relax the best combination}
%     \If{$curr.bops < best.bops$ \textnormal{\textbf{and}} $anda\_acc \geq (1-\delta) \cdot fp\_acc$}{
%         $best.comb \gets curr.comb$, $best.bops \gets curr.bops$\;
%         $neighbors \gets \textbf{GenerateCandidates}(curr.comb)$\;
%         \ForEach{$n \in neighbors$}{
%             \If{$n \notin visited$}{
%                 $Q.\text{push}(n)$\;
%             }
%         }
%     }
%     \If{$Q.\text{empty}()$}{
%         \textbf{break}\;
%     }
%     \textit{iterations} $\gets$ \textit{iterations} + 1\;
% }
% \Return $best.comb$
% \end{algorithm}

\begin{algorithm}[t]
\small
\SetAlgoLined
\caption{Adaptive Precision Combination Search}
\label{alg:anda_search}
\KwIn{LLM model $L$, calibration dataset $D$, \newline accuracy loss tolerance $\delta$, max iterations $N$}
\KwOut{Optimized precision combination $best\_comb$ denoted as a 4-tuple $[M_{qkv}, M_{o}, M_{u}, M_{d}]$}
% \vspace{2pt}
\tcp{S1: Initialize search starting points}
% {Initialize priority queue $Q$ with combinations \newline \hspace*{2em} from $[4,4,4,4]$ to $[13,13,13,13]$}\;
$Q \gets PriorityQueue([4,4,4,4], ..., [13, 13, 13, 13])$\;
$best\_comb \gets \text{null}$\; 
$best\_bops \gets \infty$\; 
\textit{iterations} $\gets$ 0\;
$visited \gets \{\}$\;
$fp\_acc \gets \textbf{EvaluateAccuracy}(L, D)$\; 
\While{iterations $< N$}{
    \tcp{S2: Check the promising combination}
    $bops\_eval \gets Q.\text{map}(\textbf{EvalBOPs})$\;
    $curr\_bops \gets min(bops\_eval)$\;
    % $curr\_bops \gets \text{min}(\textbf{EvalBOPs}(Q.\text{forEach}()))))$\;
    $curr\_comb \gets Q.\text{get}(bops\_eval.\text{index}(curr\_bop))$\;
    $visited \gets visited \cup \{curr\_comb\}$\;
    $anda\_acc \gets \textbf{EvaluateAccuracy}(L, D, curr\_comb)$\;
    \tcp{S3: Update and relax the best combination}
    \If{$curr\_bops < best\_bops$ \textnormal{\textbf{and}} $anda\_acc \geq (1-\delta) \cdot fp\_acc$}{
        $best\_comb \gets curr\_comb$\; 
        $best\_bops \gets curr\_bops$\;
        $neighbors \gets \textbf{GenerateCandidates}(curr\_comb)$\;
        \ForEach{$n \in neighbors$}{
            \If{$n \notin visited$}{
                $Q.\text{push}(n)$\;
            }
        }
    }
    \If{$Q.\text{empty}()$}{
        \textbf{break}\;
    }
    \textit{iterations} $\gets$ \textit{iterations} + 1\;
}
\Return $best\_comb$
\end{algorithm}


\subsection{Adaptive Precision Combination Search}

% \rOneFC{Due to varying sensitivity across different activation tensor types in weight-only quantized LLMs, finding the optimal precision for each activation tensor type and selecting the most suitable Anda format is crucial for improving LLM inference efficiency.}
% \rOneFC{Hence, we propose an adaptive precision combination search algorithm aimed at finding the optimal precision combination for four key activation tensor types, i.e., $A_{qkv}$, $A_o$, $A_u$, and $A_d$ in weight-only quantized LLMs.}
% \rOneFC{These types are represented by their mantissa lengths: $M_0$, $M_1$, $M_2$, and $M_3$, respectively.}
% \mv{It is important to note that for each tensor type the same mantissa lengths are used across all layers of an LLM. 
% We will in the remainder of the paper represent the selected mantissa lengths} by a 4-tuple $[M_0, M_1, M_2, M_3]$ as shown in Fig.~\ref{fig:algo}.

\rOneFC{To maximize the performance benefits of the Anda format, we propose an adaptive precision search algorithm that aims to optimize mantissa length combination for four key activation tensor types: $A_{qkv}$, $A_o$, $A_u$, and $A_d$,
% . \ms{The mantissa bitwidth candidates of these tensors are} 
where the combination is represented as a 4-tuple $[M_{qkv}, M_o, M_u, M_d]$.}
% \rOneFC{By accounting for the varying sensitivity across different activation types, our algorithm assigns unique mantissa lengths to each type, while keeping these lengths consistent across all layers, %enabling us to
% striking a good balance between model accuracy and performance.}
\rOneFC{By accounting for the varying sensitivity across different activation types, our algorithm assigns unique mantissa lengths to each type while maintaining consistency across all layers, striking a balance between model accuracy and performance.}
% \rOneFC{By accounting for the varying sensitivity across different activation tensor types in weight-only quantized LLMs, our approach maintains consistent mantissa lengths for each activation type across all layers, thereby achieving an optimal balance between model accuracy and performance.}
% \rOneFC{Due to varying sensitivity across different activation tensor types in weight-only quantized LLMs, we propose an adaptive precision combination search algorithm to find the optimal mantissa lengths represented by a 4-tuple, $[M_0, M_1, M_2, M_3]$, for four key activation tensor types: $A_{qkv}$, $A_o$, $A_u$, and $A_d$. These mantissa lengths of each activation type are consistent across all layers of an LLM.}
% We will in the remainder of the paper represent the selected mantissa lengths by a 4-tuple $[M_0, M_1, M_2, M_3]$ as shown in Fig.~\ref{fig:algo}.

% \rOneFC{The algorithm takes the LLM model, a calibration dataset, an accuracy tolerance, and a maximum number of iterations \ms{as inputs}. 
% % The calibration dataset is sampled from training data for experiments, while deployment site data is used for real-world applications. 
% The calibration dataset is sampled from the training dataset in our experiments. For real-world applications, %however, 
% calibration data %should
% \ms{can} be collected on-site to reflect the actual deployment environment.
% % An accuracy tolerance specifies the acceptable level of performance degradation. In practice, a 1\% accuracy loss is generally considered negligible for inference deployment, allowing for significant optimization.
% The accuracy tolerance specifies the acceptable level of performance degradation. %typically set at 1\% loss. 
% The maximum number of iterations serves as a \ms{search} termination criterion, concluding the algorithm within a reasonable time frame.}
% \ms{Processing these inputs, our algorithm eventually}
% %The algorithm 
% outputs the 4-tuple precision combination that best balances model accuracy and inference efficiency across the model's key components.
% \rOneFC{The algorithm consists of three key steps, \ms{as shown in Fig.~\ref{fig:algo} [modify here]}:}
% % The algorithm \mv{to find the best 4-tuple leading to a precision loss $< 1\%$} consists of three key steps as shown in Fig.~\ref{fig:algo}: 

\rOneFC{As outlined in Algorithm~\ref{alg:anda_search}, we take the LLM model~$L$, a calibration dataset $D$, an accuracy loss tolerance $\delta$, and a maximum number of iterations $N$ as inputs. The calibration dataset is sampled from the training dataset in our experiments.
For real-world applications, calibration data can be collected on-site to reflect the actual deployment environment.
The accuracy tolerance $\delta$ specifies the acceptable level of performance degradation, while the maximum number of iterations $N$ serves as a termination criterion, ensuring the algorithm concludes within a reasonable time frame. With these inputs, our algorithm finds the optimal 4-tuple precision combination within the given iterations that best balances model accuracy and inference efficiency across the model's key activation components.}
The search process consists of three key steps.

\rOneFC{\textbf{Step 1: Initialize search starting points.} %We initialize 
A priority~queue with precision combinations of equal precision across all modules \ms{is initialized first}. These \ms{precision} combinations range from aggressive (e.g., $[4,4,4,4]$) to conservative (e.g., $[13,13,13,13]$). This strategy enables the rapid discovery of efficient combinations while ensuring the existence of feasible solutions, as validated by our prior experiments in Fig.~\ref{fig:acc_wrt_mbits}.}

% \rOneFC{\textbf{Step 2: Find and evaluate the promising combination.} In each iteration, we extract the combination with the lowest bit operations (BOPs) from the priority queue. The BOP metric~\cite{abati2023resq, koryakovskiy2023one, li2024quasar} serves as a rapid proxy for estimating computational cost. Specifically, BOP calculates the total number of bit operations required for all necessary multiplications under a given precision combination. This quick estimation allows us to efficiently prioritize promising combinations without full model evaluation. We then evaluate the accuracy of this minimal-BOP combination on the calibration dataset, a more time-consuming but crucial step to ensure model accuracy. This two-step approach balances rapid exploration of the search space with thorough validation of model accuracy, enabling efficient discovery of optimal precision combinations.}

\rOneFC{\textbf{Step 2: Check the promising combination.} 
% In each iteration, we extract the combination with the lowest bit operations (BOPs) from the priority queue as depicted in \ms{Fig.~\ref{fig:algo} modify here}.
% In each iteration, the combination with the lowest bit operations (BOPs) is extracted from the priority queue, which is considered a promising combination.
In each iteration, the combination with the lowest bit operations (BOPs) is extracted from the priority queue and added to the visited set.
The BOP metric~\cite{abati2023resq, koryakovskiy2023one, li2024quasar, tian2023bebert} quickly estimates computational cost by calculating the total number of bit operations for the necessary multiplications under a given combination. 
This allows us to efficiently prioritize promising combinations %\rg{with a low computing cost.} 
without a full model evaluation. 
The accuracy of the promising combination is then examined on the calibration dataset.} 
% We then examine the accuracy of the promising combination on the calibration dataset.} 
%\ms{[the last sentence breaks the consistency with the following step and is repeated with the last para, so comment out.]}%This two-step approach balances rapid search space exploration with accurate model accuracy validation, enabling efficient discovery of optimal precision combinations.}

\rOneFC{\textbf{Step 3: Update and relax the best combination.} If the evaluated combination yields lower BOPs than the current best while maintaining accuracy within the specified tolerance, it becomes the new best combination. 
To generate nearby precision candidates, the algorithm then relaxes this best combination by decreasing the mantissa length of each tensor type by one, while keeping the other tensor types unchanged.
For example, if the current best combination is $[6,7,5,5]$, the generated candidates will be $[5,7,5,5]$, $[6,6,5,5]$, $[6,7,4,5]$, and $[6,7,5,4]$.
% , such as $[M_{qkv}-1, M_o, M_u, M_d]$, $[M_{qkv}, M_o-1, M_u, M_d]$, etc. 
The generated candidates that have not been visited before are added to the priority queue.
If the accuracy constraint is not met, no update is made.}
% We then relax this combination by generating nearby precision combinations (e.g., [6,6,5,5], [6,7,4,5], [6,7,5,4], [5,7,5,5]) and add them to the priority queue for future evaluation. \mv{If the accuracy constraint is not met}, no update is made.}

% \rOneFC{The process of Step 2 and 3 repeats until meeting predefined termination criteria, such as reaching a maximum number of iterations or exhausting the search space. This approach efficiently navigates the vast search space, prioritizing the most promising precision combinations and ensuring convergence to an optimal solution that balances accuracy and efficiency.}
\rOneFC{Step 2 and 3 are repeated until the maximum number of iterations is reached or the search space is exhausted. The use of the visited set ensures that the algorithm does not evaluate the same combination multiple times.}
This approach efficiently navigates the vast search space, prioritizing the most promising precision combinations and ensuring convergence to an optimal solution that balances accuracy and efficiency.

% Step 2 and 3 are repeated iteratively until a predefined termination condition is met \mv{[which one? This is too vague...]}. This iterative process allows the algorithm to explore the search space efficiently and find an optimal precision combination that balances computational cost and model accuracy. The algorithm ensures that each combination is evaluated for accuracy at most once, significantly saving \mv{convergence time}. 
%Through the iterative process between Step 2 and Step 3, an excellent precision combination that satisfies the constraints can be found for subsequent efficient deployment.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/greedy_search_with_arrows.pdf}
    \caption{Search process of the proposed adaptive precision combination search algorithm on the OPT-125M model with constraint under 1\% accuracy loss, which efficiently finds the global optimum within 10 iterations.}
    \label{fig:prec_comb_eff}
\end{figure}

\subsection{Precision Combination Search Efficiency}
% \ms{feel this subsection should be moved to Section III, right after III.C; this is also not matched with V.A}
% \rOneFC{[Goal: Quantitatively analyze the search efficiency and compare it with methods like brute-force search to demonstrate the superiority of the proposed approach.]}

% \TODO{Rewrite to adapt the whole structure}

\rOneFC{To further demonstrate the efficiency of our adaptive precision search algorithm, we compare it with conventional brute-force approaches~\cite{dai2021vs,darvish2020pushing,darvish2023shared} on the OPT-125M model. Exhaustive search for all precision combinations on larger LLMs would be computationally infeasible, making OPT-125M, a mini-size LLM, \rg{more suited} for this comparison.}

% \rOneFC{As illustrated in Fig.~\ref{fig:prec_comb_eff}, the search space for OPT-125M contains over 10,000 possible combinations, denoted as yellow dots. Our algorithm, however, identifies the global optimum combination $[7, 7, 6, 5]$ within just 10 iterations, preserving accuracy within a 1\% loss.}
\rTwoFC{The OPT-125M search space shown in Fig.~\ref{fig:prec_comb_eff} includes over 10,000 possible combinations, denoted as yellow dots. Our algorithm identifies the global optimum combination $[7, 7, 6, 5]$ within just 10 iterations, maintaining accuracy within a 1\% loss.
The entire search process is illustrated in the bottom right corner of Fig.~\ref{fig:prec_comb_eff}.}
% This showcases our algorithm's ability to efficiently navigate the vast search space and locate optimal solutions with significantly reduced computational overhead.}
% \rOneFC{Our algorithm can efficiently navigate the vast search space to approach optimal solutions, significantly reducing computational overhead.}
\rOneFC{The training-free adaptive precision search algorithm employs forward-only evaluation on LLMs in just a few iterations, making it highly suitable for widespread adoption in LLM deployment scenarios.}
% \rOneFC{Moreover, our training-free algorithm outperforms conventional methods like MSFP~\cite{darvish2020pushing} and VS-Quant~\cite{dai2021vs}, which often require costly retraining processes. By leveraging fast validation on a calibration dataset, our algorithm finds optimal combinations within a given accuracy tolerance, greatly reducing the search time before deployment.}
% \rOneFC{By leveraging fast validation on a calibration dataset, our training-free algorithm efficiently finds optimal combinations within a given accuracy tolerance, greatly reducing the search time before deployment.}
% \rOneFC{This training-free adaptive precision combination search algorithm can quickly locate optimal solutions within a few numbers of iterations for forward-only evaluation on LLMs in a one-shot way, significantly reducing computational overhead and making it suitable for wide adoption.}
% \rOneFC{Our training-free adaptive precision search algorithm can efficiently locate optimal solutions for LLMs within a small number of iterations using forward-only evaluation, significantly reducing computational overhead and making it suitable for wide adoption in LLM deployment scenarios.}

% \rOneFC{The efficiency of our algorithm stems from two key factors. First, the BOP metric enables quick computational cost estimation without full model evaluation. Second, the relaxation step generates promising nearby combinations, guiding the search towards the optimal solution. These techniques allow our algorithm to efficiently explore the search space and converge to an optimal precision combination that balances accuracy and efficiency, making it suitable for wide adoption in LLM deployment.}

% We first evaluate the efficiency of the proposed adaptive precision combination search method, which is essential \rg{[not that essential because you only need to run it once right?]} for rapid LLM deployment \rg{[make sure distinction between deployment and inference/serving is clear throughout the paper}] in real-world scenarios. \rg{This helps with rapidly adapting a LLM to a different task and easily switching the LLM run on the Anda Architecture}
% \ms{In this section,}
% %To demonstrate 
% the advantages of our method compared to conventional brute-force search approaches~\cite{dai2021vs,darvish2020pushing,darvish2023shared} \ms{are discussed}. \ms{The smallest} OPT-125M \ms{is adopted as the baseline model, because the other LLM models are too gigantic to conduct an exhaustive search for all}
% %, we choose OPT-125M as the baseline model, as it allows for an exhaustive search of all 
% precision combinations.
% %Conventional methods become prohibitively time-consuming for LLMs, while our method efficiently finds optimal combinations within a given error range by fast validation on a calibration dataset, significantly reducing the searching time before deployment.

% Setting the minimum mantissa bit-width to 4, %we
% \ms{our algorithm} searches for the best combination within 10 iterations. As shown in Fig.~\ref{fig:prec_comb_eff}, \ms{yellow dots are all the possible combination candidates explored exhaustively.} For the OPT-125M model, the total number of possible precision combinations exceeds 10,000. \ms{This number will exponentially increase in larger LLMs,}
% making exhaustive search \ms{become unrealistic.} %computationally expensive. 
% \as{[Some numbers regarding search time would help here, even if they're ballpark.]} \ms{On the contrary,}
% our method progressively approaches the global optimum, finding the optimal combination [7, 7, 6, 5] in the 9\textsuperscript{th} iteration.
% % Our algorithm demonstrates superior efficiency by finding the global optimum in just 10 iterations. 
% \ms{This training-free adaptive precision combination search algorithm}
% %Our algorithm demonstrates it \rg{[We demonstrate that the algorithm]} 
% can quickly locate optimal solutions within \ms{a few} %an acceptable 
% number of iterations for LLMs \ms{in a one-shot way, significantly} reducing computational overhead and making it suitable for wide adoption. 
% %Experimental results show that our searching method outperforms MX~\cite{darvish2020pushing,darvish2023shared} and VS-Quant~\cite{dai2021vs} in terms of efficiency and effectiveness, while allowing flexible adjustment of iterations and precision thresholds to balance accuracy and speed for various scenarios. 
% %Additionally, our method does not require backpropagation, reducing computational overhead and making it suitable for wide adoption. 
% \rg{[It's not really clear that this is for a specific target data set]}




==> archive/4-arch.tex <==
\section{Anda Architecture} \label{sec:arch}

% In this section, we present the Anda Architecture, a computing system designed to optimize LLM inference using the Anda Format. The architecture is characterized by three key components: 1) A variable-length activation data layout in \ms{on-chip} memory storage, 2) a bit-serial mantissa dot-product computation unit, and 3) a runtime bit-plane compressor for output activations.
% These components jointly enhance storage efficiency, computational performance, and energy conservation for LLM deployment.
\rTwoFC{In this section, we first present the three key components of the Anda architecture: (a) A variable-length activation data layout in on-chip memory storage, (b) an Anda-enhanced bit-serial processing unit, and (c) a runtime bit-plane compressor for output activations. These components collectively enhance storage efficiency, computational performance, and energy conservation. Finally, we present how these components integrate to form the overall Anda architecture, a computing system designed to optimize LLM inference using the Anda format.}

% \rOneFC{The Anda architecture enhances memory utilization via a bit-plane data layout scheme, improves FP-INT GeMM efficiency using mantissa-bit-serial DPUs, and reduces data transfer overhead through on-the-fly bit-plane compression. \as{The described architecture can be extended to any group size.} These innovations, detailed in subsequent sections, enable flexible adaptation to various LLM inference tasks.}


\subsection{Bit-plane Data Layout Scheme} \label{subsec:scheme}

%\rOneFC{Efficient data layout is crucial in LLM inference, which directly impacts memory bandwidth utilization and computation efficiency. 
\ms{Anda-based activation values feature a variable-length mantissa, necessitating careful data layout arrangement in the on-chip buffer to maintain regular memory access. Otherwise, irregular memory accesses caused by an ineffective data layout could completely undo the benefits provided by Anda.}

%\TODO{Prior fixed-length data arrangement methods~\cite{noh2023flexblock, kim2024isca, sharma2018bit, huang2024precision} struggle to balance storage efficiency and computational flexibility for variable-length activation values with varying precision requirements, often leading to suboptimal memory resource utilization.}}

% The bit-plane data layout scheme, as shown in Fig.~\ref{fig:mem_layout}, is designed to efficiently handle variable-length Anda format data while minimizing storage overhead and maximizing data access efficiency. This scheme addresses the challenges posed by the variable precision nature of Anda format activations by introducing a novel approach to data organization.

\rOneFC{To tackle these challenges, we propose the bit-plane data layout scheme as illustrated in Fig.~\ref{fig:mem_layout}.}
\rOneFC{\ms{Unlike prior fixed-length data arrangement methods~\cite{noh2023flexblock, kim2024isca, sharma2018bit, huang2024precision}}, \ms{which treat each FP data element as an \rg{atomic}
%integrated
unit,}
our approach separates and reorganizes the sign bit, mantissa, and exponent of FP numbers within grouped data blocks from a bit-plane view.}
\rOneFC{A transposed data arrangement is introduced where bits of the same significance across multiple numbers are packed together to \ms{keep the regularity of memory access.}
\ms{Taking the common memory bank word width into account, 64 Anda-type values are grouped to implement the bit-plane data layout scheme.}}
%{optimize storage and access efficiency with flexibility in adapting to different variable-length Anda formats.}
\rOneFC{As shown in Fig.~\ref{fig:mem_layout}, Group \#0 shows the layout for 4-bit mantissa Anda numbers, while Group \#1 presents the arrangement for 5-bit mantissa Anda numbers. \ms{The variable mantissa length only reflects on the different memory address depths, without impacting memory bandwidth utilization, and can be easily managed during address generation.} 
Therefore, in both cases, the bit-plane data layout efficiently accommodates these formats with varying lengths, maintaining consistent access patterns.}

\rOneFC{Note that INT weights can similarly utilize this data layout scheme to address the increasingly aggressive pursuit of weight-only quantization from INT4~\cite{shao2024omniquant} to INT1~\cite{xu2024onebit} in current LLM inference.}
\rOneFC{Furthermore, the bit-plane organization inherently facilitates parallel processing, inspiring the design of a novel processing unit for the Anda data format to enhance LLM inference in both computing and energy efficiency.}
\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.92\linewidth]{figs/mem_layout_v2.pdf}
    % \caption{Efficient data storage layout scheme for INT4 weights and Anda activations. \TODO{The caption to be replaced.}}
    \caption{The proposed bit-plane data layout scheme in memory for efficient variable-length activation data storage.}
    \label{fig:mem_layout}
\end{figure}

%\ms{repeated with previous sentences, so comment out}
%\rOneFC{The bit-plane data layout scheme effectively addresses the challenges faced by prior fixed-length data arrangement methods, balancing storage efficiency and computational flexibility for variable-length Anda activation values.}

% Moreover, our scheme's bit-plane organization naturally facilitates parallel processing, motivating the design of a novel processing unit for Anda values to further improve LLM inference efficiency.}

% At the core of this layout scheme is the separation of exponents and mantissas. The exponents, each 5 bits wide (denoted as $e_0$), are stored separately from the mantissas. The key innovation lies in the bit-plane organization of mantissas, which significantly improves storage utilization. Rather than allocating fixed-width blocks for each activation, which would result in wasted space due to varying mantissa lengths, this scheme packs mantissa bits efficiently across the entire allocated space. In the optimized layout, activation mantissas ($a_0$ to $a_{63}$) are stored contiguously, with sign bits ($s$) preceding each mantissa. This approach ensures full utilization of each 64-bit block, eliminating the waste seen in naive implementations. The variable-length nature of Anda format is accommodated by allowing mantissas to span across block boundaries seamlessly, enabling efficient storage of activations with different precisions.

% Complementing the activation data layout, the scheme also addresses the storage of INT4 weights. It organizes 64 weight values ($w_0$ to $w_{63}$) in each 64-bit block, aligning with the activation group size used in computations. This alignment facilitates efficient data retrieval and processing during matrix operations. \rg{[This is not clear to me yet, maybe the new fig. 11 will help]}

% The advantages of this layout scheme are manifold. By eliminating wasted bits in mantissa storage, it significantly decreases the overall memory footprint. The contiguous storage of mantissa bits allows for efficient retrieval of variable-length data, improving data access efficiency. Furthermore, the 64-value grouping in both activation and weight storage aligns well with the dot-product units in the MXU, facilitating smooth data flow during computations.

% Through this innovative approach to data organization, the bit-plane data layout scheme contributes significantly to the overall efficiency of the Anda architecture. It addresses the critical challenges of reducing memory bandwidth requirements and enhancing computational throughput, making it an essential component in optimizing large language model inference.

% \subsection{Mantissa-bit-serial Anda Processing Element} \label{subsec:dpu}
% \subsection{Mantissa-bit-serial Dot-Product Unit} \label{subsec:dpu}
\subsection{Anda-enhanced Bit-serial Processing Unit} \label{subsec:dpu}

% \TODO{Would it be better if we change a subtitle like Anda Processing Unit?}

% The Mantissa-bit-serial Dot-product Unit (DPU) is the core computational element of the Anda architecture, designed to efficiently handle dot-product operations between variable-length Anda format activations and fixed-point weights. The DPU's key innovation lies in its bit-serial processing of mantissas, allowing it to flexibly adapt to Anda format data of varying lengths without additional adjustments. This design directly addresses the challenge of dynamic precision in LLM inference.

% \rOneFC{The mantissa-bit-serial DPU serves as the key computational component of the Anda architecture, optimized for efficient dot-product operations between variable-length Anda format activations and INT weights.}
% \rOneFC{It is built upon the bit-plane data layout scheme, enabling high computational efficiency.}
% \rOneFC{At the core of the DPU lies the Anda processing element (PE), seamlessly embedded within a conventional FP fused multiply-add (FMA) unit.}
% \rOneFC{This integration extends support for the Anda format while preserving existing FP capabilities, allowing the Anda PE to efficiently perform FP-INT dot-product operations within an Anda group.}

\rOneFC{The Anda-enhanced bit-serial processing unit (APU), as depicted in Fig.~\ref{fig:dpu_pattern}, serves as the key computational element of the Anda architecture, embracing Anda processing element (PE) and an FP accumulator. Anda PE efficiently executes dot-product operations between variable-length Anda format activations and INT weights, seamlessly integrating with the bit-plane data layout scheme to enhance performance.}
\rTwoFC{The FP accumulator follows the PE to complete the APU functionality by accumulating the cross-group dot-product results.}
% A conventional FP fused multiply-add (FMA) unit follows the PE to complete the DPU functionality and provide support for traditional FP multiply accumulate operations.}

\rOneFC{The computation process begins with the Anda PE storing the sign and exponent in internal registers.}
\rOneFC{Concurrently, the INT weights are stored in the PE using a double-buffer design, allowing overlapped weight loading and computation to minimize loading latency.}
\rOneFC{The PE then loads the bit-plane mantissas and performs computations with the INT weights. By employing bit-serial processing of mantissas, the Anda PE can adapt to Anda format data of varying lengths without additional hardware overhead.}

% \rOneFC{A key feature of the Anda PE is its implementation of a first-element-then-bit-plane reduction pattern. In this approach, a partial sum is obtained for each bit-plane by accumulating all elements within that bit-plane using an adder tree. This method offers several advantages. First, it reduces storage requirements by storing only one partial sum per bit-plane instead of all intermediate results. Second, it minimizes data movement and processing overhead by performing subsequent shift operations only on the single partial sum rather than individual elements. Finally, it significantly reduces hardware resource consumption by using a single shared accumulator for all bit-plane accumulations.}

\rOneFC{To further optimize hardware efficiency, the Anda PE implements a first-element-then-bit-plane reduction pattern. In this approach, a partial sum is obtained for each bit-plane by accumulating all elements within that bit-plane using an adder tree. This method reduces storage requirements by storing only one partial sum per bit-plane instead of all intermediate results. It also minimizes data movement and processing overhead by performing subsequent shift operations only on the single partial sum rather than individual elements. Furthermore, it significantly reduces hardware resource consumption by using a single shared accumulator for all bit-plane accumulations.}

\rOneFC{The bit-plane partial sums are then sequentially accumulated to complete the dot-product operation. Upon completion, the Anda PE dynamically shifts the dot-product result based on the Anda mantissa length and converts it to FP16 using the shared exponent. The result is then multiplied with the group-wise scale factor of the INT weights, followed by cross-group accumulation using the FP accumulator. Finally, the accumulated FP32 result is converted to FP16 for output.}
% Conventional dot-product computation units typically employ a first-bit-plane-then-element reduction pattern, as shown in Fig.~\ref{fig:dpu_pattern}(a). In this approach, each activation's mantissa bits are first multiplied with corresponding weights, followed by bit-plane level reduction, and finally element-wise reduction. While intuitive, this method has significant drawbacks when processing variable-length mantissas: it generates excessive intermediate results, increases data movement overhead, and leads to inefficient computation, \rg{[Elaborate a bit more why this is the case?]} especially for large-scale matrix operations \rg{[Why does this chnage for larger matrices?]}. Crucially, this design requires an independent accumulator for each element, substantially increasing hardware costs.

% To overcome these limitations, we propose an innovative first-element-then-bit-plane reduction pattern, illustrated in Fig.~\ref{fig:dpu_pattern}(b). This design reverses the traditional approach by first performing element-wise multiplication and reduction, followed by bit-plane level operations. This method effectively reduces intermediate result storage requirements and simplifies data flow paths, significantly enhancing computational efficiency. The most notable improvement is that our design requires only one shared accumulator to complete calculations for the entire group, greatly reducing hardware resource consumption. \rg{[After reading this paragraph, it seems trivial to do element-then-bit-plane reduction, yet this is your innovation. Why is bit-plane-then-element reduction the default? Maybe highlight more than the advantage of bit-plane-then-element is specific to the variable bit-width]}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.96\linewidth]{figs/dpu_pattern_v2.pdf}
    % \caption{(a) first-bit-plane-then-element reduction pattern; (b) first-element-then-bit-plane reduction pattern. \TODO{To be replaced.}}
    \caption{The architecture of Anda-enhanced bit-serial processing unit, which enables efficient dot-product operations for Anda activations and INT weights.}
    \label{fig:dpu_pattern}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/bpc.pdf}
    \caption{The architecture of the on-the-fly bit plane compressor and the mantissa alignment process performed in the parallel-to-serial mantissa aligner.}
    \label{fig:bpc}
\end{figure}

\subsection{On-the-fly Bit-plane Compressor} \label{subsec:comp}
% \TODO{Please skip this subsection until it is rebuilt.}

% The on-the-fly bit-plane compressor is a key component of the Anda architecture, designed to convert FP16 activation values into the compressed Anda format in real-time \rg{[On-the-fly]}. This component efficiently addresses the challenges of \rg{variable-width} activation storage and transfer in LLM inference.

\rOneFC{The bit-plane compressor (BPC) is a critical component of the Anda architecture, enabling on-the-fly conversion of FP16 activation values into the compressed Anda format. It efficiently addresses the challenges of variable-length Anda activation storage and transfer in LLM inference by processing a large number of activation values in parallel and outputting them in a bit-serial manner.}

% The compressor employs a highly parallel structure, processing 1024 FP16 inputs \rg{[In the diagram, it is not clear whether the input is 1024 bit or 1024x16 bit. Is it possible to show the bit-sequential nature?]} simultaneously through 16 channels, each handling 64 values. The FP Data Extractor initiates the process by decomposing each FP16 input into its sign, exponent, and mantissa components. Within each channel, the maximum exponent is determined, serving as a shared exponent for all 64 values in a block.

\rOneFC{Fig.~\ref{fig:bpc} illustrates the architecture of the proposed BPC.}
\rOneFC{It consists of 16 parallel lanes, each capable of processing 64 grouped FP16 values simultaneously. Within each lane, the FP field extractor decomposes the FP16 inputs into their sign, exponent, and mantissa components. 
The maximum exponent catcher identifies the maximum exponent within a grouped lane, and then calculates the difference of each exponent to the shared maximum exponent.}
% \rOneFC{The core of the compression process lies in the mantissa alignment, performed by the parallel-to-serial mantissa aligner. 
% It calculates the difference between each input's exponent and the lane's maximum exponent, determining the left-shift amount for each mantissa. 
% As illustrated in Fig.~\ref{fig:bpc}, the mantissa bits are shifted out serially over multiple cycles based on the calculated exponent difference. In each cycle, a counter is compared with each element's difference in exponent value to determine whether the mantissa should be left-shifted or remain unchanged.}

% \rOneFC{The core of the compression process lies in the mantissa alignment performed by the parallel-to-serial mantissa aligner. As shown in Fig.~\ref{fig:bpc}, the aligner shifts out mantissa bits serially over multiple cycles, with the shift amount determined by comparing a cycle counter with each element's exponent difference.}
\rOneFC{The core of the compression process lies in the mantissa alignment performed by the parallel-to-serial mantissa aligner. 
% In each cycle, the aligner compares a counter value with each element's exponent difference to determine whether the most significant mantissa bit should be shifted out or remain unchanged, as illustrated in Fig.~\ref{fig:bpc}.
\rTwoFC{As shown in Fig.~\ref{fig:bpc}, in each cycle, each element's exponent difference decreases by one until it reaches zero. When the exponent difference is zero, the most significant mantissa bit of that element should be shifted out each cycle; otherwise, it remains unchanged and output zero.}
\rTwoFC{The shifted-out bits among each element in the lane are packed into the bit-plane aligned mantissa.}
This process continues for multiple cycles until the number of output bit-planes reaches the configurable mantissa length.}
\rOneFC{The parallel-to-serial mantissa alignment process generates compressed bit-planes directly. The resulting bit-serial output, along with the sign bits and shared maximum exponents from all lanes, is passed to the data packager unit. This unit assembles the final compressed output in a format compatible with the proposed bit-plane compression scheme.}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.98\linewidth]{figs/arch.pdf}
    \caption{Anda system architecture.}
    \label{fig:arch}
\end{figure}

\subsection{Overall Architecture} 
% \ms{Move this to the last subsection, and add some context for dataflow}
\label{subsec:overall}

% Fig.~\ref{fig:arch} illustrates the Overall Architecture of Anda. The memory system comprises three components: the instruction memory for storing execution instructions, the activation buffer for efficient storage of variable-length Anda format activation data, and the Weight Buffer for 4-bit quantized weight parameters.
% A top controller coordinates operations, managing instruction execution and data interaction between buffers and external memory. The Matrix Computation Unit (MXU) performs efficient calculations using Anda format activation data and INT4 fixed-point weights.
% To optimize storage and reduce memory access overhead, a Bit-plane compressor converts FP16 computation results into the Anda data format on-the-fly. 
% A SIMD-style vector unit handles non-linear function calculations in Transformer Blocks, including activation functions, softmax, and LayerNorms.
% These components work in concert through carefully designed data flow and control logic. 
% The Anda Architecture's approach to handling variable precision data and its optimizations across computation, storage, and data transfer enable it to support various scales and types of LLMs.

\rOneFC{Fig.~\ref{fig:arch} illustrates the overall architecture of Anda, which includes the top controller, address generator, activation buffer, weight buffer, matrix computation unit (MXU), vector unit, and bit-plane compressor.}
The LLM inference is orchestrated as follows: \rOneFC{\ding{182} Initially, the instruction memory is programmed through the I/O interface of the top controller, which governs the address generator during operation.}
\rOneFC{\ding{183} The address generator produces read and write addresses for both activation and weight buffers.} %ensuring efficient dataflow.}
\rTwoFC{Both the activation buffer and weight buffer follow the proposed bit-plane-based data layout for efficient data handling.}
% \rOneFC{\ding{184} The MXU, featuring a 16$\times$16 dot-product unit (DPU) array, performs matrix computations with dedicated \ms{data} dispatchers for Anda activations and INT4 weights, with each DPU supporting 64-element grouped FP-INT dot-product operations.}
\rTwoFC{\ding{184} The MXU, featuring a 16$\times$16 APU array, performs FP-INT GeMM operations following typical output stationary dataflow~\cite{lee2024tender}.}
\rTwoFC{The weight data dispatcher, equipped with registers, allows overlapping weight loading and computation, broadcasting weights row-wise to each APU for data reuse. 
The activation data dispatcher supplies a bit-plane vector of activations each cycle, sequentially feeding it into the MXU and sharing it across columns to maximize input reuse and enable multiple calculations with the same input.}
%\ms{I think current contents are enough}
% \rOneFC{Me too. Yeaaaaah :)!}
% \rTwoFC{The Anda PE in each DPU performs 64-element grouped FP-INT dot-product operations in a bit plane per cycle, and the when dot-product result within a group is completed, then it will pass to the FP unit in the DPU to perform cross-group accumulation.}
% \rTwoFC{The Anda PE in each DPU performs 64-element grouped FP-INT dot-product operations in a bit plane per cycle. When the dot-product result within a group is completed, it is passed to the FP unit in the DPU to perform cross-group accumulation.
\rTwoFC{Upon completing the GeMM computation, the output results are delivered to the BPC via the output data dispatcher.}
% \rTwoFC{Finally, each DPU }
% \rTwoFC{In this way, when DPUs finishes to compute an output element of the GeMM, the output activation results are delivered to the BPC via output data dispatcher.}
%\ms{This is toooo long...,can you just find some similar works, say something like: we adopt xx-based dataflow? no need 100\% fill in all pages...it is okay to leave some spaces. Don't you think this part is too heavy compared with others?}
% \rTwoFC{But we indeed require these sentences to fill in 11 pages? =.= Ok.}
\rOneFC{\ding{185}~Complementing MXU, the vector unit processes the non-linear functions of the transformer block.}
\rOneFC{\ding{186}~FP16 outputs of MXU or vector unit can be optionally compressed to Anda format by the BPC, optimizing storage efficiency.}
\rOneFC{\ding{187}~Processed \ms{outputs are} %data is 
written back to the activation buffer.
\ding{188}~Finally, activation results are transferred %back
to external memory for subsequent operations.} 
% \rOneFC{The overall architecture effectively enhances memory utilization, improves the computational efficiency of FP-INT GeMMs, reduces data transfer overhead, and adapts seamlessly to various LLM structures.}
% \rOneFC{The Anda architecture enhances memory utilization via a bit-plane data layout scheme, improves FP-INT GeMM efficiency using mantissa-bit-serial DPUs, and reduces data transfer overhead through on-the-fly bit-plane compression. \as{The described architecture can be extended to any group size.} These innovations, detailed in subsequent sections, enable flexible adaptation to various LLM inference tasks.}
% \rOneFC{\ding{182}} The top controller orchestrates the overall operation, interfacing with the instruction memory via I/O for system programming. 

% The Anda Architecture presents an innovative approach to optimizing LLM inference, addressing critical challenges in memory bandwidth, computational efficiency, and energy consumption. At its core, this architecture leverages the variable-precision Anda Format for end-to-end optimization across data representation, computation, and storage. Fig.~\ref{fig:arch} illustrates the overall architecture of Anda. A sophisticated control system, centered around a top controller, manages instruction execution and coordinates data flow, controlling address generators for both activation and weight buffers to facilitate efficient data loading and direction. The heart of the computation lies in the Matrix Computation Unit (MXU), which exploits the variable-length nature of the Anda format \rg{[Be consistent in Format with capital F]} to efficiently perform matrix calculations between Anda-formatted activations and INT4 fixed-point weights. Adopting an output-stationary design with 16x16 mantissa-bit-serial dot-product units (DPUs), the MXU computes dot products for Anda activations and INT weights with a group size of 64, while integrated data dispatchers and collectors ensure smooth data flow. To further optimize storage and memory access, an on-the-fly Bit-plane Compressor efficiently converts FP16 computation results from the MXU into the Anda data format. Complementing these components, a SIMD-style Vector Unit handles non-linear function computations in Transformer Blocks, including activation functions, softmax, and LayerNorms. This integrated system design enables Anda Architecture \rg{[is there a difference between the integrated system design and the Anda Architecure?]}to achieve substantial improvements in overall efficiency and performance, offering a promising solution for enhancing LLM deployment across diverse applications. \rg{[This integrated system maximally exploits the benefits of the Anda Format, bringing substantial improvements in overall efficiency and performance and offering a promising solution for enhanced LLM deployment across diverse applications.]}


==> archive/5-eval.tex <==
\section{Evaluation} \label{sec:eval}

\subsection{Experimental Setup}

%\textbf{Software Implementation.} 
% \ms{\textbf{LLM Benchmarks:}}
% %Our algorithm is implemented using the PyTorch framework and the Hugging Face library. 
% To demonstrate the broad applicability of our proposed method, we \ms{benchmark}
% %evaluate its performance on 
% various \ms{open-source} PyTorch language models from the OPT~\cite{zhang2022opt}, LLaMA~\cite{touvron2023llama}, and LLaMA2~\cite{touvron2023llama2} model families \ms{under WikiText-2~\cite{merity2017pointer}, Penn Treebank (PTB)~\cite{marcus1994penn}, and C4~\cite{raffel2020exploring} datasets}, \ms{with diverse model scale (1.3B to 30B parameters) and tasks.} %th with model sizes ranging from 1.3B to 30B parameters. 
%The main evaluation focuses on language modeling tasks using the WikiText-2~\cite{merity2017pointer}, Penn Treebank (PTB)~\cite{marcus1994penn}, and C4~\cite{raffel2020exploring} datasets. Perplexity, a widely adopted metric for autoregressive models, is used to measure model accuracy, where the lower the better.

\rOneFC{\textbf{LLM Benchmarks:} To demonstrate the wide applicability of our proposed method, we benchmark various open-source LLMs using PyTorch and Hugging Face libraries.}
% \rOneFC{We select models from the OPT~\cite{zhang2022opt}, LLaMA~\cite{touvron2023llama}, and LLaMA2~\cite{touvron2023llama2} families, evaluating their performance on the WikiText-2~\cite{merity2017pointer}, Penn Treebank (PTB)~\cite{marcus1994penn}, and C4~\cite{raffel2020exploring} datasets.}
% \rOneFC{The selected models range in size from 1.3B to 30B parameters, showcasing the effectiveness of our method across different scales.}
\rOneFC{We evaluate their performance on WikiText-2~\cite{merity2017pointer}, Penn Treebank (PTB)~\cite{marcus1994penn}, and C4~\cite{raffel2020exploring} datasets. The models used in our benchmarks range in size from 1.3B to 30B parameters and are selected from OPT~\cite{zhang2022opt}, LLaMA~\cite{touvron2023llama}, and LLaMA2~\cite{touvron2023llama2} families, enabling the effectiveness assessment of our method across different model scales and architectures.}

% \textbf{Quantization Baselines:}
% \ms{For the precision validation of Anda format, the \ms{model accuracy of} all benchmarks optimized based on Anda are hence compared with its SotA competitors, including 
% %We compare the model accuracy of our Adna scheme with a variety of prior arts towards weight-only quantized LLMs.
% %We leverage the 
% a) Full precision baseline where activation and weight are both in FP16;
% b) post-training quantization: Omniquant~\cite{shao2024omniquant} with quantization W4A16g128 (4-bit weight-only quantization with a
% 128-group size); FIGNA~\cite{jang2024figna} realizing lossless BFP quantization with hardware architectural support. c) quantization-aware training: VS-Quant~\cite{keller202395} achieving aggressive quantization for activation and weight through costly retaining.}

\rOneFC{\textbf{Quantization Baselines:}
% To validate the model accuracy when replacing FP activations with the Anda format, we compare all benchmarks optimized with Anda against the following SotA competitors:
To validate the model accuracy when replacing FP activations with the proposed Anda format, we compare against the following SotA competitors:
% To compare the model accuracy when replacing FP activations with the proposed Anda format, we evaluate it against the following SotA competitors:
(a) Full-precision baseline where both activations and weights are represented in FP16.
(b) Weight-only quantization baseline using Omniquant~\cite{shao2024omniquant} with W4A16g128 scheme, which uses 4-bit weight quantization with a group size of 128. 
(c) Lossless BFP baseline that adopts FIGNA's~\cite{jang2024figna} approach of using extended mantissa lengths to maintain model accuracy.
(d) Aggressive BFP baseline that employs 4-bit mantissa to activations using VS-Quant~\cite{dai2021vs} quantization scheme. 
% While VS-Quant typically requires costly retraining, which is impractical for agile LLM deployment, we directly convert FP activations to BFP for evaluation.
Since VS-Quant typically requires costly retraining, making it impractical for agile LLM deployment, we bypass this step by directly converting to BFP activations.
% Although VS-Quant traditionally involves costly retraining, making it impractical for agile LLM deployment, we bypass this step by directly converting FP activations to BFP for our evaluation.
For baseline (c), (d), and our Anda method, we use baseline (b) as the starting point, and the group size of BFP activations is uniformly set to 64.}

%another baseline we consider, uses BFP to quantize both activations and weights to 4-bit. However, it requires costly retraining, which is impractical for rapid LLM deployment. Thus, we apply VS-Quant's scheme post-training to our weight-only quantized LLMs.
%\cite{shao2024omniquant,lin2024awq,frantar2023optq,lin2024qserve,zhao2024atom}, where weights are quantized to 4-bit INT precision in groups of 128, and activations are kept at 16-bit FP.
%floating-point precision.
%For software-only quantization work, we compare with Omniquant~\cite{shao2024omniquant}, which provides us the state-of-the-art post-training weight-only quantized models for deployment.
%\ms{Feel no need to talk Omniquant separately}
% We further leverage FIGNA~\cite{jang2024figna} on these W4A16 quantized LLMs produced by Omniquant.
%\rg{[As a baseline, ]}
%We further apply FIGNA~\cite{jang2024figna} \rg{[What does 'apply' mean here?]} to these LLMs quantized by Omniquant, which enables lossless post-training BFP quantization with hardware architectural support.
%VS-Quant~\cite{dai2021vs}, another baseline we consider, uses BFP to quantize both activations and weights to 4-bit. However, it requires costly retraining, which is impractical for rapid LLM deployment. Thus, we apply VS-Quant's scheme post-training to our weight-only quantized LLMs.

%\textbf{Hardware Implementation.} 
% \textbf{Hardware Baselines:} 
% \ms{To further highlight the advantages of the Anda scheme, Anda hardware, an architecture with compatible computation and memory access optimized by the Anda data type, is compared with a set of LLM inference hardware platforms, including: a) Existing standard GPU with FP-FP ALUs~\cite{sun2022dissecting}. b) GPU-like design featuring specialized FP-INT computation units. c) Y. Kim's architecture~\cite{kim2023winning} which utilizes bit-serial computation on INT weights and dynamically converts FP activations to BFP with an extended mantissa. d) FIGNA~\cite{jang2024figna}, a successor to Y. Kim's work, employs bit-parallel computation and reduces mantissa bit length in BFP to optimize computation costs. All systems are evaluated with an equivalent number of processing elements and on-chip memory resources, ensuring a fair comparison.}

\rOneFC{\textbf{Hardware Baselines:} To further highlight the advantages of the Anda scheme, we compare the Anda hardware
% —an architecture optimized for computation and memory access using the Anda data format—
architecture against several SotA platforms:
(a) FP-FP: A spatial accelerator based on FP16 Tensor Cores~\cite{zadeh2022mokey}, representative of current GPU architectures~\cite{sun2022dissecting}.
(b) FP-INT: An enhanced Tensor Core-based accelerator featuring specialized FP-INT computation units.
(c) Y. Kim et al.~\cite{kim2023winning}: A spatial accelerator employs bit-serial computation for INT weights and dynamically converts FP activations to BFP format with extended mantissa before computation.
(d) FIGNA~\cite{jang2024figna}: An evolution of (c) leveraging bit-parallel computation and optimized mantissa length in BFP to enhance computational efficiency.
All systems are configured to have equivalent peak throughput and on-chip memory resources to ensure a fair comparison~\cite{shi2024bitwave}.}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table]{xcolor}
\begin{table*}[htbp]
\centering
% \caption{Comparison of computation methods of weight-only quantized LLMs \\ Key Metrics: Perplexity (Black, lower is better), \textcolor[HTML]{3A9262}{Accuracy Drop (Green)} and \textcolor{red}{BOPs Reduction (Red)}}
\caption{Comparison of computation methods for weight-only quantized LLMs \\ Key Metrics: Perplexity (Black, lower is better), \textcolor{red}{Accuracy Drop (Red)} and \textcolor[HTML]{3A9262}{BOPs Reduction (Green)}}
\label{tab:algo_res}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll|*{9}{l}@{}}
\toprule
\multicolumn{2}{c|}{} & OPT-1.3B & OPT-2.7B & OPT-6.7B & LLaMA-7B & LLaMA2-7B & OPT-13B & LLaMA-13B & LLaMA2-13B & OPT-30B \\ \midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{WikiText2}} & FP16 & ${14.62}$ & ${12.47}$ & ${10.86}$ & ${5.68}$ & ${5.47}$ & ${10.13}$ & ${5.09}$ & ${4.88}$ & ${9.56}$ \\ 
& Omniquant~\cite{shao2024omniquant} & ${14.88}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${12.65}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.96}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.77}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.59}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.20}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.17}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${4.95}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${9.62}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
& FIGNA~\cite{jang2024figna} & ${14.90}^{\textcolor{red}{-0.13\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${12.65}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.96}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.78}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.60}^{\textcolor{red}{-0.18\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.22}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.18}^{\textcolor{red}{-0.19\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${4.96}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${9.61}^{\textcolor{red}{0.10\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
& VS-Quant~\cite{keller202395} & ${19.04}^{\textcolor{red}{-27.96\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${16.41}^{\textcolor{red}{-22.91\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.24}^{\textcolor{red}{-11.68\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${7.45}^{\textcolor{red}{-29.12\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.26}^{\textcolor{red}{-47.76\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${11.63}^{\textcolor{red}{-13.98\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${6.36}^{\textcolor{red}{-23.02\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${6.43}^{\textcolor{red}{-29.90\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${10.67}^{\textcolor{red}{-10.91\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
& Ours (0.1\%) & \cellcolor{yellow!30}${14.91}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{2.74\times}}$ & \cellcolor{yellow!30}${12.66}^{\textcolor{red}{-0.07\%}}_{\textcolor[HTML]{3A9262}{2.91\times}}$ & \cellcolor{yellow!30}${10.95}^{\textcolor{red}{0.09\%}}_{\textcolor[HTML]{3A9262}{3.10\times}}$ & \cellcolor{yellow!30}${5.78}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{1.99\times}}$ & \cellcolor{yellow!30}${5.60}^{\textcolor{red}{-0.18\%}}_{\textcolor[HTML]{3A9262}{1.96\times}}$ & \cellcolor{yellow!30}${10.21}^{\textcolor{red}{-0.10\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!30}${5.18}^{\textcolor{red}{-0.19\%}}_{\textcolor[HTML]{3A9262}{1.88\times}}$ & \cellcolor{yellow!30}${4.96}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.80\times}}$ & \cellcolor{yellow!30}${9.60}^{\textcolor{red}{0.20\%}}_{\textcolor[HTML]{3A9262}{3.10\times}}$ \\ 
& Ours (1\%) & \cellcolor{yellow!90}${14.99}^{\textcolor{red}{-0.74\%}}_{\textcolor[HTML]{3A9262}{2.95\times}}$ & \cellcolor{yellow!90}${12.76}^{\textcolor{red}{-0.86\%}}_{\textcolor[HTML]{3A9262}{3.25\times}}$ & \cellcolor{yellow!90}${10.99}^{\textcolor{red}{-0.27\%}}_{\textcolor[HTML]{3A9262}{3.31\times}}$ & \cellcolor{yellow!90}${5.82}^{\textcolor{red}{-0.87\%}}_{\textcolor[HTML]{3A9262}{2.56\times}}$ & \cellcolor{yellow!90}${5.65}^{\textcolor{red}{-1.07\%}}_{\textcolor[HTML]{3A9262}{2.56\times}}$ & \cellcolor{yellow!90}${10.30}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{3.20\times}}$ & \cellcolor{yellow!90}${5.23}^{\textcolor{red}{-1.16\%}}_{\textcolor[HTML]{3A9262}{2.59\times}}$ & \cellcolor{yellow!90}${5.00}^{\textcolor{red}{-1.01\%}}_{\textcolor[HTML]{3A9262}{2.44\times}}$ & \cellcolor{yellow!90}${9.71}^{\textcolor{red}{-0.94\%}}_{\textcolor[HTML]{3A9262}{3.31\times}}$ \\ 
\midrule 
\multirow{6}{*}{\rotatebox[origin=c]{90}{PTB}} & FP16 & ${16.96}$ & ${15.12}$ & ${13.09}$ & ${8.80}$ & ${20.82}$ & ${12.34}$ & ${8.07}$ & ${28.93}$ & ${11.84}$ \\ 
& Omniquant~\cite{shao2024omniquant} & ${17.40}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${15.28}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${13.25}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${8.97}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${21.52}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${12.46}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${8.14}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${30.19}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.94}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
& FIGNA~\cite{jang2024figna} & ${17.41}^{\textcolor{red}{-0.06\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${15.28}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${13.26}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${8.98}^{\textcolor{red}{-0.11\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${21.52}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${12.47}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${8.15}^{\textcolor{red}{-0.12\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${30.19}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.95}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
& VS-Quant~\cite{keller202395} & ${25.64}^{\textcolor{red}{-47.36\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${21.09}^{\textcolor{red}{-27.55\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${15.50}^{\textcolor{red}{-16.98\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${15.78}^{\textcolor{red}{-75.92\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${53.46}^{\textcolor{red}{-148.42\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${14.47}^{\textcolor{red}{-16.13\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.54}^{\textcolor{red}{-54.05\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${49.91}^{\textcolor{red}{-65.32\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${13.47}^{\textcolor{red}{-12.81\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
& Ours (0.1\%) & \cellcolor{yellow!30}${17.41}^{\textcolor{red}{-0.06\%}}_{\textcolor[HTML]{3A9262}{1.64\times}}$ & \cellcolor{yellow!30}${15.29}^{\textcolor{red}{-0.07\%}}_{\textcolor[HTML]{3A9262}{2.13\times}}$ & \cellcolor{yellow!30}${13.26}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${8.98}^{\textcolor{red}{-0.11\%}}_{\textcolor[HTML]{3A9262}{2.21\times}}$ & \cellcolor{yellow!30}${21.48}^{\textcolor{red}{0.20\%}}_{\textcolor[HTML]{3A9262}{2.19\times}}$ & \cellcolor{yellow!30}${12.47}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.84\times}}$ & \cellcolor{yellow!30}${8.15}^{\textcolor{red}{-0.12\%}}_{\textcolor[HTML]{3A9262}{2.35\times}}$ & \cellcolor{yellow!30}${30.18}^{\textcolor{red}{0.03\%}}_{\textcolor[HTML]{3A9262}{2.84\times}}$ & \cellcolor{yellow!30}${11.96}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ \\ 
& Ours (1\%) & \cellcolor{yellow!90}${17.57}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.31\times}}$ & \cellcolor{yellow!90}${15.42}^{\textcolor{red}{-0.91\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${13.35}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${9.05}^{\textcolor{red}{-0.89\%}}_{\textcolor[HTML]{3A9262}{2.54\times}}$ & \cellcolor{yellow!90}${21.61}^{\textcolor{red}{-0.42\%}}_{\textcolor[HTML]{3A9262}{2.39\times}}$ & \cellcolor{yellow!90}${12.58}^{\textcolor{red}{-0.96\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${8.22}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${30.41}^{\textcolor{red}{-0.73\%}}_{\textcolor[HTML]{3A9262}{2.92\times}}$ & \cellcolor{yellow!90}${12.03}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ \\ 
\midrule 
\multirow{6}{*}{\rotatebox[origin=c]{90}{C4}} & FP16 & ${14.72}$ & ${13.16}$ & ${11.74}$ & ${7.08}$ & ${6.97}$ & ${11.20}$ & ${6.61}$ & ${6.47}$ & ${10.69}$ \\ 
& Omniquant~\cite{shao2024omniquant} & ${15.03}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${13.38}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.85}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${7.21}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${7.12}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.29}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${6.69}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${6.56}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.75}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
& FIGNA~\cite{jang2024figna} & ${15.04}^{\textcolor{red}{-0.07\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${13.38}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.86}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${7.22}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${7.12}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.29}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${6.70}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${6.57}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.75}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
& VS-Quant~\cite{keller202395} & ${19.00}^{\textcolor{red}{-26.41\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${16.65}^{\textcolor{red}{-19.64\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${13.13}^{\textcolor{red}{-10.80\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.89}^{\textcolor{red}{-23.30\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${10.36}^{\textcolor{red}{-45.51\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.64}^{\textcolor{red}{-11.96\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${7.85}^{\textcolor{red}{-17.34\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.35}^{\textcolor{red}{-27.29\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${11.91}^{\textcolor{red}{-10.79\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
& Ours (0.1\%) & \cellcolor{yellow!30}${15.05}^{\textcolor{red}{-0.13\%}}_{\textcolor[HTML]{3A9262}{1.86\times}}$ & \cellcolor{yellow!30}${13.40}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{2.11\times}}$ & \cellcolor{yellow!30}${11.87}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${7.22}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{2.16\times}}$ & \cellcolor{yellow!30}${7.13}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{2.04\times}}$ & \cellcolor{yellow!30}${11.30}^{\textcolor{red}{-0.09\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${6.70}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{2.16\times}}$ & \cellcolor{yellow!30}${6.57}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{2.14\times}}$ & \cellcolor{yellow!30}${10.76}^{\textcolor{red}{-0.09\%}}_{\textcolor[HTML]{3A9262}{2.31\times}}$ \\ 
& Ours (1\%) & \cellcolor{yellow!90}${15.17}^{\textcolor{red}{-0.93\%}}_{\textcolor[HTML]{3A9262}{2.43\times}}$ & \cellcolor{yellow!90}${13.51}^{\textcolor{red}{-0.96\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${11.97}^{\textcolor{red}{-1.01\%}}_{\textcolor[HTML]{3A9262}{3.05\times}}$ & \cellcolor{yellow!90}${7.28}^{\textcolor{red}{-0.97\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${7.19}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${11.37}^{\textcolor{red}{-0.71\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${6.74}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${6.62}^{\textcolor{red}{-0.91\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${10.85}^{\textcolor{red}{-0.93\%}}_{\textcolor[HTML]{3A9262}{3.09\times}}$ \\ 
\bottomrule
\end{tabular}%
}
\end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \usepackage[table]{xcolor}
% \begin{table*}[t]
% \centering
% \caption{\TODO{We need a better caption.}Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better) and BOPS Reduction (\textcolor{red}{Red})}
% \label{tab:algo_res}
% \resizebox{0.92\textwidth}{!}{%
% \begin{tabular}{@{}ll|*{9}{l}@{}}
% \toprule
% \multicolumn{2}{c|}{} & OPT-1.3B & OPT-6.7B & LLaMA-7B & LLaMA2-7B & OPT-13B & LLaMA-13B & LLaMA2-13B & OPT-30B & LLaMA-30B \\ \midrule
% \multirow{6}{*}{\rotatebox[origin=c]{90}{WikiText2}} & FP16 & ${14.62}$ & ${10.86}$ & ${5.68}$ & ${5.47}$ & ${10.13}$ & ${5.09}$ & ${4.88}$ & ${9.56}$ & ${4.10}$ \\ 
% & Omniquant~\cite{shao2024omniquant} & ${14.88}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.96}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.77}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.59}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.20}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${5.17}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${4.95}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${9.62}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${4.19}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
% & FIGNA~\cite{jang2024figna} & ${14.90}^{\textcolor{red}{-0.13\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.96}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.78}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.60}^{\textcolor{red}{-0.18\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.22}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${5.18}^{\textcolor{red}{-0.19\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${4.96}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${9.61}^{\textcolor{red}{0.10\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${4.20}^{\textcolor{red}{-0.24\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
% & VSQuant~\cite{keller202395} & ${19.04}^{\textcolor{red}{-27.96\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.24}^{\textcolor{red}{-11.68\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${7.45}^{\textcolor{red}{-29.12\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.26}^{\textcolor{red}{-47.76\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${11.63}^{\textcolor{red}{-13.98\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${6.36}^{\textcolor{red}{-23.02\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${6.43}^{\textcolor{red}{-29.90\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${10.67}^{\textcolor{red}{-10.91\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${5.10}^{\textcolor{red}{-21.72\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
% & Ours (0.1\%) & \cellcolor{yellow!30}${14.91}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{2.74\times}}$ & \cellcolor{yellow!30}${10.95}^{\textcolor{red}{0.09\%}}_{\textcolor[HTML]{3A9262}{2.43\times}}$ & \cellcolor{yellow!30}${5.78}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{1.99\times}}$ & \cellcolor{yellow!30}${5.60}^{\textcolor{red}{-0.18\%}}_{\textcolor[HTML]{3A9262}{1.96\times}}$ & \cellcolor{yellow!30}${10.21}^{\textcolor{red}{-0.10\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!30}${5.18}^{\textcolor{red}{-0.19\%}}_{\textcolor[HTML]{3A9262}{1.88\times}}$ & \cellcolor{yellow!30}${4.96}^{\textcolor{red}{-0.20\%}}_{\textcolor[HTML]{3A9262}{1.80\times}}$ & \cellcolor{yellow!30}${9.60}^{\textcolor{red}{0.20\%}}_{\textcolor[HTML]{3A9262}{3.10\times}}$ & \cellcolor{yellow!30}${TBD}^{\textcolor{red}{\%}}_{\textcolor[HTML]{3A9262}{\times}}$ \\ 
% & Ours (1\%) & \cellcolor{yellow!90}${14.99}^{\textcolor{red}{-0.74\%}}_{\textcolor[HTML]{3A9262}{2.95\times}}$ & \cellcolor{yellow!90}${10.99}^{\textcolor{red}{-0.27\%}}_{\textcolor[HTML]{3A9262}{3.31\times}}$ & \cellcolor{yellow!90}${5.82}^{\textcolor{red}{-0.87\%}}_{\textcolor[HTML]{3A9262}{2.56\times}}$ & \cellcolor{yellow!90}${5.65}^{\textcolor{red}{-1.07\%}}_{\textcolor[HTML]{3A9262}{2.56\times}}$ & \cellcolor{yellow!90}${10.30}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{3.20\times}}$ & \cellcolor{yellow!90}${5.23}^{\textcolor{red}{-1.16\%}}_{\textcolor[HTML]{3A9262}{2.59\times}}$ & \cellcolor{yellow!90}${5.00}^{\textcolor{red}{-1.01\%}}_{\textcolor[HTML]{3A9262}{2.44\times}}$ & \cellcolor{yellow!90}${9.71}^{\textcolor{red}{-0.94\%}}_{\textcolor[HTML]{3A9262}{3.31\times}}$ & \cellcolor{yellow!90}${4.23}^{\textcolor{red}{-0.95\%}}_{\textcolor[HTML]{3A9262}{2.44\times}}$ \\ 
% \midrule 
% \multirow{6}{*}{\rotatebox[origin=c]{90}{PTB}} & FP16 & ${16.96}$ & ${13.09}$ & ${8.80}$ & ${20.82}$ & ${12.34}$ & ${8.07}$ & ${28.93}$ & ${11.84}$ & ${TBD}$ \\ 
% & Omniquant~\cite{shao2024omniquant} & ${17.40}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${13.25}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${8.97}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${21.52}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${12.46}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${8.14}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${30.19}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.94}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${7.39}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
% & FIGNA~\cite{jang2024figna} & ${17.41}^{\textcolor{red}{-0.06\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${13.26}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${8.98}^{\textcolor{red}{-0.11\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${21.52}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${12.47}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${8.15}^{\textcolor{red}{-0.12\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${30.19}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.95}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${7.40}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
% & VSQuant~\cite{keller202395} & ${25.64}^{\textcolor{red}{-47.36\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${15.50}^{\textcolor{red}{-16.98\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${15.78}^{\textcolor{red}{-75.92\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${53.46}^{\textcolor{red}{-148.42\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${14.47}^{\textcolor{red}{-16.13\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.54}^{\textcolor{red}{-54.05\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${49.91}^{\textcolor{red}{-65.32\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${13.47}^{\textcolor{red}{-12.81\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${9.92}^{\textcolor{red}{-34.24\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
% & Ours (0.1\%) & \cellcolor{yellow!30}${17.41}^{\textcolor{red}{-0.06\%}}_{\textcolor[HTML]{3A9262}{1.64\times}}$ & \cellcolor{yellow!30}${13.26}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${8.98}^{\textcolor{red}{-0.11\%}}_{\textcolor[HTML]{3A9262}{2.21\times}}$ & \cellcolor{yellow!30}${21.48}^{\textcolor{red}{0.20\%}}_{\textcolor[HTML]{3A9262}{2.19\times}}$ & \cellcolor{yellow!30}${12.47}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.84\times}}$ & \cellcolor{yellow!30}${8.15}^{\textcolor{red}{-0.12\%}}_{\textcolor[HTML]{3A9262}{2.35\times}}$ & \cellcolor{yellow!30}${30.18}^{\textcolor{red}{0.03\%}}_{\textcolor[HTML]{3A9262}{2.84\times}}$ & \cellcolor{yellow!30}${11.96}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${TBD}^{\textcolor{red}{\%}}_{\textcolor[HTML]{3A9262}{\times}}$ \\ 
% & Ours (1\%) & \cellcolor{yellow!90}${17.57}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.31\times}}$ & \cellcolor{yellow!90}${13.35}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${9.05}^{\textcolor{red}{-0.89\%}}_{\textcolor[HTML]{3A9262}{2.54\times}}$ & \cellcolor{yellow!90}${21.61}^{\textcolor{red}{-0.42\%}}_{\textcolor[HTML]{3A9262}{2.39\times}}$ & \cellcolor{yellow!90}${12.58}^{\textcolor{red}{-0.96\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${8.22}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${30.41}^{\textcolor{red}{-0.73\%}}_{\textcolor[HTML]{3A9262}{2.92\times}}$ & \cellcolor{yellow!90}${12.03}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${7.45}^{\textcolor{red}{-0.81\%}}_{\textcolor[HTML]{3A9262}{2.92\times}}$ \\ 
% \midrule 
% \multirow{6}{*}{\rotatebox[origin=c]{90}{C4}} & FP16 & ${14.72}$ & ${11.74}$ & ${7.08}$ & ${6.97}$ & ${11.20}$ & ${6.61}$ & ${6.47}$ & ${10.69}$ & ${5.98}$ \\ 
% & Omniquant~\cite{shao2024omniquant} & ${15.03}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.85}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${7.21}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${7.12}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${11.29}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${6.69}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${6.56}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${10.75}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ & ${6.06}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.00\times}}$ \\ 
% & FIGNA~\cite{jang2024figna} & ${15.04}^{\textcolor{red}{-0.07\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.86}^{\textcolor{red}{-0.08\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${7.22}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${7.12}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${11.29}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${6.70}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${6.57}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${10.75}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ & ${6.06}^{\textcolor{red}{0.00\%}}_{\textcolor[HTML]{3A9262}{1.23\times}}$ \\ 
% & VSQuant~\cite{keller202395} & ${19.00}^{\textcolor{red}{-26.41\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${13.13}^{\textcolor{red}{-10.80\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.89}^{\textcolor{red}{-23.30\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${10.36}^{\textcolor{red}{-45.51\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${12.64}^{\textcolor{red}{-11.96\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${7.85}^{\textcolor{red}{-17.34\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${8.35}^{\textcolor{red}{-27.29\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${11.91}^{\textcolor{red}{-10.79\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ & ${6.85}^{\textcolor{red}{-13.04\%}}_{\textcolor[HTML]{3A9262}{4.00\times}}$ \\ 
% & Ours (0.1\%) & \cellcolor{yellow!30}${15.05}^{\textcolor{red}{-0.13\%}}_{\textcolor[HTML]{3A9262}{1.86\times}}$ & \cellcolor{yellow!30}${11.87}^{\textcolor{red}{-0.17\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${7.22}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{2.16\times}}$ & \cellcolor{yellow!30}${7.13}^{\textcolor{red}{-0.14\%}}_{\textcolor[HTML]{3A9262}{2.04\times}}$ & \cellcolor{yellow!30}${11.30}^{\textcolor{red}{-0.09\%}}_{\textcolor[HTML]{3A9262}{2.23\times}}$ & \cellcolor{yellow!30}${6.70}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{2.16\times}}$ & \cellcolor{yellow!30}${6.57}^{\textcolor{red}{-0.15\%}}_{\textcolor[HTML]{3A9262}{2.14\times}}$ & \cellcolor{yellow!30}${10.76}^{\textcolor{red}{-0.09\%}}_{\textcolor[HTML]{3A9262}{2.31\times}}$ & \cellcolor{yellow!30}${TBD}^{\textcolor{red}{\%}}_{\textcolor[HTML]{3A9262}{\times}}$ \\ 
% & Ours (1\%) & \cellcolor{yellow!90}${15.17}^{\textcolor{red}{-0.93\%}}_{\textcolor[HTML]{3A9262}{2.43\times}}$ & \cellcolor{yellow!90}${11.97}^{\textcolor{red}{-1.01\%}}_{\textcolor[HTML]{3A9262}{3.05\times}}$ & \cellcolor{yellow!90}${7.28}^{\textcolor{red}{-0.97\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${7.19}^{\textcolor{red}{-0.98\%}}_{\textcolor[HTML]{3A9262}{2.67\times}}$ & \cellcolor{yellow!90}${11.37}^{\textcolor{red}{-0.71\%}}_{\textcolor[HTML]{3A9262}{2.86\times}}$ & \cellcolor{yellow!90}${6.74}^{\textcolor{red}{-0.75\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${6.62}^{\textcolor{red}{-0.91\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ & \cellcolor{yellow!90}${10.85}^{\textcolor{red}{-0.93\%}}_{\textcolor[HTM L]{3A9262}{3.09\times}}$ & \cellcolor{yellow!90}${6.10}^{\textcolor{red}{-0.66\%}}_{\textcolor[HTML]{3A9262}{2.70\times}}$ \\ 
% \bottomrule 
% \end{tabular}%
% }
% \end{table*}

\rOneFC{\textbf{Evaluation Methodologies}:
Our comprehensive assessment encompasses both model accuracy and hardware efficiency. 
% Model performance is evaluated using three key metrics: (1) perplexity (PPL)~\cite{jelinek1977perplexity} with a sequence length of 2048, where lower values indicate higher accuracy; (2) relative accuracy loss of FIGNA, VS-Quant, and our Anda method compared to Omniquant, demonstrating the accuracy drop during BFP conversion in the deployment process; and (3) reduction in bit-level operations (BOPs), which quantifies the decrease in theoretical model computation, with one FP16-INT4 operation considered equivalent to 64 BOPs for simplicity.
For model accuracy, we employ three key metrics: (1) perplexity (PPL)~\cite{jelinek1977perplexity} using a 2048 sequence length, where lower values indicate higher model accuracy; (2) relative accuracy loss of FIGNA, VS-Quant, and our Anda method compared to Omniquant, which demonstrates the accuracy drop during BFP conversion in the deployment process; and (3) bit-level operations (BOPs)~\cite{abati2023resq} reduction, quantifying the decrease in theoretical model computation, where we consider one FP16-INT4 operation as equivalent to 64 BOPs for simplicity.
% Hardware performance validation is conducted at both the PE and system levels. PE-level analysis examines area, power, area efficiency, and energy efficiency, while system-level evaluation compares Anda with other architectures, focusing on speedup, energy efficiency, and power and area breakdown.
% \ms{Hardware performance evaluation spans two levels: at the PE level, we analyze area, power consumption, area efficiency, and energy efficiency; at the system level, we compare Anda with baseline architectures, focusing on speedup and energy efficiency. [Dont think you need to mention this, redundant.]}
Hardware performance evaluation spans two levels: at the PE level, we analyze area and power along with corresponding efficiencies; at the system level, we compare Anda with baseline architectures, focusing on speedup and energy efficiency. 
% For hardware performance evaluation, in alignment with prior studies~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}, \ms{we use LLMs using a batch size of 1 and the maximum acceptable input sequence length: 2048 for OPT and LLaMA models, and 4096 for LLaMA2 models with the WikiText2 dataset. [repeated?]}
In alignment with prior studies~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}, system-level evaluation uses LLMs with a batch size of 1 and the maximum acceptable input sequence length under the WikiText2 dataset.
% \ms{All hardware designs [ALL?even for baseline accelerators??]} 
PE-level baselines and Anda system are implemented in SystemVerilog RTL and synthesized using Cadence Genus~\cite{candence2024genus} at 16nm technology node, operating at a clock frequency of 285 MHz and 0.8 V nominal voltage. 
Power evaluation is performed using value change dump (VCD) files generated from synthesized netlist simulations and analyzed by Genus. 
A cycle-accurate simulator, rigorously verified against functional simulations, assesses the energy and performance of Anda and baseline accelerators. 
HBM2 memory is modeled with an access energy of 3.9 pJ/bit and a bandwidth of 256 GB/s~\cite{jouppi2021ten, jang2024figna}.}
% In alignment with prior studies~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}, we evaluate LLMs using a batch size of 1 and an input-to-output sequence length ratio of 2048:1.}

% \rOneFC{\textbf{Evaluation Methodologies}: We consider both model accuracy and hardware performance. For model accuracy, we measure perplexity, denoted as PPL, using a sequence length of 2048, compare the accuracy loss of FIGNA, VS-Quant, and our Anda method relative to Omniquant, and quantify the reduction in bit operations, denoted as BOPs. Hardware performance validation begins at the PE level, focusing on area, power, area efficiency, and energy efficiency. At the system level, we compare the Anda architecture with other architecture baselines, emphasizing speedup and energy efficiency, and analyze its power and area breakdown. We implement the RTL design of all relevant hardware with SystemVerilog, and synthesize them using Cadence Genus at 16nm to obtain area results. The synthesis output netlist is simulated to generate a value change dump (VCD) file, which is then analyzed by the Genus for power evaluation. A cycle-level simulator, validated against functional simulation, evaluates the energy and performance of Anda and baseline accelerators. We model HBM2 memory with an access energy of 3.9 pJ/bit and a bandwidth of 256 GB/s~\cite{jang2024figna, jouppi2021ten}. To align with previous evaluations~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}, we assess the speedup and energy efficiency of LLMs using a batch size of 1 and an input-to-output sequence length ratio of 2048:1.}

% \ms{\textbf{Simulation}}: 
% \ms{\textbf{Evaluation Methodology}}: 
% We implement Anda architecture in RTL with SystemVerilog \ms{and conduct synthesis based on}
% %and verify the functionality of each component via RTL simulation.
% %We report the area of Anda by synthesizing the components using a commercial 
% 16 nm technology node through Cadence Genus.
% \ms{The synthesis output netlist is simulated to generate a value change dump (VCD) file, which is then analyzed by the Genus for power assessment.}
% Moreover, a cycle-level simulator 
% % with Ramulator~\cite{kim2015ramulator} for DRAM timing 
% \ms{is built} to \ms{access} the \ms{energy and performance of Anda and baseline accelerators.}
% %The power \rg{consumption} of Anda is evaluated by simulating the synthesis netlist to generate a VCD file, which is then analyzed using the Design Compiler.
% %On-chip SRAMs are also synthesized from a commercial memory compiler with the same technology.
% HBM2 memory which has the access energy of 3.9 pJ/bit and a bandwidth of 256 GB/s~\cite{jang2024figna, jouppi2021ten} \ms{is used to characterize}
% off-chip memory. We evaluate the speedup and energy efficiency in LLMs with a batch size of 1, setting the input-to-output sequence length to 2048:1, in alignment with previous evaluations~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}. 
% In subsequent benchmarks, we limit the search iterations to a maximum of 32. 
% On an A100-80G GPU, 32 iterations take less than 10 minutes for OPT-1.3b and 2.5 hours for llama-30b. In comparison, PTQ algorithms like Omniquant~\cite{shao2024omniquant} require 4.5 hours to quantize llama-30b, highlighting the significant time efficiency advantage of our method.

%, we use .which will be discussed in the following subsections in detail.} 
%converts activations to BFP, but uses bit-parallel processing and reduces mantissa length, achieving more efficient FP-INT operations.
%We implement a cycle-level simulator with Ramulator~\cite{kim2015ramulator} for DRAM timing to compare the performance of Anda and baseline accelerators. The timing parameters of the simulator are set based on the RTL synthesis results.
% \textbf{Baselines.}
% The accelerators are configured with identical memory bandwidth and on-chip buffer sizes, which are sufficiently large to fully utilize the compute cores. 
%We compare Anda with four baseline hardware accelerators.
%The first two are tensor-core based: one with FP-FP units simulating existing GPU computation schemes, and another with dedicated FP-INT units modeling GPUs with specialized integrated computation units. Y. Kim's architecture~\cite{kim2023winning} converts floating-point activations to BFP by increasing mantissa length and employs bit-serial computation for fixed-point weights. Similarly, FIGNA~\cite{jang2024figna} converts activations to BFP, but uses bit-parallel processing and reduces mantissa length, achieving more efficient FP-INT operations.
% \textbf{Workloads.}
%We evaluate the speedup and energy efficiency in LLMs with a batch size of 1, setting the input-to-output sequence length to 2048:1, in alignment with previous evaluations~\cite{guo2023olive, xiao2023smoothquant, jang2024figna, kim2023winning}. During the generation phase, \rg{[What do you mean exactly?]} Anda remains effective  with substantial benefits on reduced memory and computation due to length-variable grouped activations. \rg{[Not clear what you mean with 'remain effective']} However, as highlighted in previous studies~\cite{hong2022dfx, yuan2024llm}, commercial accelerators \rg{[hardware platforms; I wouldn't call a GPU an accelerator]} such as GPUs and TPUs often face significant under-utilization issues. To address this challenge, ongoing research investigates efficient batch decoding methods~\cite{sheng2023flexgen, yu2022orca, zhong2024distserve}, with which Anda can synergistically operate to enhance performance further. \rg{[I don't see the link between batch decoding, underutilization and Anda]}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Hardware Configuration of Anda and Baseline Designs}
% \label{tab:hw_configs}
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{@{}rcccccc@{}}
% \toprule
%                              & \begin{tabular}[c]{@{}c@{}}\#PEs \\ in MXU\end{tabular} & \#BOPs/PE/Cycle        & \begin{tabular}[c]{@{}c@{}}\#Equivalent \\ FP MAC\end{tabular} & \begin{tabular}[c]{@{}c@{}}Memory\\ (MB)\end{tabular} & INT unit     & \begin{tabular}[c]{@{}c@{}}Precision\\ Scalablity\end{tabular} \\ \midrule
% FP-FP                        & 32$\times$32                                            & 1$\times$(16$\times$4) & \multirow{5}{*}{1024}                                          & \multirow{5}{*}{2.215}                                & \XSolidBrush & \XSolidBrush                                                   \\
% FP-INT                       & 32$\times$32                                            & 1$\times$(16$\times$4) &                                                                &                                                       & \XSolidBrush & \XSolidBrush                                                   \\
% Y. Kim~\cite{kim2023winning} & 32$\times$32                                            & 4$\times$(30$\times$1) &                                                                &                                                       & \Checkmark   & \XSolidBrush                                                   \\
% FIGNA~\cite{jang2024figna}   & 32$\times$32                                            & 1$\times$(14$\times$4) &                                                                &                                                       & \Checkmark   & \XSolidBrush                                                   \\
% Anda                         & 16$\times$16                                            & 64$\times$(1$\times$4) &                                                                &                                                       & \Checkmark   & \Checkmark                                                     \\ \bottomrule
% \end{tabular}%
% }
% \end{table}




\subsection{Inference Accuracy}

% \rOneFC{[Goal: Evaluate the inference accuracy of the Anda format on standard datasets and models, proving that comparable accuracy to full precision can be achieved with lower bitwidths.]}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[htbp]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better) and BOPS Reduction (\textcolor{red}{Red})}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccccccc@{}}
% \toprule
% \multicolumn{2}{c|}{}                                                           & OPT-1.3B                                     & OPT-6.7B                                     & LLaMA-7B                                    & LLaMA2-7B                                    & OPT-13B                                      & LLaMA-13B                                   & LLaMA2-13B                                   & OPT-30B                                      & LLaMA-30B                                   \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{WikiText2}} & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 14.88/\textcolor{red}{1.00$\times$}          & 10.96/\textcolor{red}{1.00$\times$}          & 5.77/\textcolor{red}{1.00$\times$}          & 5.59/\textcolor{red}{1.00$\times$}           & 10.20/\textcolor{red}{1.00$\times$}          & 5.17/\textcolor{red}{1.00$\times$}          & 4.95/\textcolor{red}{1.00$\times$}           & 9.62/\textcolor{red}{1.00$\times$}           & 4.19/\textcolor{red}{1.00$\times$}          \\
%                                            & FIGNA~\cite{jang2024figna}         & 14.90/\textcolor{red}{1.23$\times$}          & 10.96/\textcolor{red}{1.23$\times$}          & 5.78/\textcolor{red}{1.23$\times$}          & 5.60/\textcolor{red}{1.23$\times$}           & 10.22/\textcolor{red}{1.23$\times$}          & 5.18/\textcolor{red}{1.23$\times$}          & 4.96/\textcolor{red}{1.23$\times$}           & 9.61/\textcolor{red}{1.23$\times$}           & 4.20/\textcolor{red}{1.23$\times$}          \\
%                                            & VSQuant~\cite{keller202395}        & 19.04/\textcolor{red}{4.00$\times$}          & 12.24/\textcolor{red}{4.00$\times$}          & 7.45/\textcolor{red}{4.00$\times$}          & 8.26/\textcolor{red}{4.00$\times$}           & 11.63/\textcolor{red}{4.00$\times$}          & 6.36/\textcolor{red}{4.00$\times$}          & 6.43/\textcolor{red}{4.00$\times$}           & 10.67/\textcolor{red}{4.00$\times$}          & 5.10/\textcolor{red}{4.00$\times$}          \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{14.99/\textcolor{red}{2.95$\times$}} & \textbf{10.99/\textcolor{red}{3.31$\times$}} & \textbf{5.82/\textcolor{red}{2.56$\times$}} & \textbf{5.65/\textcolor{red}{2.56$\times$}}  & \textbf{10.30/\textcolor{red}{3.20$\times$}} & \textbf{5.23/\textcolor{red}{2.59$\times$}} & \textbf{5.00/\textcolor{red}{2.44$\times$}}  & \textbf{9.71/\textcolor{red}{3.31$\times$}}  & \textbf{4.23/\textcolor{red}{2.44$\times$}} \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{PTB}}       & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 17.40/\textcolor{red}{1.00$\times$}          & 13.25/\textcolor{red}{1.00$\times$}          & 8.97/\textcolor{red}{1.00$\times$}          & 21.52/\textcolor{red}{1.00$\times$}          & 12.46/\textcolor{red}{1.00$\times$}          & 8.14/\textcolor{red}{1.00$\times$}          & 30.19/\textcolor{red}{1.00$\times$}          & 11.94/\textcolor{red}{1.00$\times$}          & 7.39/\textcolor{red}{1.00$\times$}          \\
%                                            & FIGNA~\cite{jang2024figna}         & 17.41/\textcolor{red}{1.23$\times$}          & 13.26/\textcolor{red}{1.23$\times$}          & 8.98/\textcolor{red}{1.23$\times$}          & 21.52/\textcolor{red}{1.23$\times$}          & 12.47/\textcolor{red}{1.23$\times$}          & 8.15/\textcolor{red}{1.23$\times$}          & 30.19/\textcolor{red}{1.23$\times$}          & 11.95/\textcolor{red}{1.23$\times$}          & 7.40/\textcolor{red}{1.23$\times$}          \\
%                                            & VSQuant~\cite{keller202395}        & 25.64/\textcolor{red}{4.00$\times$}          & 15.50/\textcolor{red}{4.00$\times$}          & 15.78/\textcolor{red}{4.00$\times$}         & 53.46/\textcolor{red}{4.00$\times$}          & 14.47/\textcolor{red}{4.00$\times$}          & 12.54/\textcolor{red}{4.00$\times$}         & 49.91/\textcolor{red}{4.00$\times$}          & 13.47/\textcolor{red}{4.00$\times$}          & 9.92/\textcolor{red}{4.00$\times$}          \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{17.57/\textcolor{red}{2.31$\times$}} & \textbf{13.35/\textcolor{red}{2.86$\times$}} & \textbf{9.05/\textcolor{red}{2.54$\times$}} & \textbf{21.61/\textcolor{red}{2.39$\times$}} & \textbf{12.58/\textcolor{red}{2.67$\times$}} & \textbf{8.22/\textcolor{red}{2.67$\times$}} & \textbf{30.41/\textcolor{red}{2.92$\times$}} & \textbf{12.03/\textcolor{red}{2.86$\times$}} & \textbf{7.45/\textcolor{red}{2.92$\times$}} \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{C4}}        & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 15.03/\textcolor{red}{1.00$\times$}          & 11.85/\textcolor{red}{1.00$\times$}          & 7.21/\textcolor{red}{1.00$\times$}          & 7.12/\textcolor{red}{1.00$\times$}           & 11.29/\textcolor{red}{1.00$\times$}          & 6.69/\textcolor{red}{1.00$\times$}          & 6.56/\textcolor{red}{1.00$\times$}           & 10.75/\textcolor{red}{1.00$\times$}          & 6.06/\textcolor{red}{1.00$\times$}          \\
%                                            & FIGNA~\cite{jang2024figna}         & 15.04/\textcolor{red}{1.23$\times$}          & 11.86/\textcolor{red}{1.23$\times$}          & 7.22/\textcolor{red}{1.23$\times$}          & 7.12/\textcolor{red}{1.23$\times$}           & 11.29/\textcolor{red}{1.23$\times$}          & 6.70/\textcolor{red}{1.23$\times$}          & 6.57/\textcolor{red}{1.23$\times$}           & 10.75/\textcolor{red}{1.23$\times$}          & 6.06/\textcolor{red}{1.23$\times$}          \\
%                                            & VSQuant~\cite{keller202395}        & 19.00/\textcolor{red}{4.00$\times$}          & 13.13/\textcolor{red}{4.00$\times$}          & 8.89/\textcolor{red}{4.00$\times$}          & 10.36/\textcolor{red}{4.00$\times$}          & 12.64/\textcolor{red}{4.00$\times$}          & 7.85/\textcolor{red}{4.00$\times$}          & 8.35/\textcolor{red}{4.00$\times$}           & 11.91/\textcolor{red}{4.00$\times$}          & 6.85/\textcolor{red}{4.00$\times$}          \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{15.17/\textcolor{red}{2.43$\times$}} & \textbf{11.97/\textcolor{red}{3.05$\times$}} & \textbf{7.28/\textcolor{red}{2.70$\times$}} & \textbf{7.19/\textcolor{red}{2.67$\times$}}  & \textbf{11.37/\textcolor{red}{2.86$\times$}} & \textbf{6.74/\textcolor{red}{2.70$\times$}} & \textbf{6.62/\textcolor{red}{2.70$\times$}}  & \textbf{10.85/\textcolor{red}{3.09$\times$}} & \textbf{6.10/\textcolor{red}{2.70$\times$}} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[htbp]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better) and BOPS Reduction (\textcolor{red}{Red})}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccccccc@{}}
% \toprule
% \multicolumn{2}{c|}{}                                                           & OPT-1.3B                                     & OPT-6.7B                                     & LLaMA-7B                                    & LLaMA2-7B                                    & OPT-13B                                      & LLaMA-13B                                   & LLaMA2-13B                                   & OPT-30B                                      & LLaMA-30B                                   \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{WikiText2}} & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 14.88 (0.00\%, \textcolor{red}{1.00x})       & 10.96 (0.00\%, \textcolor{red}{1.00x})       & 5.77 (0.00\%, \textcolor{red}{1.00x})       & 5.59 (0.00\%, \textcolor{red}{1.00x})        & 10.20 (0.00\%, \textcolor{red}{1.00x})       & 5.17 (0.00\%, \textcolor{red}{1.00x})       & 4.95 (0.00\%, \textcolor{red}{1.00x})        & 9.62 (0.00\%, \textcolor{red}{1.00x})        & 4.19 (0.00\%, \textcolor{red}{1.00x})       \\
%                                            & FIGNA~\cite{jang2024figna}         & 14.90 (-0.13\%, \textcolor{red}{1.23x})      & 10.96 (0.00\%, \textcolor{red}{1.23x})       & 5.78 (-0.17\%, \textcolor{red}{1.23x})      & 5.60 (-0.18\%, \textcolor{red}{1.23x})       & 10.22 (-0.20\%, \textcolor{red}{1.23x})      & 5.18 (-0.19\%, \textcolor{red}{1.23x})      & 4.96 (-0.20\%, \textcolor{red}{1.23x})       & 9.61 (0.10\%, \textcolor{red}{1.23x})        & 4.20 (-0.24\%, \textcolor{red}{1.23x})      \\
%                                            & VSQuant~\cite{keller202395}        & 19.04 (-27.96\%, \textcolor{red}{4.00x})     & 12.24 (-11.68\%, \textcolor{red}{4.00x})     & 7.45 (-29.12\%, \textcolor{red}{4.00x})     & 8.26 (-47.76\%, \textcolor{red}{4.00x})      & 11.63 (-13.98\%, \textcolor{red}{4.00x})     & 6.36 (-23.02\%, \textcolor{red}{4.00x})     & 6.43 (-29.90\%, \textcolor{red}{4.00x})      & 10.67 (-10.91\%, \textcolor{red}{4.00x})     & 5.10 (-21.72\%, \textcolor{red}{4.00x})     \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{14.99 (-0.74\%, \textcolor{red}{2.95x})} & \textbf{10.99 (-0.27\%, \textcolor{red}{3.31x})} & \textbf{5.82 (-0.87\%, \textcolor{red}{2.56x})} & \textbf{5.65 (-1.07\%, \textcolor{red}{2.56x})}  & \textbf{10.30 (-0.98\%, \textcolor{red}{3.20x})} & \textbf{5.23 (-1.16\%, \textcolor{red}{2.59x})} & \textbf{5.00 (-1.01\%, \textcolor{red}{2.44x})}  & \textbf{9.71 (-0.94\%, \textcolor{red}{3.31x})}  & \textbf{4.23 (-0.95\%, \textcolor{red}{2.44x})} \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{PTB}}       & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 17.40 (0.00\%, \textcolor{red}{1.00x})       & 13.25 (0.00\%, \textcolor{red}{1.00x})       & 8.97 (0.00\%, \textcolor{red}{1.00x})       & 21.52 (0.00\%, \textcolor{red}{1.00x})       & 12.46 (0.00\%, \textcolor{red}{1.00x})       & 8.14 (0.00\%, \textcolor{red}{1.00x})       & 30.19 (0.00\%, \textcolor{red}{1.00x})       & 11.94 (0.00\%, \textcolor{red}{1.00x})       & 7.39 (0.00\%, \textcolor{red}{1.00x})       \\
%                                            & FIGNA~\cite{jang2024figna}         & 17.41 (-0.06\%, \textcolor{red}{1.23x})      & 13.26 (-0.08\%, \textcolor{red}{1.23x})      & 8.98 (-0.11\%, \textcolor{red}{1.23x})      & 21.52 (0.00\%, \textcolor{red}{1.23x})       & 12.47 (-0.08\%, \textcolor{red}{1.23x})      & 8.15 (-0.12\%, \textcolor{red}{1.23x})      & 30.19 (0.00\%, \textcolor{red}{1.23x})       & 11.95 (-0.08\%, \textcolor{red}{1.23x})      & 7.40 (-0.14\%, \textcolor{red}{1.23x})      \\
%                                            & VSQuant~\cite{keller202395}        & 25.64 (-47.36\%, \textcolor{red}{4.00x})     & 15.50 (-16.98\%, \textcolor{red}{4.00x})     & 15.78 (-75.92\%, \textcolor{red}{4.00x})    & 53.46 (-148.42\%, \textcolor{red}{4.00x})    & 14.47 (-16.13\%, \textcolor{red}{4.00x})     & 12.54 (-54.05\%, \textcolor{red}{4.00x})    & 49.91 (-65.32\%, \textcolor{red}{4.00x})     & 13.47 (-12.81\%, \textcolor{red}{4.00x})     & 9.92 (-34.24\%, \textcolor{red}{4.00x})     \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{17.57 (-0.98\%, \textcolor{red}{2.31x})} & \textbf{13.35 (-0.75\%, \textcolor{red}{2.86x})} & \textbf{9.05 (-0.89\%, \textcolor{red}{2.54x})} & \textbf{21.61 (-0.42\%, \textcolor{red}{2.39x})} & \textbf{12.58 (-0.96\%, \textcolor{red}{2.67x})} & \textbf{8.22 (-0.98\%, \textcolor{red}{2.67x})} & \textbf{30.41 (-0.73\%, \textcolor{red}{2.92x})} & \textbf{12.03 (-0.75\%, \textcolor{red}{2.86x})} & \textbf{7.45 (-0.81\%, \textcolor{red}{2.92x})} \\ \midrule
% \multirow{6}{*}{\rotatebox{90}{C4}}        & FP16                               &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & Omniquant~\cite{shao2024omniquant} & 15.03 (0.00\%, \textcolor{red}{1.00x})       & 11.85 (0.00\%, \textcolor{red}{1.00x})       & 7.21 (0.00\%, \textcolor{red}{1.00x})       & 7.12 (0.00\%, \textcolor{red}{1.00x})        & 11.29 (0.00\%, \textcolor{red}{1.00x})       & 6.69 (0.00\%, \textcolor{red}{1.00x})       & 6.56 (0.00\%, \textcolor{red}{1.00x})        & 10.75 (0.00\%, \textcolor{red}{1.00x})       & 6.06 (0.00\%, \textcolor{red}{1.00x})       \\
%                                            & FIGNA~\cite{jang2024figna}         & 15.04 (-0.07\%, \textcolor{red}{1.23x})      & 11.86 (-0.08\%, \textcolor{red}{1.23x})      & 7.22 (-0.14\%, \textcolor{red}{1.23x})      & 7.12 (0.00\%, \textcolor{red}{1.23x})        & 11.29 (0.00\%, \textcolor{red}{1.23x})       & 6.70 (-0.15\%, \textcolor{red}{1.23x})      & 6.57 (-0.15\%, \textcolor{red}{1.23x})       & 10.75 (0.00\%, \textcolor{red}{1.23x})       & 6.06 (0.00\%, \textcolor{red}{1.23x})       \\
%                                            & VSQuant~\cite{keller202395}        & 19.00 (-26.41\%, \textcolor{red}{4.00x})     & 13.13 (-10.80\%, \textcolor{red}{4.00x})     & 8.89 (-23.30\%, \textcolor{red}{4.00x})     & 10.36 (-45.51\%, \textcolor{red}{4.00x})     & 12.64 (-11.96\%, \textcolor{red}{4.00x})     & 7.85 (-17.34\%, \textcolor{red}{4.00x})     & 8.35 (-27.29\%, \textcolor{red}{4.00x})      & 11.91 (-10.79\%, \textcolor{red}{4.00x})     & 6.85 (-13.04\%, \textcolor{red}{4.00x})     \\
%                                            & \textbf{Ours (0.1\%)}              &                                              &                                              &                                             &                                              &                                              &                                             &                                              &                                              &                                             \\
%                                            & \textbf{Ours (1\%)}                & \textbf{15.17 (-0.93\%, \textcolor{red}{2.43x})} & \textbf{11.97 (-1.01\%, \textcolor{red}{3.05x})} & \textbf{7.28 (-0.97\%, \textcolor{red}{2.70x})} & \textbf{7.19 (-0.98\%, \textcolor{red}{2.67x})}  & \textbf{11.37 (-0.71\%, \textcolor{red}{2.86x})} & \textbf{6.74 (-0.75\%, \textcolor{red}{2.70x})} & \textbf{6.62 (-0.91\%, \textcolor{red}{2.70x})}  & \textbf{10.85 (-0.93\%, \textcolor{red}{3.09x})} & \textbf{6.10 (-0.66\%, \textcolor{red}{2.70x})} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[htbp]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better) and BOPS Reduction (Black)}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}c@{}c|*{9}{c@{\hspace{-0.3em}}c@{\hspace{0.7em}}}@{}}
% \toprule
% \multicolumn{2}{c|}{}                                                           & \multicolumn{2}{c}{OPT-1.3B} & \multicolumn{2}{c}{OPT-6.7B} & \multicolumn{2}{c}{LLaMA-7B} & \multicolumn{2}{c}{LLaMA2-7B} & \multicolumn{2}{c}{OPT-13B} & \multicolumn{2}{c}{LLaMA-13B} & \multicolumn{2}{c}{LLaMA2-13B} & \multicolumn{2}{c}{OPT-30B} & \multicolumn{2}{c}{LLaMA-30B} \\ \midrule
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox{3cm}{\centering WikiText2}}} & FP16 & \multicolumn{18}{c}{} \\ 
% & Omniquant~\cite{shao2024omniquant} & 14.88 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 10.96 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 5.77 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 5.59 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 10.20 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 5.17 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 4.95 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 9.62 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 4.19 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} \\ 
% & FIGNA~\cite{jang2024figna} & 14.90 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.13\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 10.96 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 5.78 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.17\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 5.60 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.18\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 10.22 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.20\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 5.18 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.19\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 4.96 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.20\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 9.61 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.10\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 4.20 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.24\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} \\ 
% & VSQuant~\cite{keller202395} & 19.04 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-27.96\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 12.24 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-11.68\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 7.45 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-29.12\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 8.26 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-47.76\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 11.63 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-13.98\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 6.36 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-23.02\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 6.43 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-29.90\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 10.67 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-10.91\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 5.10 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-21.72\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} \\ 
% & \textbf{Ours (0.1\%)} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\ 
% & \textbf{Ours (1\%)} & \textbf{14.99} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.74\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.95}}$\times$ \end{tabular}} & \textbf{10.99} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.27\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{3.31}}$\times$ \end{tabular}} & \textbf{5.82} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.87\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.56}}$\times$ \end{tabular}} & \textbf{5.65} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-1.07\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.56}}$\times$ \end{tabular}} & \textbf{10.30} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.98\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{3.20}}$\times$ \end{tabular}} & \textbf{5.23} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-1.16\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.59}}$\times$ \end{tabular}} & \textbf{5.00} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-1.01\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.44}}$\times$ \end{tabular}} & \textbf{9.71} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.94\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{3.31}}$\times$ \end{tabular}} & \textbf{4.23} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.95\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.44}}$\times$ \end{tabular}} \\ 
% \midrule 
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox{3cm}{\centering PTB}}} & FP16 & \multicolumn{18}{c}{} \\ 
% & Omniquant~\cite{shao2024omniquant} & 17.40 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 13.25 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 8.97 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 21.52 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 12.46 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 8.14 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 30.19 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 11.94 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 7.39 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} \\ 
% & FIGNA~\cite{jang2024figna} & 17.41 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.06\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 13.26 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.08\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 8.98 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.11\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 21.52 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 12.47 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.08\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 8.15 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.12\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 30.19 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 11.95 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.08\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 7.40 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.14\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} \\ 
% & VSQuant~\cite{keller202395} & 25.64 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-47.36\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 15.50 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-16.98\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 15.78 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-75.92\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 53.46 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-148.42\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 14.47 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-16.13\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 12.54 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-54.05\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 49.91 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-65.32\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 13.47 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-12.81\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 9.92 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-34.24\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} \\ 
% & \textbf{Ours (0.1\%)} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\ 
% & \textbf{Ours (1\%)} & \textbf{17.57} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.98\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.31}}$\times$ \end{tabular}} & \textbf{13.35} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.75\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.86}}$\times$ \end{tabular}} & \textbf{9.05} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.89\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.54}}$\times$ \end{tabular}} & \textbf{21.61} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.42\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.39}}$\times$ \end{tabular}} & \textbf{12.58} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.96\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.67}}$\times$ \end{tabular}} & \textbf{8.22} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.98\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.67}}$\times$ \end{tabular}} & \textbf{30.41} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.73\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.92}}$\times$ \end{tabular}} & \textbf{12.03} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.75\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.86}}$\times$ \end{tabular}} & \textbf{7.45} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.81\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.92}}$\times$ \end{tabular}} \\ 
% \midrule 
% \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox{3cm}{\centering C4}}} & FP16 & \multicolumn{18}{c}{} \\ 
% & Omniquant~\cite{shao2024omniquant} & 15.03 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 11.85 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 7.21 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 7.12 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 11.29 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 6.69 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 6.56 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 10.75 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} & 6.06 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.00}$\times$ \end{tabular}} \\ 
% & FIGNA~\cite{jang2024figna} & 15.04 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.07\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 11.86 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.08\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 7.22 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.14\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 7.12 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 11.29 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 6.70 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.15\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 6.57 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-0.15\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 10.75 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} & 6.06 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{0.00\%} \\ \textcolor[RGB]{0,100,0}{1.23}$\times$ \end{tabular}} \\ 
% & VSQuant~\cite{keller202395} & 19.00 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-26.41\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 13.13 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-10.80\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 8.89 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-23.30\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 10.36 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-45.51\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 12.64 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-11.96\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 7.85 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-17.34\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 8.35 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-27.29\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 11.91 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-10.79\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} & 6.85 & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{-13.04\%} \\ \textcolor[RGB]{0,100,0}{4.00}$\times$ \end{tabular}} \\ 
% & \textbf{Ours (0.1\%)} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{} \\ 
% & \textbf{Ours (1\%)} & \textbf{15.17} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.93\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.43}}$\times$ \end{tabular}} & \textbf{11.97} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-1.01\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{3.05}}$\times$ \end{tabular}} & \textbf{7.28} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.97\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.70}}$\times$ \end{tabular}} & \textbf{7.19} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.98\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.67}}$\times$ \end{tabular}} & \textbf{11.37} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.71\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.86}}$\times$ \end{tabular}} & \textbf{6.74} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.75\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.70}}$\times$ \end{tabular}} & \textbf{6.62} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.91\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.70}}$\times$ \end{tabular}} & \textbf{10.85} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.93\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{3.09}}$\times$ \end{tabular}} & \textbf{6.10} & {\scriptsize\begin{tabular}[c]{r@{}l}\textcolor{red}{\textbf{-0.66\%}} \\ \textcolor[RGB]{0,100,0}{\textbf{2.70}}$\times$ \end{tabular}} \\ 
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[htbp]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better), BOPS Reduction (\textcolor{red}{Red}), and Activation Tensor Compression Ratio (\textcolor{blue}{Blue})}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}ccccccccccc@{}}
% \toprule
% \multicolumn{2}{c}{}                                                                                 & OPT-1.3B                                                                    & OPT-6.7B                                                                    & LLaMA-7B                                                                   & LLaMA2-7B                                                                   & OPT-13B                                                                     & LLaMA-13B                                                                  & LLaMA2-13B                                                                  & OPT-30B                                                                     & LLaMA-30B                                                                  \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{WikiText2}} & \multicolumn{1}{c|}{Omniquant~\cite{shao2024omniquant}} & 14.88/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 10.96/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.77/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.59/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 4.95/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 9.62/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 4.19/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{AWQ~\cite{lin2024awq}}              & 14.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 10.93/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.81/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.62/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 4.97/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 9.59/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 4.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{GPTQ~\cite{frantar2023optq}}        & 14.89/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 10.93/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.85/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.61/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 4.98/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 9.58/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 4.23/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{RTN~\cite{dettmers2022gpt3}}        & 15.29/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 11.15/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.96/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.72/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.30/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 5.25/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 4.98/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 9.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 4.23/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{FIGNA~\cite{jang2024figna}}         & 14.90/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 10.96/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 5.78/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 5.60/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}           & 10.22/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 5.18/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 4.96/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}           & 9.61/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}           & 4.20/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{VSQuant~\cite{keller202395}}        & 19.04/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 12.24/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 7.45/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 8.26/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}           & 11.63/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 6.36/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 6.43/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}           & 10.67/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 5.10/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          \\
%                                            & \multicolumn{1}{c|}{\textbf{Ours}}                      & \textbf{14.99/\textcolor{red}{2.95$\times$}/\textcolor{blue}{2.72$\times$}} & \textbf{10.99/\textcolor{red}{3.31$\times$}/\textcolor{blue}{2.94$\times$}} & \textbf{5.82/\textcolor{red}{2.56$\times$}/\textcolor{blue}{2.22$\times$}} & \textbf{5.65/\textcolor{red}{2.56$\times$}/\textcolor{blue}{2.22$\times$}}  & \textbf{10.30/\textcolor{red}{3.20$\times$}/\textcolor{blue}{2.79$\times$}} & \textbf{5.23/\textcolor{red}{2.59$\times$}/\textcolor{blue}{2.28$\times$}} & \textbf{5.00/\textcolor{red}{2.44$\times$}/\textcolor{blue}{2.04$\times$}}  & \textbf{9.71/\textcolor{red}{3.31$\times$}/\textcolor{blue}{2.94$\times$}}  & \textbf{4.23/\textcolor{red}{2.44$\times$}/\textcolor{blue}{2.04$\times$}} \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{PTB}}       & \multicolumn{1}{c|}{Omniquant~\cite{shao2024omniquant}} & 17.40/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 13.25/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 8.97/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 21.52/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 12.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 8.14/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 30.19/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 11.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.39/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{AWQ~\cite{lin2024awq}}              & 17.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 13.28/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 12.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 11.90/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             \\
%                                            & \multicolumn{1}{c|}{GPTQ~\cite{frantar2023optq}}        & 17.41/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 13.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 12.42/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 11.89/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             \\
%                                            & \multicolumn{1}{c|}{RTN~\cite{dettmers2022gpt3}}        & 33.63/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 16.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 15.40/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}              & 14.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}             \\
%                                            & \multicolumn{1}{c|}{FIGNA~\cite{jang2024figna}}         & 17.41/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 13.26/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 8.98/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 21.52/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 12.47/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 8.15/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 30.19/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 11.95/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 7.40/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{VSQuant~\cite{keller202395}}        & 25.64/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 15.50/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 15.78/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}         & 53.46/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 14.47/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 12.54/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}         & 49.91/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 13.47/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 9.92/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          \\
%                                            & \multicolumn{1}{c|}{\textbf{Ours}}                      & \textbf{17.57/\textcolor{red}{2.31$\times$}/\textcolor{blue}{2.11$\times$}} & \textbf{13.35/\textcolor{red}{2.86$\times$}/\textcolor{blue}{2.54$\times$}} & \textbf{9.05/\textcolor{red}{2.54$\times$}/\textcolor{blue}{2.09$\times$}} & \textbf{21.61/\textcolor{red}{2.39$\times$}/\textcolor{blue}{2.17$\times$}} & \textbf{12.58/\textcolor{red}{2.67$\times$}/\textcolor{blue}{2.28$\times$}} & \textbf{8.22/\textcolor{red}{2.67$\times$}/\textcolor{blue}{2.28$\times$}} & \textbf{30.41/\textcolor{red}{2.92$\times$}/\textcolor{blue}{2.40$\times$}} & \textbf{12.03/\textcolor{red}{2.86$\times$}/\textcolor{blue}{2.54$\times$}} & \textbf{7.45/\textcolor{red}{2.92$\times$}/\textcolor{blue}{2.40$\times$}} \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{C4}}        & \multicolumn{1}{c|}{Omniquant~\cite{shao2024omniquant}} & 15.03/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 11.85/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.12/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 11.29/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.75/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{AWQ~\cite{lin2024awq}}              & 15.04/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 11.87/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.13/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 11.28/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.70/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.75/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{GPTQ~\cite{frantar2023optq}}        & 15.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 11.87/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.12/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 11.26/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.74/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{RTN~\cite{dettmers2022gpt3}}        & 15.71/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 12.31/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.37/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 7.24/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 11.51/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.58/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}           & 10.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{FIGNA~\cite{jang2024figna}}         & 15.04/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 11.86/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 7.22/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 7.12/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}           & 11.29/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 6.70/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 6.57/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}           & 10.75/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          & 6.06/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}          \\
%                                            & \multicolumn{1}{c|}{VSQuant~\cite{keller202395}}        & 19.00/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 13.13/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 8.89/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 10.36/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 12.64/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 7.85/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 8.35/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}           & 11.91/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          & 6.85/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}          \\
%                                            & \multicolumn{1}{c|}{\textbf{Ours}}                      & \textbf{15.17/\textcolor{red}{2.43$\times$}/\textcolor{blue}{2.19$\times$}} & \textbf{11.97/\textcolor{red}{3.05$\times$}/\textcolor{blue}{2.79$\times$}} & \textbf{7.28/\textcolor{red}{2.70$\times$}/\textcolor{blue}{2.34$\times$}} & \textbf{7.19/\textcolor{red}{2.67$\times$}/\textcolor{blue}{2.28$\times$}}  & \textbf{11.37/\textcolor{red}{2.86$\times$}/\textcolor{blue}{2.54$\times$}} & \textbf{6.74/\textcolor{red}{2.70$\times$}/\textcolor{blue}{2.34$\times$}} & \textbf{6.62/\textcolor{red}{2.70$\times$}/\textcolor{blue}{2.34$\times$}}  & \textbf{10.85/\textcolor{red}{3.09$\times$}/\textcolor{blue}{2.86$\times$}} & \textbf{6.10/\textcolor{red}{2.70$\times$}/\textcolor{blue}{2.34$\times$}} \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \caption{Weight-only quantization Results of Popular LLMs \\ Key Metrics: Perplexity (Black, lower is better), \textcolor{red}{OPS Reduction (Red)}, and \textcolor{blue}{Activation Tensor Compression Ratio (Blue)}}
% \label{tab:algo_res}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cc|ccccccccc@{}}
% \toprule
% \multicolumn{2}{c|}{}                                                          & OPT-1.3B                                                           & OPT-6.7B                                                           & LLaMA-7B                                                           & LLaMA2-7B                                                          & OPT-13B                                                            & LLaMA-13B                                                          & LLaMA2-13B                                                         & OPT-30B                                                            & LLaMA-30B                                                         \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{WikiText2}} & Omniquant\cite{shao2024omniquant} & 14.88/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 10.96/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.77/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 5.59/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.95/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 9.62/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.19/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & AWQ\cite{lin2024awq}              & 14.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 10.93/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.81/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 5.62/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.97/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 9.59/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & GPTQ\cite{frantar2023optq}        & 14.89/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 10.93/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.85/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 5.61/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.20/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.98/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 9.58/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.23/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & RTN\cite{nagel2021white}        & 15.29/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 11.15/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.96/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 5.72/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.30/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 5.25/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.98/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 9.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 4.23/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & FIGNA\cite{jang2024figna}         & 14.90/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 10.96/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 5.78/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 5.60/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 10.22/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 5.18/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 4.96/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 9.61/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 4.20/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & VSQuant\cite{keller202395}        & 19.04/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 12.24/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 7.45/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 8.26/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 11.63/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 6.36/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 6.43/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 10.67/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 5.10/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} \\
%                                            & Ours                              & 14.99/\textcolor{red}{2.95$\times$}/\textcolor{blue}{2.72$\times$} & 10.99/\textcolor{red}{3.31$\times$}/\textcolor{blue}{2.94$\times$} & 5.82/\textcolor{red}{2.56$\times$}/\textcolor{blue}{2.22$\times$}  & 5.65/\textcolor{red}{2.56$\times$}/\textcolor{blue}{2.22$\times$}  & 10.30/\textcolor{red}{3.20$\times$}/\textcolor{blue}{2.79$\times$} & 5.23/\textcolor{red}{2.59$\times$}/\textcolor{blue}{2.28$\times$}  & 5.00/\textcolor{red}{2.44$\times$}/\textcolor{blue}{2.04$\times$}  & 9.71/\textcolor{red}{3.31$\times$}/\textcolor{blue}{2.94$\times$}  & 4.23/\textcolor{red}{2.44$\times$}/\textcolor{blue}{2.04$\times$} \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{PTB}}       & Omniquant\cite{shao2024omniquant} & 17.40/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 13.25/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 8.97/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 21.52/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 12.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 8.14/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 30.19/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 11.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 7.39/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & AWQ\cite{lin2024awq}              & 17.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 13.28/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 12.46/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 11.90/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}    \\
%                                            & GPTQ\cite{frantar2023optq}        & 17.41/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 13.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 12.42/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 11.89/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}    \\
%                                            & RTN\cite{nagel2021white}        & 33.63/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 16.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 15.40/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}     & 14.17/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & -/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}    \\
%                                            & FIGNA\cite{jang2024figna}         & 17.41/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 13.26/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 8.98/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 21.52/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 12.47/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 8.15/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 30.19/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 11.95/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 7.40/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & VSQuant\cite{keller202395}        & 25.64/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 15.50/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 15.78/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 53.46/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 14.47/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 12.54/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 49.91/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 13.47/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 9.92/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} \\
%                                            & Ours                              & 18.15                                                              &                                                                    & 9.02                                                               & 22.12                                                              &                                                                    &                                                                    & 30.21                                                              &                                                                    &                                                                   \\ \midrule
% \multirow{7}{*}{\rotatebox{90}{C4}}        & Omniquant\cite{shao2024omniquant} & 15.03/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 11.85/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 7.12/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 11.29/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.75/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & AWQ\cite{lin2024awq}              & 15.04/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 11.87/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 7.13/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 11.28/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.70/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.75/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & GPTQ\cite{frantar2023optq}        & 15.05/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 11.87/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 7.21/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 7.12/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 11.26/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 6.56/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.74/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & RTN\cite{nagel2021white}        & 15.71/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 12.31/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 7.37/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 7.24/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 11.51/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.69/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 6.58/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$}  & 10.94/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} & 6.06/\textcolor{red}{1.00$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & FIGNA\cite{jang2024figna}         & 15.04/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 11.86/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 7.22/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 7.12/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 11.29/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 6.70/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 6.57/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$}  & 10.75/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} & 6.06/\textcolor{red}{1.23$\times$}/\textcolor{blue}{1.00$\times$} \\
%                                            & VSQuant\cite{keller202395}        & 19.00/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 13.13/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 8.89/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 10.36/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 12.64/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 7.85/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 8.35/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$}  & 11.91/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} & 6.85/\textcolor{red}{4.00$\times$}/\textcolor{blue}{3.88$\times$} \\
%                                            & Ours                              & 15.44                                                              &                                                                    & 7.25                                                               & 7.17                                                               &                                                                    &                                                                    & 6.59                                                               &                                                                    &                                                                   \\ \bottomrule
% \end{tabular}%
% }
% \end{table*} 

% \rOneFC{We evaluate inference accuracy using the Anda format to present the effectiveness of our adaptive precision search algorithm across various LLM models and datasets. For each dataset, we sample 128 sequences of length 2048 from the training set for calibration. We limit the adaptive precision search algorithm to 32 iterations.}

\rOneFC{We evaluate inference accuracy using the \ms{optimal} Anda format \ms{explored by} adaptive precision search algorithm across \ms{all benchmarks.} %various LLM models and datasets. 
For each dataset, 128 random sequences of length 2048 \ms{are sampled} for calibration~\cite{shao2024omniquant}, limiting the adaptive precision search algorithm to 32 iterations.}
\rOneFC{Note that Anda is capable of adapting mantissa bits according to the user-defined accuracy tolerance. Therefore, we report results for two accuracy constraints: 0.1\% representing minimal loss and 1\% representing acceptable loss for most scenarios.}
% Moreover, Anda's consistent performance improvements across various models and datasets showcase its effectiveness and robust generalization.}

% \ms{In this section, we compare our approach against sota LLM quantization strategies, focusing on} model accuracy and overall computational cost reduction. 
% % PPL \rg{[write in full?]} \ms{is served as} the metric for model inference accuracy (lower is better), while BOPs \ms{What is the op standing for? FP16xINT4?} \rg{[Billion ops? or ops per second? -> write in full]} \ms{quantify} the reduction in overall computational cost. \ms{We use FP16 models as the baseline and compare them to LLMs} \ms{quantized based on} Omniquant, FIGNA and VS-Quant methods, \ms{respectively}. 
% % \ms{Apart from other Sota that exploits fixed or even extended mantissa bits, 
% \ms{Anda is capable of adapting mantissa bits according to the different user-defined accuracy tolerance. Therefore, the performance of the Anda scheme derived by the optimal mantissa bit combination candidate} under 0.1\% \ms{accuracy degradation} (representing nearly no loss) and 1\% \ms{accuracy drop} (indicating acceptable loss for most scenarios) \ms{are presented}. 
%we evaluate the performance of our Anda quantization strategy, obtained through adaptive precision combination search, in terms of model accuracy and overall computational cost reduction. PPL \rg{[write in full?]} serves as the metric for model inference accuracy, while BOPs \rg{[Billion ops? or ops per second? -> write in full]} measures the reduction in overall computational cost. 
%To validate the effectiveness of our method, we set two relative accuracy loss thresholds: 0.1\%, representing nearly no accuracy loss, and 1\%, indicating acceptable accuracy loss for most scenarios.
%LLMs provided by Omniquant \ms{is adopted} as baseline models and apply FIGNA \cite{jang2024figna} and VS-Quant \cite{keller202395} methods on these models for comparison.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figs/best_combination_heatmap.pdf}
    \caption{Identified best precision combinations of various LLMs on different datasets given different accuracy tolerances.}
    \label{fig:combination_heatmap}
\end{figure}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figs/pe_level_eval.pdf}
    % \caption{Area and power breakdown of Anda.}
    \caption{PE-level comparison for FP-INT GEMM operations in terms of area, area efficiency, power, and energy efficiency. All data are normalized to FP-FP for simplicity.}
    \label{fig:pe_level}
\end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/perf_benchmark_v4.pdf}
    \caption{Speedup and energy efficiency comparison across the accelerators. All data are normalized to FP-FP for simplicity. Higher is better.}
    \label{fig:benchmark}
\end{figure*}
\rOneFC{Table~\ref{tab:algo_res} compares Anda's performance against baseline quantization methods, where PPL values are shown in black, the relative accuracy drop is displayed in red, and the BOPs reduction is presented in green.
\rTwoFC{Note that the occasional slight exceedance of the validation accuracy loss over the constraint is normal for Anda due to differences between the calibration and validation datasets.}
The results demonstrate that Anda achieves significant BOPs reductions while maintaining accuracy close to the target constraints. For instance, on the WikiText2 dataset, Anda achieves 1.80$\sim$3.10$\times$ and 2.44$\sim$3.31$\times$ BOPs reduction under 0.1\% and 1\% accuracy loss, respectively, flexibly meeting varying accuracy-efficiency requirements.}
%\rOneFC{Anda's consistent performance improvements across various models and datasets showcase the effectiveness and robust generalization of our proposed adaptive precision search algorithm.}
\rOneFC{Compared to FIGNA, which yields a 1.23$\times$ BOPs reduction with shorter bit-width multiplication, Anda further achieves 1.46$\sim$2.69$\times$ BOPs reductions at similar accuracy loss levels by leveraging different mantissa lengths for activation tensors} %based on their quantization sensitivity.} 
\rOneFC{In contrast to VS-Quant, a BFP method requiring retraining, directly deploying it leads to severe accuracy degradation despite achieving 4$\times$ BOPs reduction. For example, VS-Quant suffers a 27.96\% accuracy loss on OPT-1.3B with WikiText2. Anda, however, achieves a much better accuracy-efficiency balance, obtaining nearly 3$\times$ BOPs reduction with only a 0.74\% accuracy loss in the same scenario.}
%\ms{move the following sentence to here to better connect with next para}
\rOneFC{Anda's consistent performance improvements across various models and datasets showcase the effectiveness and robust generalization of our adaptive precision search algorithm.}
% Table~\ref{tab:algo_res} %demonstrates that our quantization strategy consistently achieves significant BOPS reduction while maintaining high inference accuracy 
% \ms{demonstrates the effectiveness of our quantization strategy in significantly reducing BOPs}
% across various models and datasets, \ms{coming from the flexible mantissa bits of the Anda representation with minimal accuracy drop.} \ms{Specifically,} %For instance, 
% on the OPT-30B model with the WikiText2 dataset, our method achieves a 3.31$\times$ BOPs reduction at a 1\% relative accuracy loss compared to Omniquant. \ms{Although FIGNA alleviates the computation cost with shorter bit-width multiplication, yielding a 1.23$\times$ BOPs reduction} for the OPT-1.3B model on the WikiText2 dataset,
% %Compared to FIGNA, 
% our method achieves 2.95$\times$ BOPs reduction at similar accuracy loss levels. 
% %Taking  as an example, our method achieves a 2.95$\times$ BOPS reduction at a 1\% relative accuracy loss, while FIGNA only achieves 1.23$\times$.
% \ms{In contrast to VS-Quant, which forces FP16 activations to lower precision for competitive performance but suffers server accuracy degradation, our method succeeds in a good balance between computational costs and accuracy loss.} %our method significantly reduces computational cost while keeping accuracy loss within acceptable ranges. 
% On the LLaMA2-7B model with the PTB dataset, VS-Quant results in a high PPL of 53.46 at a 4$\times$ BOPs reduction, while our method controls the PPL at 21.61 with a 2.39$\times$ BOPs reduction. \ms{This consistent performance improvement across different models and datasets}
% %Our method consistently demonstrates similar advantages across various models and datasets, 
% indicates the good generalizability and robustness of our quantization strategy. 
% Moreover, our method flexibly meets varying accuracy-efficiency requirements %within relative accuracy loss thresholds. 
% %For instance, 
% \ms{offering} 2.74$\times$ and 2.95$\times$ BOPs reduction at 0.1\% and 1\% relative accuracy loss, respectively, on the OPT-1.3B model with the WikiText2 dataset.

%on the OPT-1.3B model with the WikiText2 dataset, our method achieves 2.31$\times$ and 2.95$\times$ BOPS reduction at 0.1\% and 1\% relative accuracy loss, respectively.
%The model scale and datasets also influence the optimal precision combination.

% In summary, our proposed search algorithm achieves an impressive accuracy-efficiency balance across various models and datasets. Compared to FIGNA and VSQuant, our method demonstrates clear advantages in computational cost reduction and accuracy preservation, exhibiting stronger practical value. The unique advantages of our method—adaptiveness, accuracy-efficiency trade-off, and practical deployment value—highlight its potential for further optimization to meet more practical constraints.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/perf_benchmark_v4.pdf}
%     \caption{Speedup and energy efficiency comparison across the accelerators.}
%     \label{fig:benchmark}
% \end{figure*}

\rOneFC{Fig.~\ref{fig:combination_heatmap} presents the best precision combination driven by 0.1\% and 1\% relative accuracy loss, revealing the patterns of quantization precision choices for different activation parts across models. The optimal precision combinations vary under different accuracy constraints, highlighting the importance of the adaptive precision combination search algorithm in automatically adjusting the mantissa lengths based on LLM module sensitivity.
Examining the module types reveals that $A_{qkv}$, involved with the $Q$, $K$, and $V$ projection layers, prefers higher precision due to higher sensitivity, while $A_u$ and $A_d$ in the feed-forward layers, especially $A_d$, can be more aggressively quantized to lower precision, demonstrating higher tolerance.}

% \ms{[Feel fig.15 should be firstly discussed before the accuracy comparison, as the performance of "our" in table I is based on the best bit combination, no?]}
% Fig.~\ref{fig:combination_heatmap} shows the best precision combination heatmaps \ms{driven by 0.1\% and 1\% relative accuracy loss} and reveals the patterns of quantization precision choices for different activation parts \ms{across various} models. $A_{qkv}$ involved with the $Q$, $K$ and $V$ projection layers prefer higher precision, ranging 6 to 8 bits, indicating a higher sensitivity to quantization precision, while $A_u$ and $A_d$ in the feed-forward layers, especially $A_d$, can be \ms{more aggressively} quantized to lower precision, ranging from 4 to 6 bits, demonstrating higher tolerance. \ms{It is important to note that the accuracy and performance of benchmarks for the Anda scheme are derived from these optimal precision settings and will be compared with the SotA methods in the following subsections.}



% \subsection{Area and Power Breakdown}

% \textbf{PE-level Evaluation.}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/perf_benchmark_v4.pdf}
%     \caption{Speedup and energy efficiency comparison across the accelerators.}
%     \label{fig:benchmark}
% \end{figure*}

\subsection{PE-level Evaluation}
%FP-INT operations are the most prevalent in weight-only quantized LLMs, making the PE crucial for enhancing computational efficiency \rg{[Why?]}. We therefore first evaluate the hardware performance at the PE level.
% Next, we quantitatively compare the proposed \ms{Anda} PE with \ms{common} FP-FP units~\cite{mach2020fpnew}, FP-INT units, the \ms{dedicated} PE units proposed by Y. Kim~\cite{kim2023winning} and FIGNA~\cite{jang2024figna}, \ms{receptively}. %For a fair comparison, 
% We ensure all \ms{PEs} with equal computational throughput \ms{per cycle} to observe power and area differences \ms{for an equitable evaluation.} \ms{One same dot product workload is processed by different PEs to collect the resulting area efficiency (TOPS/mm$^2$) and energy efficiency (TOPS/W)}. All results are normalized to the FP-FP unit.

\rOneFC{We quantitatively compare the proposed Anda PE with common FP-FP units~\cite{mach2020fpnew}, enhanced FP-INT units, and dedicated PE units proposed by Y. Kim et al.~\cite{kim2023winning} and FIGNA~\cite{jang2024figna}, respectively.}
\rOneFC{To ensure an equitable evaluation, all PEs are configured with equal computational throughput per cycle. We process an identical dot product workload across different PEs to measure area efficiency (TOPS/mm$^2$) and energy efficiency (TOPS/W). All results are normalized to the FP-FP unit.}

%that complete the same number of FP-INT operations per cycle to observe area and power differences under equal computational throughput . 
%Additionally, we have all PE units execute the same dot product operation and record their operation cycles to obtain area efficiency (TOPS/mm$^2$) and energy efficiency (TOPS/W). For consistency, all results are normalized to the FP-FP unit.
% \ms{[Can we mark the (a),(b),(c),(d) for each small figure in figure16?]}
% Fig.~\ref{fig:pe_level}\ms{ (a) and (b) shows the area and power of Anda and baselines.}
%As for area and power, 
% \ms{Anda consumes less than 60\% power and area overheads compared to FP-FP and FP-INT PEs.}
%the Anda PE reduces area by 77\% and 63\% and power consumption by 80\% and 62\% compared to FP-FP and FP-INT PEs, respectively. 
% This significant reduction is achieved \ms{by the shared exponent,} eliminating complex alignment and normalization processes \ms{in traditional floating-point operations}. 
\rOneFC{Fig.~\ref{fig:pe_level} (a) and (b) illustrate the area and power consumption of Anda and baseline PEs.}
\rOneFC{Anda presents significant reductions, consuming less than 60\% of the power and area compared to FP-FP and FP-INT PEs. This is primarily achieved through shared exponents, which eliminates complex alignment and normalization processes typical in FP operations.} 
\rOneFC{Compared to the PE of Y. Kim et al., Anda offers 12\% and 29\% reductions in area and power, respectively. This improvement stems from Anda's avoidance of high-overhead ultra-wide multipliers and registers necessary for maintaining FP16 precision.}
% \ms{[Why can Anda avoid this?]}. 
%However, the Anda PE incurs 27\% and 18\% additional area and power overhead compared to FIGNA's PE due to its bit-serial design, which requires more control logic and registers than FIGNA's bit-parallel MAC operations.
%Despite the additional \ms{27\%} power and \ms{18\%} area overhead 
% \ms{Despite incurring an additional 27\% power and 18\% area overhead compared to FIGNA due to its uncompacted bit-serial structure}, Anda \ms{featuring} adaptive precision can 
% %'s adaptive precision feature, which adjusts the mantissa length before deployment through adaptive precision search, 
% significantly lower \ms{workload execution time,} %computation cycles for the same %dot product operations, 
% %enhancing 
% \ms{allowing higher} area and energy efficiency \ms{in system level}. 
\rOneFC{Moreover, despite incurring a 27\% power and 18\% area overhead compared to FIGNA due to its uncompacted bit-serial structure, Anda's adaptive precision capability can significantly reduce workload execution time, leading to higher area and energy efficiency.}
% \rOneFC{Fig.~\ref{fig:pe_level} (c) and (d) further exhibit Anda's superior area and energy efficiency across various mantissa bit-width configurations. We denote these configurations as Anda-M(\textit{x}), where \textit{x} represents the number of preserved mantissa bits.}
\rOneFC{Fig.~\ref{fig:pe_level} (c) and (d) further exhibit superior area and energy efficiency of Anda PE with variable-length mantissas, labeled as Anda-M(\textit{x}), where \textit{x} is the number of preserved mantissa bits.}
\rOneFC{Refering back to Fig.~\ref{fig:combination_heatmap}, the retained mantissa lengths of Anda typically range between 4$\sim$8 bits with negligible 1\% accuracy impact, resulting in the area and energy efficiency improvements of 1.38$\sim$2.48$\times$ and 1.52$\sim$2.74$\times$ over FIGNA, respectively.}
% Fig.~\ref{fig:pe_level} \ms{(c) and (d) further exhibit the area and energy efficiency priority of Anda under varied (\textit{x})} mantissa \ms{bit}, donated as Anda-M\textit{x}. \ms{Refering back to}
%As shown in Fig.~\ref{fig:pe_level}, the number \textit{x} in
%Anda-M\textit{x} denotes the retained mantissa length in the Anda format. 
%The Anda PE surpasses FIGNA's PE in area and energy efficiency when the mantissa lengths are 11 and 12, respectively. According to 
% fig.~\ref{fig:combination_heatmap}, 
% the retained mantissa lengths of Anda typically range between 4-8 bits \ms{with negligible accuracy impact}, resulting in the area and energy efficiency improvements of 1.38$\sim$2.48$\times$ and 1.52$\sim$2.74$\times$ over FIGNA's PE.




% \textbf{Anda System Evaluation.}

% \rOneFC{[Goal: Estimate and analyze the area and power consumption of the hardware architecture based on the Anda format. Break down the area and power distribution of different modules, illustrating how Anda significantly reduces storage and computational overheads.]}

% \subsection{Speedup and Efficiency Improvements}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/anda_combined_charts.pdf}
%     \caption{Area and power breakdown of Anda.}
%     \label{fig:breakdown}
% \end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}




% \rOneFC{[Goal: Evaluate the acceleration effects of Anda in terms of speedup, energy efficiency, and area efficiency metrics. Provide quantitative comparisons with traditional approaches and analyze the main sources of performance improvements.]}

\subsection{System-Level Evaluation}
%For a fair comparison, we configure the baselines to have the same clock frequency and the same processing capabilities to perform an equivalent number of FP MAC operations as Anda for performance and energy evaluation.

% Fig.~\ref{fig:benchmark} presents the system-level speedup and energy efficiency comparison between Anda and several baseline architectures.
% \as{Fig.~\ref{fig:benchmark} compares the system-level speedup and energy efficiency reduction between Anda and several baseline architectures.}
\rOneFC{Fig.~\ref{fig:benchmark} presents a comprehensive comparison of system-level speedup and energy efficiency between Anda and several baseline architectures, where the results are normalized to FP-FP baseline.}
\rOneFC{Anda exhibits significant advantages in both metrics across all benchmarks.}
\rOneFC{When ensuring lossless accuracy within 0.1\%, Anda achieves an average speedup of 2.143$\times$ and an average energy efficiency improvement of 3.070$\times$ compared to FP-FP baseline.}
\rOneFC{Allowing a 1\% accuracy loss tolerance further enhances Anda's performance, yielding an average speedup of 2.489$\times$ and an average energy efficiency improvement of 3.160$\times$.}
% \rOneFC{With a 1\% negligible accuracy loss, Anda's performance gains are even more pronounced, demonstrating an average speedup of 2.489$\times$ and an average energy efficiency improvement of 3.160$\times$.}
% \rOneFC{In contrast with the work of Y. Kim et al. and FIGNA, which focus primarily on energy optimization through customized designs but fall short in computation acceleration during computation, Anda leverages its bit-serial architecture to skip the computation of redundant mantissa bits identified at compile time. Moreover, BPC compresses output by storing only the essential mantissa bits in memory, significantly minimizing memory stalls and eliminating memory accesses, thereby improving energy efficiency.}
In contrast to Y. Kim et al. and FIGNA, which solely optimize energy during computation, Anda leverages its bit-serial architecture to skip the computation of redundant mantissa bits identified by the adaptive precision search algorithm. Moreover, the BPC compresses the output to the Anda data type, significantly minimizing memory stalls and reducing the required memory accesses. 
\rOneFC{These capabilities result in Anda's superior speedup and energy efficiency, surpassing 2.143$\times$ and 2.069$\times$, respectively.}
% These capabilities result in Anda's superior speedup and energy efficiency over 2.143$\times$ and 2.069$\times$, respectively.

\rOneFC{To gain deeper insights into Anda's energy optimizations, we conduct an energy breakdown analysis on the LLaMA-13B model.}
\rOneFC{As shown in Fig.~\ref{fig:energy_breakdown}, compared to the FP-FP baseline, Anda achieves energy reductions of 90\%, 54\%, and 50\% in computation, SRAM access, and DRAM access, respectively.}
\rOneFC{The computational energy saving stems from the massive number of skipped computations and the efficient PE units free of alignment and normalization. 
% Concurrently, Anda's unique compressed data format substantially reduces the energy overhead associated with data movement. 
% Compared to other architectures, Anda consistently saves energy over 2.04$\times$ at least.}
Moreover, Anda's compressed data format substantially reduces the energy overhead associated with data movement, consistently saving energy by at least 2.043$\times$ compared to other architectures.}
%including FP-FP, FP-INT, Y.Kim, and FIGNA, on 9 different language models ranging from 1.3B to 30B parameters, covering the OPT, LLaMA, and LLaMA-2 series. All results are normalized to the FP-FP baseline.
%\textbf{Speedup:} 

% \ms{Anda}
% %The experimental results d
% demonstrates %that Anda exhibits 
% substantial advantages in both 
% speedup and energy efficiency \ms{across all benchmarks, as shown in Fig.~\ref{fig:benchmark}(a).} 
% \ms{In sharp contrast to Y. Kim and FIGNA, which focus on energy optimization} through customized designs \ms{but fall short in computation acceleration, Anda leverages its bit-serial architecture to skip the computation of redundant mantissa bits identified at compile time. %On the other hand
% Besides, BPC compresses output by storing only the essential mantissa bits in memory, significantly minimizing memory stalls and eliminating memory accesses. This capability further contributes to Anda's superior performance and energy efficiency. In concert term,} 

% \as{Anda demonstrates substantial advantages in both metrics across all benchmarks. Compared to the work of Y. Kim and FIGNA, which focuses solely on energy optimization, the Anda architecture leverages its bit-serial architecture to skip the computation of pruned mantissa bits. Moreover, the BPC compresses the output to the Anda data type, significantly minimizing memory stalls and reducing the required memory accesses. These capabilities result in Anda's superior speedup and energy efficiency.}

 %lower the power consumption of individual operations through customized designs, 
%and energy efficiency. 
% Under an accuracy loss of 0.1\%, 
% Anda achieves an average speedup of 1.823$\times$ and an average energy efficiency improvement of 2.223$\times$ 
% compared to %the FP-FP 
% baselines. When allowing a 1\% accuracy loss, Anda's performance gains are even more pronounced, with an average speedup of 2.428$\times$. and an average energy efficiency improvement of 3.148$\times$. % over FP-FP.
%Anda's speedup improvements can be attributed to its adaptive precision search mechanism and efficient compute unit design. By quickly searching for the optimal data format that satisfies the accuracy requirements before deployment, Anda significantly reduces the computational overhead. In contrast, while Y.Kim and FIGNA lower the energy consumption of individual operations through customized designs, they do not achieve compute acceleration. 
%Moreover, 
%The experimental data \ms{also} reveals differences in accuracy sensitivity across model series. The OPT series exhibits higher tolerance to accuracy loss compared to the LLaMA series, enabling \ms{a higher speedup through} the \ms{adoption} of lower data bit widths. %to achieve higher speedups.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.96\linewidth]{figs/energy_breakdown_with_savings_v2.pdf}
    \caption{Energy breakdown of Anda in contrast with the baseline accelerators. Energy consumption during the LLaMA-13B inference is evaluated.}
    \label{fig:energy_breakdown}
\end{figure}

%\textbf{Energy:} 
%In terms of energy efficiency, 
%Anda's advantages stem from two main aspects: efficient compute unit design and significant memory access savings. 
% To gain a deeper understanding of Anda's energy optimization mechanisms, we conducted an energy breakdown analysis on the LLaMA-13B model. As shown in Fig.~\ref{fig:energy_breakdown}, compared to FP-FP, Anda achieves energy reductions of 90\%, 54\%, and 50\% in computation, SRAM access, and DRAM access, respectively. %On one hand
% \ms{Specifically, 90\% computational energy saving comes from the massive skipped computations and the efficient alignment and normalization free}
%this can be attributed to Anda's use of 
%customized integer 
% MAC units. %of \ms{Anda architecture}, which avoid the energy-intensive alignment and normalization operations \ms{presented} in floating-point %computations
%\ms{operations}. %On the other hand, 
% \ms{Simultaneously},
% Anda's unique compressed data format substantially reduces the energy overhead associated with data movement.
% In the comparison \ms{of} the energy %efficiency improvements 
% \ms{reduction with} other architectures, \ms{Anda saves over $1.5\times$ energy in general. } %This is because}  
% are relatively limited.
%FP-INT, Y.Kim, and FIGNA primarily focus on optimizing compute units, reducing computation energy to some extent. However, 
%they overlook memory access optimization, limiting their overall energy efficiency gains.

% In conclusion, Anda demonstrates exceptional speedup and energy efficiency performance on inference tasks across a wide range of LLMs, owing to its coordinated optimizations in both computation and storage. Anda's adaptive precision search and data compression techniques effectively balance the trade-off between accuracy and performance. At the same time, its customized compute units and data access methods maximize hardware resource utilization, enabling Anda to significantly outperform other architectures in terms of speedup and energy efficiency.






\begin{table}[tb]
\centering
\caption{Area and Power Characteristics of Anda}
\label{tab:area_breakdown}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}llcc@{}}
\toprule
Component               & Setup                         & Area {[}mm$^2${]}        & Power {[}mW{]}            \\ \midrule
MXU & 16$\times$16 APUs & 0.41 (18.89\%)           & 54.34 (66.94\%)           \\
BPC    & 16 Lanes                      & 0.07 (3.23\%)            & 1.06 (1.31\%)             \\
Vector Unit             & 64 FPUs                       & 0.05 (2.30\%)            & 0.87 (1.07\%)             \\
Activation Buffer       & 1MB (Mant.) + 0.125MB (Exp.)  & 0.87 (40.09\%)           & 16.94 (20.87\%)           \\
Weight Buffer           & 1MB                           & 0.80 (36.87\%)           & 7.96 (9.81\%)             \\
Others                  & Top controller                & 0.01 (0.46\%)            & 0.01 (0.00\%)             \\ \midrule
\textbf{Total}          & \textbf{}                     & \textbf{2.17 (100.00\%)} & \textbf{81.18 (100.00\%)} \\ \bottomrule
\end{tabular}%
}
\end{table}

\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/acc_eff_trade_off.pdf}
    \caption{Speedup and energy efficiency improvement of Anda over FP-FP baseline towards various acceptable accuracy losses.}
    \label{fig:acc_eff_trade_off}
\end{figure}
\subsection{Power and Area breakdown}
% We conduct a detailed analysis of the area and power characteristics of the Anda architecture \ms{handling} %when running FP-INT operations 
% LLaMA-13B within a 1\% accuracy drop.
% Table~\ref{tab:area_breakdown} presents the \ms{area breakdown}
% %resource allocation 
% and power distribution %among various components 
% of Anda architecture.
% Operating at a clock frequency of 285 MHz and 0.8 V nominal voltage, Anda has an area of 2.17 mm$^2$ with 81.18 mW power consumption.
\rOneFC{We conduct a detailed hardware analysis of the Anda architecture for LLaMA-13B inference within 1\% accuracy loss. Table~\ref{tab:area_breakdown} presents the area breakdown and power distribution.}
\rOneFC{Operating at 285 MHz and 0.8 V, Anda occupies 2.17 mm$^2$ with 81.18 mW power consumption.}
The MXU, serving as the core computing component of the Anda architecture, consumes 66.94\% of the total power despite occupying only 18.89\% of the area. 
The BPC unit, which enables efficient online compression from the full-precision FP outputs to the Anda format, costs a small portion of the total area (3.23\%) and power consumption (1.31\%).
%has very small area and power consumption ratios of 3.23\% and 1.31\%, respectively. 
%This \ms{demonstrates the BPC }
%indicates that the additional overhead this component introduces is minimal, allowing for efficient format conversion.
On-chip SRAM is the primary area contributor, with the activation buffer and weight buffer accounting for 40.09\% and 36.87\% of the total area, respectively. Their power consumption ratios are relatively low at 20.87\% and 9.81\% because of efficient data reuse within the Anda system.
%Despite occupying a large area, these buffers play a crucial role in supporting efficient data access and management, ensuring the system's fast response. \rg{[Why 'despite'? Isn't it good that large importance = large area?]}





% \rOneFC{[Goal: Discuss the trade-off between accuracy and performance under the Anda format. Plot curves such as accuracy-latency and accuracy-energy efficiency to demonstrate how Anda achieves a better balance.]}
\subsection{Accuracy-Performance Trade-off}
\rOneFC{This section explores speedup and energy efficiency improvements of the Anda system over the FP-FP baseline with accuracy loss constraints ranging from 0.1\% to 5\%.}
\rOneFC{As shown in Fig.~\ref{fig:acc_eff_trade_off}, using LLaMA-13B as an example, Anda achieves a 1.73$\times$ speedup and 2.95$\times$ energy efficiency improvement with only 0.1\% accuracy loss, increasing to 2.74$\times$ and 3.22$\times$, respectively, when the constraint is relaxed to 5\%. All models exhibit significant acceleration and efficiency gains as the tolerated accuracy loss increases.}
\rOneFC{Notably, OPT and LLaMA models exhibit distinct characteristics when using the Anda format.}
\rOneFC{This stems from OPT's lower sensitivity to bit-width reductions, allowing the use of shorter mantissa bit-widths with minimal accuracy sacrifice. Consequently, under tighter accuracy constraints, e.g., 0.1\%$\sim$0.5\%, OPT models achieve greater speedups and energy efficiency improvements compared to LLaMA models. However, as accuracy constraints relax, their performance gains gradually converge.}
% \rOneFC{Under tighter accuracy constraints, e.g., 0.1\%$\sim$1\%, OPT models consistently achieve greater speedups and energy efficiency improvements compared to LLaMA models. This is due to OPT's lower sensitivity to bit-width reductions, allowing for shorter mantissa bit-widths with minor accuracy sacrifice.}
% \rOneFC{The differences in accuracy-performance trade-offs between OPT and LLaMA models highlight the impact of model architecture on Anda's effectiveness.}
% \rOneFC{To leverage these differences and adapt to various model characteristics, our architecture can grant the balance between the system performance and accuracy in diverse practical application scenarios with the integration of the adaptive precision combination search algorithm with Anda format, enabling efficient LLM inference under varying requirements.}
% \rOneFC{The differences in accuracy-performance trade-offs between OPT and LLaMA models highlight the impact of model architecture on Anda's effectiveness.}
\rOneFC{By integrating the adaptive precision combination search algorithm with the Anda format, our architecture achieves flexible balancing of system performance and accuracy across diverse practical application scenarios, enabling efficient LLM inference under different LLM architectures and varying requirements.}
% \rOneFC{Under tighter constraints (0.1\%-1\%), OPT models achieve greater speedups, suggesting their architecture is more amenable to BFP representation. This allows for shorter mantissa bit-widths with minimal accuracy impact. Energy efficiency trends mirror the speedup patterns, with the OPT series generally outperforming LLaMA.}
%Maintaining acceptable accuracy while pursuing high performance is a core challenge in deep learning acceleration. 
% This section explores the performance improvements of Anda compared to the FP-FP baseline under various accuracy loss constraints.
% We %conduct experiments 
% \ms{evaluate Anda system speedup and energy efficiency} on multiple LLMs from the OPT and LLaMA series, with accuracy loss constraints ranging from 0.1\% to 5\%. %The evaluation metrics include speedup and energy efficiency.
% \ms{As shown in} Fig.~\ref{fig:acc_eff_trade_off}, 
% %shows the speedup as the accuracy loss constraint changes. 
% Anda already achieves a 1.6$\times$ speedup at a 0.1\% accuracy loss \ms{tolerance}. \ms{High to 3.2$\times$ speedup is obtained when}
% %As 
% the constraint relaxes to 5\%. %, the speedup significantly increases to 3.2$\times$. 
% \ms{A notable point is that} OPT and LLaMA series models exhibit different \ms{quantization characteristics}: %characteristics
% under tighter accuracy constraints (e.g., 0.1\%-1\%), OPT models achieve more significant speedup compared to LLaMA models. This is due to OPT's lower sensitivity to bit-width changes in its model design, allowing the use of %lower
% \ms{shorter} mantissa bit-widths \ms{with minor accuracy sacrifice.}
% %while maintaining high accuracy.
% %As shown in Fig.~\ref{fig:acc_eff_trade_off}, 
% \ms{Generally,} energy efficiency \ms{displays} a similar trend in Fig.~\ref{fig:acc_eff_trade_off}, \ms{OPT-series yields a higher gain compared with LLaMA-family.}
%reaching a 3.3$\times$ improvement at 10\% accuracy loss. %Even under the strict 0.1\% accuracy loss constraint, Anda still achieves nearly 3$\times$ energy efficiency improvement, demonstrating its ability to optimize energy consumption while maintaining high accuracy.
% The differences in accuracy-performance trade-offs between OPT and LLaMA models highlight the impact of model architecture on quantization effects. \ms{Integration of adaptive precision combination search algorithm with Anda format, our architecture can grant the balance between the system performance and accuracy in diverse practical application scenarios, offering}
% %This finding provides %important references 
% \ms{valuable insights} for model design and quantization strategy choices. 
%By flexibly adjusting accuracy loss constraints, Anda can adapt to various application scenarios, from high-precision scientific computing to inference tasks that allow larger errors, offering valuable flexibility for practical deployment.

% \subsection{Towards Aggressive Weight-Only Quantization Scheme}

% \subsection{Anda Architecture Scalability}

% \rOneFC{[Goal: Through theoretical analysis and experimental validation, show that the proposed Anda architecture can efficiently shift to different group size configuration, exhibiting good scalability.]}


% \begin{itemize}
%     \item Model Accuracy
%     \item PE-level Efficiency
%         \begin{itemize}
%             \item 5 Baselines: FP-FP, FP-INT, Y.KIM~\cite{kim2023winning}, FIGNA(-C)~\cite{jang2024figna}
%             \item 2 Modifications: bit-plane reduction first, element-plane reduction first
%             \item Metrics: Norm. Area/Power? (Norm. Area/Power per MAC?) [Fig.~\ref{fig:11}]
%         \end{itemize}
%     \item Anda System Breakdown 
%         \begin{itemize}
%             \item 11 Workloads: OPT Series (125M, 1.3B, 2.7B, 6.7B, 13B, 30B); Llama Series (7B, 13B, 30B); Llama-2 Series (7B, 13B);
%             \item Energy breakdown on different workloads; [Fig.~\ref{fig:12}] 
%             \item Area and power breakdown of Anda; [Fig.~\ref{fig:13}]
%         \end{itemize}
%     \item System-level Efficiency 
%         \begin{itemize}
%             \item 4 Baselines: FP-FP, FP-INT, Y.KIM~\cite{kim2023winning}, FIGNA(-C)~\cite{jang2024figna}
%             \item 11 Workloads: OPT Series (125M, 1.3B, 2.7B, 6.7B, 13B, 30B); Llama Series (7B, 13B, 30B); Llama-2 Series (7B, 13B);
%             \item Metrics
%                 \begin{itemize}
%                     \item Area Efficiency: Norm. TOPS/mm$^2$ [Fig.~\ref{fig:14}]
%                     \item Energy Efficiency: Norm. TOPS/W [Fig.~\ref{fig:15}]
%                     \item Computational Utilization: \% [Fig.~\ref{fig:16}]
%                 \end{itemize}
%         \end{itemize}
% \end{itemize}

==> archive/6-rel.tex <==
\section{Related Works}

\textbf{LLM Quantization.}
\cite{guo2022ant, guo2023olive}

\textbf{Efficient Transformer Accelerators.}
\cite{qin2023fact, fan2022adaptable, fang2022algorithm}

\textbf{Precision-scalable DNN Accelerators.}
\cite{shi2024bitwave, huang2024precision, judd2016stripes, sharify2018loom}

==> archive/7-concls.tex <==
\section{Conclusion} \label{sec:concls}
% \ms{DONT FORGET TO ADD CONCLUSION AND REMOVE ACKNOWLEDGEMENT}

% This work introduces Anda, an innovative solution for efficient large language model (LLM) inference. We address the energy and performance bottlenecks in weight-only quantized LLMs by proposing a variable-length grouped activation data format. Anda leverages the redundancy in floating-point activations across different models and modules, employing shared exponents and dynamic mantissa allocation. We develop a post-training adaptive precision search algorithm to optimize bit-width allocation, balancing accuracy and efficiency. Complementary hardware optimizations, including bit-plane data organization, bit-serial computation units, and a runtime compressor, further enhance Anda's performance. Evaluations on popular LLM families demonstrate that Anda achieves significant improvements in both speed (2.428×) and energy efficiency (3.148×) compared to existing GPU solutions. Anda's adaptability across various precision requirements and deployment scenarios enables efficient LLM inference in diverse environments, addressing critical challenges in the deployment of large language models.

% This work introduces Anda, a variable-length grouped activation data format that addresses the energy and performance bottlenecks in weight-only quantized large language model (LLM) inference. Recognizing the redundancy in FP activations across different models and modules, we propose an adaptive data format with dynamically shared exponents and adjustable mantissa widths. 
\rOneFC{This work presents Anda, a variable-length grouped activation data format that addresses energy and performance bottlenecks of weight-only quantized large language model (LLM) inference by exploiting redundancy in floating point activations across different models and their modules.}
To fully harness the potential of Anda, we develop an iterative post-training algorithm that optimizes bit-width allocation across LLM modules, balancing accuracy, energy efficiency, and inference speed.
We design complementary hardware optimizations to maximize the benefits of Anda, including a bit-plane-based data organization scheme in memory, Anda-enhanced bit-serial processing units, and a runtime bit-plane compressor. 
Our evaluations show that Anda achieves a 2.4$\times$ speedup and a 3.1$\times$ improvement in energy efficiency on average for popular LLMs compared to existing GPU-based solutions. 
With its adaptability across various application scenarios and performance requirements, Anda enables efficient LLM inference in diverse deployment environments, paving the way for broader adoption of LLMs in resource-constrained settings.
